NextGAN: Towards Simple and Scalable GAN Training for Image and Video Generation

Adversarial training enables one- and few-step image and video generation, but conventional adversarial losses supervise critic values without directly specifying the gradients used to update the generator. We present NEXTGAN, which trains a scalar critic by regressing its input gradient onto displacements between independently paired reference and generated features at interpolated locations in frozen representation spaces. For a fixed generator, this regression is equivalent to an adversarial objective with a gradient-energy penalty, while the generator retains the standard potential-based GAN update. The same objective adapts pre-trained image and video generators with up to 14B parameters, without auxiliary losses, online teacher scores, or trajectories. On ImageNet $256 \times 256$, NEXTGAN achieves one-step FIDs of 2.87 with pixel-space JiT-B and 1.54 with latent-space DiT-XL/1; its adversarial form further reaches 1.36. For text-to-video generation, a single trained Wan2.1-1.3B model supports one-, two-, and four-step sampling, achieving the highest VBench total scores among the compared 1.3B methods at one and two steps. At two steps, NEXTGAN scores 83.13, exceeding rCM and AnyFlow by 1.25 and 0.47 points, respectively. Code is available at https://github.com/LINs-lab/NextGAN.git.

==> figures/toy8_native_data/centers.tex <==
% Generated from original vector marker centers; do not edit by hand.
\toyPoint{65.80645161}{40.00000000}
\toyPoint{58.24791662}{58.24791662}
\toyPoint{39.99999887}{65.80645161}
\toyPoint{21.75208338}{58.24791662}
\toyPoint{14.19354839}{39.99999774}
\toyPoint{21.75208645}{21.75208030}
\toyPoint{40.00000031}{14.19354839}
\toyPoint{58.24792277}{21.75208953}


==> figures/toy8_native_data/logistic_0.tex <==
% Generated from original vector marker centers; do not edit by hand.
\toyPoint{40.41417864}{39.90581646}
\toyPoint{40.44728152}{39.90325303}
\toyPoint{40.58649836}{40.13321936}
\toyPoint{40.73147382}{39.83377199}
\toyPoint{41.12307447}{40.15253559}
\toyPoint{40.33770905}{39.96868067}
\toyPoint{40.80145463}{39.75011262}
\toyPoint{40.50027572}{40.12581327}
\toyPoint{40.31243418}{39.89858325}
\toyPoint{40.38169844}{39.96649718}
\toyPoint{40.56778644}{39.88890711}
\toyPoint{40.29253988}{39.94904889}
\toyPoint{40.89780765}{40.26286107}
\toyPoint{40.68574625}{39.88023336}
\toyPoint{40.16941315}{39.82813966}
\toyPoint{40.45256307}{39.93493233}
\toyPoint{40.67207116}{39.92559972}
\toyPoint{40.29241106}{39.87669134}
\toyPoint{41.09261880}{40.22338783}
\toyPoint{40.70530936}{40.31790637}
\toyPoint{40.22477214}{39.87115855}
\toyPoint{40.36353902}{39.89782256}
\toyPoint{40.56371823}{39.90430647}
\toyPoint{40.73310704}{40.00602238}
\toyPoint{40.11335585}{39.79580598}
\toyPoint{40.77322606}{39.87847762}
\toyPoint{40.54787191}{39.93317247}
\toyPoint{40.68903830}{40.13260822}
\toyPoint{40.31608961}{39.91548536}
\toyPoint{40.14901531}{39.80821746}
\toyPoint{40.56362839}{39.89025702}
\toyPoint{40.44838007}{40.01479738}
\toyPoint{40.61167815}{39.99039913}
\toyPoint{40.76887877}{39.93142161}
\toyPoint{40.41321785}{40.06170431}
\toyPoint{39.99254375}{39.58745972}
\toyPoint{40.59438814}{39.90645937}
\toyPoint{40.79108880}{39.82384354}
\toyPoint{40.70775771}{40.05958464}
\toyPoint{40.31564346}{39.88202971}
\toyPoint{40.71249806}{39.82892765}
\toyPoint{40.89505363}{40.44367967}
\toyPoint{40.54728427}{40.16575698}
\toyPoint{40.56904189}{39.92268609}
\toyPoint{40.44486556}{39.99250132}
\toyPoint{40.74191757}{39.81679067}
\toyPoint{40.71198219}{39.84585994}
\toyPoint{40.74811953}{40.05450662}
\toyPoint{40.58712022}{39.96493975}
\toyPoint{40.91794460}{40.14359355}
\toyPoint{40.56195225}{40.01379833}
\toyPoint{40.74383655}{40.12804957}
\toyPoint{40.87638690}{40.01353180}
\toyPoint{40.88017746}{39.68431284}
\toyPoint{40.67448919}{39.87985422}
\toyPoint{40.16651192}{39.82949536}
\toyPoint{40.54591875}{40.07426792}
\toyPoint{40.59816837}{39.90723394}
\toyPoint{40.27179884}{39.86322403}
\toyPoint{40.24894827}{39.87901423}
\toyPoint{40.18748927}{39.84331251}
\toyPoint{40.43590184}{39.90884842}
\toyPoint{40.78488257}{39.94780251}
\toyPoint{40.77969451}{39.90794973}
\toyPoint{40.29176791}{39.91455231}
\toyPoint{40.74677722}{40.05335795}
\toyPoint{40.49709995}{40.01062411}
\toyPoint{40.47530176}{40.03635060}
\toyPoint{40.97803858}{40.13647430}
\toyPoint{40.57903374}{39.88401472}
\toyPoint{40.58557511}{39.92609627}
\toyPoint{40.59681939}{39.99507565}
\toyPoint{40.23990235}{39.87747210}
\toyPoint{40.36860435}{39.90476390}
\toyPoint{40.70544972}{40.24330640}
\toyPoint{40.30829974}{39.88194238}
\toyPoint{40.42803268}{40.06209410}
\toyPoint{40.69500645}{39.89225034}
\toyPoint{40.46470271}{39.90400480}
\toyPoint{40.20550629}{39.85625455}
\toyPoint{40.75190269}{39.89968807}
\toyPoint{40.33061324}{39.88693842}
\toyPoint{40.51128879}{40.03724997}
\toyPoint{40.71636890}{40.07458936}
\toyPoint{40.52906111}{39.89714899}
\toyPoint{40.88353388}{40.22413731}
\toyPoint{41.20082171}{40.01230136}
\toyPoint{40.11599941}{39.79599659}
\toyPoint{41.00803346}{39.52997008}
\toyPoint{40.61905302}{40.15133521}
\toyPoint{40.73159049}{39.87598421}
\toyPoint{40.34465492}{39.89053391}
\toyPoint{40.61918329}{40.01628406}
\toyPoint{41.60852075}{40.29167682}
\toyPoint{40.52366742}{39.94620009}
\toyPoint{40.68285148}{39.90556632}
\toyPoint{40.13999453}{39.81096255}
\toyPoint{40.33898363}{39.89260524}
\toyPoint{40.81985535}{39.79885893}
\toyPoint{40.80489189}{39.98854900}
\toyPoint{40.39307360}{40.04024367}
\toyPoint{40.88989158}{40.04565426}
\toyPoint{40.33143807}{39.94323540}
\toyPoint{39.97629466}{39.69666932}
\toyPoint{40.65642720}{39.93822053}
\toyPoint{40.69739694}{40.06528046}
\toyPoint{40.78138901}{40.13588128}
\toyPoint{40.87955210}{40.06752139}
\toyPoint{40.79922546}{39.78359339}
\toyPoint{40.44419126}{39.93787617}
\toyPoint{40.35847911}{39.94913171}
\toyPoint{40.53911964}{40.06028307}
\toyPoint{40.89894399}{39.93873666}
\toyPoint{40.60305509}{39.91716548}
\toyPoint{40.40602059}{40.00596860}
\toyPoint{40.64924359}{39.87742413}
\toyPoint{40.60762153}{40.03232408}
\toyPoint{40.68341561}{40.12331408}
\toyPoint{40.66806424}{40.09236922}
\toyPoint{40.39440886}{39.84962957}
\toyPoint{40.80063093}{40.00867497}
\toyPoint{40.79157650}{39.97115923}
\toyPoint{40.72153302}{39.82494851}
\toyPoint{40.16463880}{39.82804639}
\toyPoint{40.22167261}{39.85537576}
\toyPoint{40.40577227}{39.90044916}
\toyPoint{40.58631022}{40.02586556}
\toyPoint{40.69155309}{39.94891435}
\toyPoint{40.40997656}{39.89990838}
\toyPoint{40.67125319}{39.94287196}
\toyPoint{40.65530048}{40.24706981}
\toyPoint{40.43457833}{39.94143346}
\toyPoint{40.74248915}{39.90399632}
\toyPoint{40.42152458}{39.92631135}
\toyPoint{41.06947230}{40.27063907}
\toyPoint{40.26543213}{39.87591313}
\toyPoint{40.35864865}{39.89309676}
\toyPoint{40.35843496}{39.93709823}
\toyPoint{40.66486934}{39.89993861}
\toyPoint{40.18926643}{39.83220865}
\toyPoint{40.74718450}{40.35389652}
\toyPoint{40.62858212}{39.87074418}
\toyPoint{40.53782021}{39.98939165}
\toyPoint{40.94752937}{40.42852351}
\toyPoint{40.86359314}{40.07886133}
\toyPoint{40.38927310}{40.01594775}
\toyPoint{40.78850946}{39.89526671}
\toyPoint{40.66968390}{39.86935206}
\toyPoint{40.21314078}{39.85296719}
\toyPoint{40.68323901}{40.00264058}
\toyPoint{40.76609821}{40.28910070}
\toyPoint{40.44348581}{39.94881193}
\toyPoint{40.76179860}{39.85762964}
\toyPoint{40.11726591}{39.79638916}
\toyPoint{40.87595774}{39.87402175}
\toyPoint{40.46633698}{40.00803123}
\toyPoint{40.57334347}{39.88540740}
\toyPoint{40.10376654}{39.79077777}
\toyPoint{40.82526726}{40.07542498}
\toyPoint{40.63477870}{40.04205195}
\toyPoint{40.37601364}{39.89647429}
\toyPoint{40.46002269}{39.96420973}
\toyPoint{40.36374095}{39.97522055}
\toyPoint{40.47429194}{39.96975341}
\toyPoint{40.57316889}{40.03390826}
\toyPoint{40.61436084}{39.89118121}
\toyPoint{40.49982994}{39.97947764}
\toyPoint{40.70978615}{39.88876920}
\toyPoint{40.88665178}{39.81854307}
\toyPoint{40.48588168}{40.00080201}
\toyPoint{40.70759539}{40.26503128}
\toyPoint{40.89689599}{40.00075098}
\toyPoint{40.68656225}{40.11434021}
\toyPoint{40.72635672}{40.22975617}
\toyPoint{40.76871586}{40.09987140}
\toyPoint{40.28599770}{39.87507233}
\toyPoint{40.60982896}{40.08449968}
\toyPoint{40.62128305}{39.94836235}
\toyPoint{40.67340357}{40.07238350}
\toyPoint{40.63109681}{39.86753327}
\toyPoint{40.12452799}{39.79743323}
\toyPoint{40.34427374}{39.93628567}
\toyPoint{40.30896337}{39.92447531}
\toyPoint{41.03351368}{40.00932914}
\toyPoint{40.33290466}{39.98612262}
\toyPoint{40.82875317}{39.70951609}
\toyPoint{40.60198768}{39.95024202}
\toyPoint{40.72422090}{39.84880445}
\toyPoint{40.45715936}{39.90919249}
\toyPoint{40.74291595}{40.08763065}
\toyPoint{40.96117123}{40.18997163}
\toyPoint{40.34692819}{39.98238954}
\toyPoint{40.78073966}{39.86819880}
\toyPoint{40.80133340}{39.74836981}
\toyPoint{40.66298362}{39.93016300}
\toyPoint{40.52070747}{40.04781829}
\toyPoint{40.67665841}{40.03233809}
\toyPoint{40.32365149}{39.89627213}
\toyPoint{40.46695605}{39.90862742}
\toyPoint{40.67476553}{40.06235662}
\toyPoint{40.45764528}{39.97141365}
\toyPoint{40.47979802}{39.90753459}
\toyPoint{40.95999164}{39.84168210}
\toyPoint{40.59228905}{39.93189218}
\toyPoint{40.32251506}{39.89890508}
\toyPoint{40.42922377}{39.90147171}
\toyPoint{40.29477537}{39.96052706}
\toyPoint{40.52953593}{39.90288786}
\toyPoint{40.34891461}{39.89085238}
\toyPoint{40.70746690}{39.82005685}
\toyPoint{40.97888352}{40.10203036}
\toyPoint{40.52259497}{39.96707180}
\toyPoint{40.54134361}{39.93119318}
\toyPoint{40.36371129}{39.94609251}
\toyPoint{40.66039485}{39.90033957}
\toyPoint{40.38225492}{39.90286143}
\toyPoint{40.43136324}{39.96933575}
\toyPoint{40.82285818}{39.76625229}
\toyPoint{40.64673275}{40.03205677}
\toyPoint{40.64709004}{39.86022103}
\toyPoint{40.47599635}{39.92243616}
\toyPoint{40.59110176}{40.02116497}
\toyPoint{40.30854147}{39.90214240}
\toyPoint{40.42822871}{39.98575563}
\toyPoint{40.44189172}{39.90180918}
\toyPoint{40.73742011}{39.85025544}
\toyPoint{40.67401235}{39.85257123}
\toyPoint{40.33680253}{39.98057237}
\toyPoint{40.89395460}{39.65869092}
\toyPoint{40.83289358}{40.08192047}
\toyPoint{40.40002758}{39.90080160}
\toyPoint{40.48284305}{40.04152181}
\toyPoint{40.18702721}{39.83665168}
\toyPoint{40.74522683}{39.94515077}
\toyPoint{40.41848974}{39.98167456}
\toyPoint{40.96036907}{40.25299487}
\toyPoint{40.84588701}{39.71966698}
\toyPoint{40.69004110}{40.02783346}
\toyPoint{40.36895535}{39.95802948}
\toyPoint{40.99326612}{40.25223654}
\toyPoint{40.58757374}{39.92825120}
\toyPoint{40.50173892}{40.15586292}
\toyPoint{40.50669135}{39.90003048}
\toyPoint{40.17818054}{39.83931244}
\toyPoint{40.36752359}{39.91045325}
\toyPoint{40.57301396}{39.89927942}
\toyPoint{41.17923752}{40.12358715}
\toyPoint{40.53649030}{39.93146631}
\toyPoint{40.64182834}{39.85937625}
\toyPoint{40.64930647}{40.09246997}
\toyPoint{40.22735605}{39.85549332}
\toyPoint{40.25693000}{39.87603734}
\toyPoint{41.05876096}{39.84083625}
\toyPoint{40.63882225}{40.05346069}
\toyPoint{40.83056092}{39.80372890}
\toyPoint{40.68627240}{40.29417728}
\toyPoint{40.38560163}{40.02346373}
\toyPoint{40.42358372}{39.90108901}
\toyPoint{40.88165172}{40.44477534}
\toyPoint{40.25063381}{39.91051499}
\toyPoint{40.82001321}{40.10834687}
\toyPoint{40.28374676}{39.91293069}
\toyPoint{40.53066847}{39.89790275}
\toyPoint{40.53230591}{40.00751371}
\toyPoint{40.77779726}{39.81610965}
\toyPoint{40.76734904}{39.86777774}
\toyPoint{40.37317180}{39.96980117}
\toyPoint{40.86726229}{39.80093453}
\toyPoint{40.56247336}{40.08883178}
\toyPoint{40.54666847}{39.96652993}
\toyPoint{40.56517836}{40.12693847}
\toyPoint{40.89262551}{40.19450476}
\toyPoint{40.38204597}{39.89855095}
\toyPoint{40.62395132}{39.86749901}
\toyPoint{40.47736081}{39.91261771}
\toyPoint{40.64762951}{39.86840873}
\toyPoint{40.23354109}{39.84650674}
\toyPoint{40.82693158}{39.80649984}
\toyPoint{40.33871157}{39.91756653}
\toyPoint{40.67732002}{39.90278457}
\toyPoint{40.64830357}{39.87395296}
\toyPoint{40.07586003}{39.71605799}
\toyPoint{40.44551271}{39.90624647}
\toyPoint{40.50663314}{39.92887403}
\toyPoint{40.49491424}{39.90558363}
\toyPoint{40.70964934}{40.36623103}
\toyPoint{40.49116011}{40.05628572}
\toyPoint{40.55924933}{40.08944383}
\toyPoint{40.41592967}{39.94190002}
\toyPoint{40.61613913}{40.05422867}
\toyPoint{40.53617935}{39.91007350}
\toyPoint{40.70498047}{40.26164819}
\toyPoint{40.40618229}{39.90271552}
\toyPoint{40.86094506}{39.97165857}
\toyPoint{40.73126939}{39.80275225}
\toyPoint{40.49450897}{39.91108663}
\toyPoint{41.06424805}{40.59542117}
\toyPoint{40.57667898}{39.97362862}
\toyPoint{40.89261993}{40.29501021}
\toyPoint{39.99272338}{39.65498327}
\toyPoint{40.58481857}{39.88760047}
\toyPoint{40.63170310}{39.95628816}
\toyPoint{40.22628697}{39.88494265}
\toyPoint{40.33792805}{39.95555902}
\toyPoint{40.88047789}{40.50078227}
\toyPoint{40.19864625}{39.85598354}
\toyPoint{40.28714737}{39.91792141}
\toyPoint{40.45616425}{39.91034052}
\toyPoint{40.45119332}{39.90202150}
\toyPoint{40.45260268}{39.96062534}
\toyPoint{40.87916226}{40.11310176}
\toyPoint{40.08664006}{39.77838161}
\toyPoint{40.36625615}{40.00200305}
\toyPoint{40.54329220}{39.99824997}
\toyPoint{40.89968039}{40.22447277}
\toyPoint{40.26958287}{39.93388295}
\toyPoint{40.62182353}{39.97493394}
\toyPoint{41.03212778}{39.85332054}
\toyPoint{40.75844094}{40.20687667}
\toyPoint{40.90713097}{40.37313229}
\toyPoint{40.07306371}{39.73818655}
\toyPoint{40.85987631}{40.35560785}
\toyPoint{40.50034672}{39.93359660}
\toyPoint{40.15736564}{39.82159875}
\toyPoint{40.88492747}{40.16295501}
\toyPoint{40.60410634}{39.87630724}
\toyPoint{40.21394174}{39.85476177}
\toyPoint{40.41790730}{39.94610576}
\toyPoint{40.42520805}{39.90792706}
\toyPoint{40.62739686}{40.00735163}
\toyPoint{40.58649000}{39.88165052}
\toyPoint{40.50846079}{39.91083366}
\toyPoint{40.59943223}{39.96296078}
\toyPoint{40.78915944}{40.29957886}
\toyPoint{40.66825820}{40.27711045}
\toyPoint{40.53599073}{39.90531660}
\toyPoint{40.47288532}{39.90509908}
\toyPoint{40.51511776}{39.90174166}
\toyPoint{40.72585066}{40.04158624}
\toyPoint{40.79568274}{39.74753193}
\toyPoint{40.76328516}{40.11230438}
\toyPoint{40.05246127}{39.75189365}
\toyPoint{40.50729311}{39.89893309}
\toyPoint{40.70603423}{39.87133259}
\toyPoint{40.25970123}{39.89044409}
\toyPoint{40.71597349}{40.12652850}
\toyPoint{40.61426754}{40.15594034}
\toyPoint{40.78233682}{40.20077728}
\toyPoint{40.80131600}{40.35407255}
\toyPoint{40.35028958}{39.90748204}
\toyPoint{40.36323777}{39.92063975}
\toyPoint{40.65873977}{39.88701687}
\toyPoint{40.57601746}{39.90642458}
\toyPoint{40.52675408}{40.05129150}
\toyPoint{40.28757261}{39.89160941}
\toyPoint{40.40089183}{39.92418677}
\toyPoint{40.62897369}{40.22733928}
\toyPoint{40.15944432}{39.82142787}
\toyPoint{40.64103623}{39.86507587}
\toyPoint{40.24719873}{39.86477403}
\toyPoint{40.82146372}{39.82438885}
\toyPoint{40.36504838}{39.91149736}
\toyPoint{40.28423883}{39.87777765}
\toyPoint{40.65756507}{40.14007529}
\toyPoint{40.43486333}{39.91023305}
\toyPoint{40.53742581}{39.98594503}
\toyPoint{40.52635035}{40.10507936}
\toyPoint{40.38259498}{39.98321767}
\toyPoint{40.71748101}{40.27981295}
\toyPoint{40.72123677}{39.85273373}
\toyPoint{40.26342864}{39.86764697}
\toyPoint{40.21752888}{39.86346009}
\toyPoint{40.44989605}{39.90571038}
\toyPoint{40.24598157}{39.89332742}
\toyPoint{40.94857802}{39.71350547}
\toyPoint{40.82451163}{40.03402646}
\toyPoint{40.38483191}{39.90018991}
\toyPoint{40.88961711}{40.10595908}
\toyPoint{40.32094107}{39.90580078}
\toyPoint{40.58255412}{39.89002706}
\toyPoint{41.22800373}{40.42094434}
\toyPoint{40.37186367}{39.89570338}
\toyPoint{40.68259729}{40.23226036}
\toyPoint{40.57315687}{40.08636948}
\toyPoint{40.32090372}{39.88514375}
\toyPoint{40.82277713}{39.71860335}
\toyPoint{40.33599898}{39.89847240}
\toyPoint{40.62167779}{39.95733268}
\toyPoint{40.13877129}{39.79257797}
\toyPoint{40.56080020}{39.95873602}
\toyPoint{40.72637912}{39.91996409}
\toyPoint{40.78307333}{39.86242612}
\toyPoint{40.43313157}{39.90588506}
\toyPoint{40.49165348}{39.92899821}
\toyPoint{40.48639784}{39.90193541}
\toyPoint{40.24203749}{39.85941732}
\toyPoint{40.37936698}{39.89228786}
\toyPoint{40.57752839}{39.88597868}
\toyPoint{40.49774171}{39.90099815}
\toyPoint{40.25241288}{39.86447090}
\toyPoint{40.27606742}{39.88658254}
\toyPoint{40.41550484}{39.95843602}
\toyPoint{40.46931347}{39.96380429}
\toyPoint{40.20022437}{39.84243758}
\toyPoint{40.82769932}{39.78453704}
\toyPoint{40.39194697}{39.90740945}
\toyPoint{40.26126444}{39.86515809}
\toyPoint{40.40990547}{39.94313311}
\toyPoint{40.63346903}{39.86720289}
\toyPoint{40.49411991}{40.03531891}
\toyPoint{40.80219916}{40.21925996}
\toyPoint{40.76062689}{39.80077679}
\toyPoint{40.53134383}{39.90586701}
\toyPoint{40.30099067}{39.90253585}
\toyPoint{40.34103283}{39.94847177}
\toyPoint{40.68311172}{40.16760869}
\toyPoint{40.49290234}{40.08392122}
\toyPoint{40.52633021}{39.92726408}
\toyPoint{40.61912412}{39.87002778}
\toyPoint{40.54651441}{40.01599236}


==> figures/toy8_native_data/logistic_1000.tex <==
% Generated from original vector marker centers; do not edit by hand.
\toyPoint{50.09603239}{15.44191114}
\toyPoint{44.95193735}{14.33870069}
\toyPoint{16.46552978}{43.76639597}
\toyPoint{47.71093369}{66.01666297}
\toyPoint{45.90795355}{11.08911084}
\toyPoint{57.09468903}{56.64442862}
\toyPoint{51.98412911}{64.51436597}
\toyPoint{18.62532216}{49.19949470}
\toyPoint{55.43600636}{17.99324682}
\toyPoint{59.26468880}{55.07464378}
\toyPoint{40.94924473}{14.45297395}
\toyPoint{59.51969824}{53.60912477}
\toyPoint{34.31880251}{13.23337370}
\toyPoint{27.33267553}{19.16889652}
\toyPoint{28.68440044}{17.90552724}
\toyPoint{65.44171887}{40.45842783}
\toyPoint{32.82009755}{67.11592644}
\toyPoint{28.16724362}{18.27838928}
\toyPoint{45.47765570}{11.15596956}
\toyPoint{27.80632788}{17.75970428}
\toyPoint{58.25958221}{19.90158912}
\toyPoint{43.87869304}{14.15268190}
\toyPoint{27.17216446}{19.10247157}
\toyPoint{15.37301587}{47.74843231}
\toyPoint{26.82276972}{18.77911445}
\toyPoint{19.39121031}{61.47326008}
\toyPoint{60.10561420}{54.96997802}
\toyPoint{16.72889617}{34.99241806}
\toyPoint{64.13958580}{29.54466774}
\toyPoint{56.11773276}{17.74698350}
\toyPoint{40.01308769}{14.54323615}
\toyPoint{40.05142910}{64.19114113}
\toyPoint{28.03391534}{64.44005013}
\toyPoint{15.84415405}{53.46855933}
\toyPoint{29.07289813}{59.73704215}
\toyPoint{31.52156307}{17.09075712}
\toyPoint{62.29068971}{51.88808872}
\toyPoint{24.30688304}{66.55793467}
\toyPoint{15.49039010}{43.14497698}
\toyPoint{19.80223010}{22.35438716}
\toyPoint{45.51429910}{14.71153659}
\toyPoint{43.05232021}{12.32780457}
\toyPoint{16.96128507}{40.64578696}
\toyPoint{20.35218639}{22.49103023}
\toyPoint{48.11052707}{62.81175890}
\toyPoint{42.17805832}{14.59672497}
\toyPoint{51.50274046}{63.86550134}
\toyPoint{15.77999946}{38.33449202}
\toyPoint{39.73140681}{66.17192730}
\toyPoint{30.28839219}{15.20605518}
\toyPoint{29.41523567}{64.09808713}
\toyPoint{18.22024438}{29.99287774}
\toyPoint{20.86149154}{24.75260427}
\toyPoint{52.90160533}{17.41935176}
\toyPoint{28.40579294}{18.59650120}
\toyPoint{53.91431132}{16.47778450}
\toyPoint{20.79011979}{56.35914618}
\toyPoint{61.27606792}{53.62011356}
\toyPoint{17.64326526}{22.47329189}
\toyPoint{55.39384165}{17.72921132}
\toyPoint{48.73892461}{14.54292697}
\toyPoint{54.14554350}{17.44410269}
\toyPoint{14.83859524}{47.60598952}
\toyPoint{19.55557916}{22.81830511}
\toyPoint{65.30731693}{33.41098339}
\toyPoint{15.72599226}{38.67799599}
\toyPoint{37.55678158}{64.90454489}
\toyPoint{32.10507793}{63.39247273}
\toyPoint{34.81916774}{12.96801536}
\toyPoint{54.00554872}{17.56308279}
\toyPoint{56.06781867}{59.46143181}
\toyPoint{29.16921154}{64.66339911}
\toyPoint{57.42442654}{19.23987296}
\toyPoint{52.53299636}{16.40180126}
\toyPoint{22.70769427}{22.31881203}
\toyPoint{32.21579336}{16.41716926}
\toyPoint{28.58811702}{60.13409061}
\toyPoint{37.12055383}{67.84162952}
\toyPoint{48.67741569}{15.06293635}
\toyPoint{53.08921076}{16.20387539}
\toyPoint{20.34164367}{61.96796325}
\toyPoint{30.32327052}{17.26686539}
\toyPoint{29.17266169}{62.95245048}
\toyPoint{15.71008898}{39.81927455}
\toyPoint{53.34019476}{17.10833703}
\toyPoint{31.52041481}{14.49969476}
\toyPoint{48.94852838}{11.07974022}
\toyPoint{30.34548959}{17.09916176}
\toyPoint{58.77770732}{22.99057714}
\toyPoint{16.42820266}{38.54111575}
\toyPoint{30.11133640}{67.64638470}
\toyPoint{22.32770120}{21.38841814}
\toyPoint{22.39822080}{60.48855597}
\toyPoint{64.81010652}{13.75452595}
\toyPoint{58.49579657}{56.72740906}
\toyPoint{22.13774158}{21.87641944}
\toyPoint{19.71739154}{22.03926394}
\toyPoint{41.59255497}{14.14235146}
\toyPoint{20.79548651}{64.67036247}
\toyPoint{15.56423372}{38.05327212}
\toyPoint{34.31250903}{61.65744228}
\toyPoint{23.46869253}{21.20487275}
\toyPoint{64.34226928}{46.38905956}
\toyPoint{16.94516336}{21.53856800}
\toyPoint{32.96910840}{66.86752196}
\toyPoint{15.55198977}{43.62847313}
\toyPoint{20.37597902}{25.55776688}
\toyPoint{23.64502384}{20.98346187}
\toyPoint{33.28068841}{69.54751292}
\toyPoint{65.31847800}{41.85035140}
\toyPoint{63.83126136}{47.77254720}
\toyPoint{22.92861139}{58.93776771}
\toyPoint{19.40390648}{27.17289586}
\toyPoint{55.89268100}{59.74471154}
\toyPoint{44.74507693}{63.07707725}
\toyPoint{61.09676484}{54.25861543}
\toyPoint{21.35110794}{58.97261989}
\toyPoint{16.35363610}{36.79670353}
\toyPoint{15.77595865}{42.94598379}
\toyPoint{13.02346999}{18.38054934}
\toyPoint{16.00595720}{36.26120675}
\toyPoint{14.91357711}{42.81374474}
\toyPoint{58.87926902}{57.78258354}
\toyPoint{49.74836426}{14.76195520}
\toyPoint{38.07555983}{14.50070689}
\toyPoint{27.86239932}{18.55691141}
\toyPoint{24.30021655}{61.46754880}
\toyPoint{23.24199184}{63.14364064}
\toyPoint{32.96309179}{16.21559789}
\toyPoint{28.32456297}{65.78007021}
\toyPoint{21.31498521}{24.66969305}
\toyPoint{65.05054628}{43.59840085}
\toyPoint{21.40351695}{62.85221161}
\toyPoint{64.51389221}{31.51937731}
\toyPoint{45.25906586}{11.21660479}
\toyPoint{44.86778828}{14.06646975}
\toyPoint{25.62052481}{19.69009184}
\toyPoint{65.53693556}{40.53710827}
\toyPoint{23.84292049}{21.00954179}
\toyPoint{18.34124565}{22.36675109}
\toyPoint{31.88988670}{15.24986421}
\toyPoint{64.96654910}{33.79825707}
\toyPoint{39.61959936}{65.52180598}
\toyPoint{44.38895725}{11.87840862}
\toyPoint{22.93195386}{21.83736494}
\toyPoint{41.51873827}{62.93255252}
\toyPoint{16.07585538}{55.42885996}
\toyPoint{57.97820214}{58.32889280}
\toyPoint{40.97758616}{14.04209875}
\toyPoint{17.96427819}{55.73080094}
\toyPoint{28.26717331}{16.81246111}
\toyPoint{63.48434694}{48.74749922}
\toyPoint{25.53738440}{66.50717151}
\toyPoint{31.43081096}{16.62767133}
\toyPoint{15.19620465}{38.04543218}
\toyPoint{41.08542529}{64.45197567}
\toyPoint{50.45386561}{15.79213265}
\toyPoint{24.18136258}{20.09161180}
\toyPoint{20.04746283}{26.10340703}
\toyPoint{18.36390772}{54.86145604}
\toyPoint{25.73600554}{19.64906539}
\toyPoint{57.87357330}{56.98929417}
\toyPoint{55.88676822}{57.90804094}
\toyPoint{54.70015434}{59.72565651}
\toyPoint{24.24527876}{61.10637388}
\toyPoint{63.90566180}{48.44654037}
\toyPoint{48.28084946}{63.33195440}
\toyPoint{33.30305361}{67.87027667}
\toyPoint{23.54430814}{21.40694864}
\toyPoint{41.88388709}{64.66724150}
\toyPoint{24.16913248}{20.64693174}
\toyPoint{21.99961570}{23.09663803}
\toyPoint{16.17267178}{37.70807316}
\toyPoint{22.75023122}{22.15298345}
\toyPoint{18.05863350}{30.28829452}
\toyPoint{29.55035287}{17.58888275}
\toyPoint{17.08355381}{50.08148270}
\toyPoint{38.14631843}{66.71171927}
\toyPoint{15.77015046}{45.47545956}
\toyPoint{64.02762598}{30.40910044}
\toyPoint{40.79369627}{14.01019066}
\toyPoint{65.51506412}{41.03256097}
\toyPoint{65.71069656}{37.36438567}
\toyPoint{35.46491831}{12.72782787}
\toyPoint{50.02115357}{60.10559267}
\toyPoint{62.22290962}{53.74954254}
\toyPoint{41.96761354}{66.11088291}
\toyPoint{43.63288579}{67.34117816}
\toyPoint{23.71864750}{20.83029101}
\toyPoint{16.60888703}{34.74842702}
\toyPoint{35.54422594}{12.71512862}
\toyPoint{52.51013433}{59.60146350}
\toyPoint{23.61577988}{21.25460071}
\toyPoint{58.57335029}{21.57577053}
\toyPoint{18.66361064}{22.87341364}
\toyPoint{26.27462541}{61.43310885}
\toyPoint{16.64574039}{51.63043207}
\toyPoint{50.86701501}{15.55643358}
\toyPoint{24.91910350}{20.20017993}
\toyPoint{15.86059724}{46.92232886}
\toyPoint{55.34096195}{59.13802085}
\toyPoint{56.57768988}{19.28236069}
\toyPoint{21.28782549}{24.11808475}
\toyPoint{51.94695580}{62.43277642}
\toyPoint{53.79427141}{16.97127096}
\toyPoint{32.82364691}{16.28979375}
\toyPoint{54.52260171}{56.78285599}
\toyPoint{61.24475971}{24.63455016}
\toyPoint{30.44499859}{17.22848615}
\toyPoint{63.32665228}{28.63485552}
\toyPoint{33.62117667}{13.46199712}
\toyPoint{50.24778197}{62.71614075}
\toyPoint{61.69959776}{52.60525719}
\toyPoint{64.51486280}{45.85947960}
\toyPoint{23.94292708}{20.95199370}
\toyPoint{48.50272871}{14.88868160}
\toyPoint{57.51476411}{57.15297545}
\toyPoint{27.41714031}{68.82273582}
\toyPoint{18.35174222}{55.25990578}
\toyPoint{64.85916076}{33.27931558}
\toyPoint{64.83769232}{33.06512725}
\toyPoint{24.59861663}{61.82521512}
\toyPoint{58.79413820}{20.86921169}
\toyPoint{51.49980099}{61.23912534}
\toyPoint{35.24269181}{15.44993893}
\toyPoint{36.77301030}{68.54221098}
\toyPoint{42.10104527}{14.51003751}
\toyPoint{52.53203884}{59.35219765}
\toyPoint{25.78250639}{69.79332093}
\toyPoint{20.86099778}{24.74848655}
\toyPoint{42.09026760}{14.19374681}
\toyPoint{30.34790762}{62.86301736}
\toyPoint{26.95168495}{18.78953565}
\toyPoint{16.89534464}{55.66394683}
\toyPoint{53.39720911}{60.11721673}
\toyPoint{37.94389471}{12.05994514}
\toyPoint{32.32789547}{70.33740751}
\toyPoint{16.24460959}{50.60608895}
\toyPoint{61.75509853}{51.78739917}
\toyPoint{40.05123274}{11.62660168}
\toyPoint{54.66848004}{60.59258338}
\toyPoint{17.81251631}{43.68790703}
\toyPoint{50.13471465}{15.59197334}
\toyPoint{58.93106276}{20.22624754}
\toyPoint{57.78928695}{20.09376372}
\toyPoint{29.38257848}{17.98015071}
\toyPoint{48.92689766}{11.18644407}
\toyPoint{62.18613471}{51.74573437}
\toyPoint{60.26764039}{23.36508659}
\toyPoint{15.94727855}{44.94063439}
\toyPoint{32.30912039}{16.31306494}
\toyPoint{48.94284633}{14.76077695}
\toyPoint{33.22645049}{13.68520921}
\toyPoint{17.40194259}{52.51750454}
\toyPoint{17.73246458}{61.15715857}
\toyPoint{25.44542405}{19.71190791}
\toyPoint{39.11441841}{62.63254658}
\toyPoint{32.72065009}{16.32466285}
\toyPoint{42.63629536}{12.46707793}
\toyPoint{64.87474257}{44.17286042}
\toyPoint{21.29915268}{24.06684783}
\toyPoint{65.45219083}{34.04661540}
\toyPoint{55.65180132}{18.62744639}
\toyPoint{34.64176932}{65.11805411}
\toyPoint{31.58229982}{68.91775254}
\toyPoint{24.36046108}{20.85536495}
\toyPoint{58.03402747}{56.24664491}
\toyPoint{14.06573757}{51.05185939}
\toyPoint{18.69427896}{52.93462015}
\toyPoint{46.68757808}{64.35523925}
\toyPoint{16.91059420}{46.20743959}
\toyPoint{30.72588874}{14.93625302}
\toyPoint{23.25193159}{20.97750602}
\toyPoint{52.49421258}{16.75929377}
\toyPoint{60.84185385}{23.93981687}
\toyPoint{64.85784254}{45.50267081}
\toyPoint{17.16931374}{22.30450538}
\toyPoint{29.42175604}{18.31356448}
\toyPoint{63.45512913}{28.03651564}
\toyPoint{39.15177745}{67.47051485}
\toyPoint{34.20031463}{16.02635814}
\toyPoint{43.64805768}{14.04486133}
\toyPoint{51.02196709}{15.85113587}
\toyPoint{65.01001050}{43.86532853}
\toyPoint{56.81005878}{19.50390846}
\toyPoint{31.97304787}{16.06735999}
\toyPoint{26.72498580}{60.98721996}
\toyPoint{18.78848045}{53.02991375}
\toyPoint{65.16771286}{42.99424606}
\toyPoint{18.56179360}{54.63858235}
\toyPoint{65.14048699}{34.80789015}
\toyPoint{23.84927319}{21.00403509}
\toyPoint{45.41501699}{14.33335550}
\toyPoint{17.84776072}{30.42007692}
\toyPoint{62.31999982}{26.60994037}
\toyPoint{61.64539829}{25.20537499}
\toyPoint{54.69949753}{14.31471578}
\toyPoint{38.69380343}{66.07675983}
\toyPoint{35.53372783}{12.85150712}
\toyPoint{29.18514021}{17.73684071}
\toyPoint{63.23111565}{28.37155296}
\toyPoint{33.22995294}{66.49105133}
\toyPoint{65.75144152}{34.59452129}
\toyPoint{61.51410349}{51.96315442}
\toyPoint{46.12950979}{13.65464241}
\toyPoint{58.85890038}{20.30447652}
\toyPoint{65.75692208}{36.96938126}
\toyPoint{22.68342172}{21.36149837}
\toyPoint{35.44728225}{15.39698847}
\toyPoint{59.58612627}{55.10951904}
\toyPoint{25.79906341}{18.68564975}
\toyPoint{25.40761086}{19.45642779}
\toyPoint{46.02641990}{61.99326331}
\toyPoint{35.99512508}{65.48175781}
\toyPoint{32.63633682}{13.92903297}
\toyPoint{59.39624048}{52.53264873}
\toyPoint{30.05157178}{65.47729092}
\toyPoint{30.44535160}{15.21898823}
\toyPoint{22.94115989}{21.81778385}
\toyPoint{40.04794968}{12.01798962}
\toyPoint{39.82729617}{14.24113212}
\toyPoint{36.83912377}{12.73209479}
\toyPoint{64.48019981}{46.07532378}
\toyPoint{22.94400246}{20.79170258}
\toyPoint{28.64969515}{16.29478516}
\toyPoint{47.15894315}{14.85817786}
\toyPoint{43.73942814}{13.93327836}
\toyPoint{64.54205790}{45.73709549}
\toyPoint{17.65808875}{22.65522834}
\toyPoint{22.81870811}{61.12562118}
\toyPoint{54.62926249}{17.97146766}
\toyPoint{63.07013235}{27.90903091}
\toyPoint{37.92092654}{66.40306104}
\toyPoint{30.04813471}{15.59169646}
\toyPoint{23.69070484}{21.59200453}
\toyPoint{63.75030979}{29.58544423}
\toyPoint{28.95164536}{18.07769775}
\toyPoint{56.49506015}{19.26991217}
\toyPoint{15.35401160}{43.35233519}
\toyPoint{63.33261428}{28.76765005}
\toyPoint{18.35573996}{29.59875414}
\toyPoint{25.16875698}{19.52825638}
\toyPoint{45.78829281}{14.51136651}
\toyPoint{27.94717481}{18.87415886}
\toyPoint{60.80710011}{22.95877518}
\toyPoint{17.18630760}{33.03447662}
\toyPoint{16.50536260}{38.21460112}
\toyPoint{23.87485627}{20.66940923}
\toyPoint{34.01722608}{13.89427923}
\toyPoint{57.08912234}{19.40745661}
\toyPoint{63.41680988}{28.11467540}
\toyPoint{53.08131833}{62.33401729}
\toyPoint{25.66623965}{19.92681688}
\toyPoint{25.20152184}{60.76303574}
\toyPoint{54.88932025}{17.53866411}
\toyPoint{63.87711463}{29.46950974}
\toyPoint{19.54310140}{28.02521536}
\toyPoint{20.26101820}{21.92381859}
\toyPoint{65.30592334}{35.75116711}
\toyPoint{36.55559255}{14.88527452}
\toyPoint{17.22031070}{59.85032943}
\toyPoint{58.71963470}{21.01290733}
\toyPoint{38.26147749}{14.51939583}
\toyPoint{16.44516422}{36.95635938}
\toyPoint{20.00942199}{22.45699021}
\toyPoint{40.86836161}{65.43703971}
\toyPoint{18.98540497}{52.03099989}
\toyPoint{53.26270103}{59.80343019}
\toyPoint{25.53147624}{19.27020134}
\toyPoint{43.17165698}{67.42033312}
\toyPoint{28.39752597}{18.13294011}
\toyPoint{54.07379181}{16.77682292}
\toyPoint{50.42892471}{15.62200023}
\toyPoint{64.74329087}{30.43166330}
\toyPoint{14.57935887}{38.99351760}
\toyPoint{18.13699169}{29.90402452}
\toyPoint{20.55566972}{22.21036696}
\toyPoint{26.28525580}{18.24072838}
\toyPoint{59.39804016}{21.58039739}
\toyPoint{35.11610500}{15.64361326}
\toyPoint{55.36326101}{12.53940951}
\toyPoint{25.71693513}{19.65430906}
\toyPoint{21.21553852}{24.52578360}
\toyPoint{18.40674000}{52.65185187}
\toyPoint{32.55859313}{16.28935998}
\toyPoint{64.97966059}{33.84080671}
\toyPoint{50.70736070}{15.52146912}
\toyPoint{35.06700347}{66.59010118}
\toyPoint{55.55303758}{17.34246254}
\toyPoint{47.28271008}{64.29845564}
\toyPoint{21.89421623}{62.86963770}
\toyPoint{24.24779523}{20.93258488}
\toyPoint{24.40780947}{20.43390397}
\toyPoint{65.37812879}{41.17793275}
\toyPoint{34.48486490}{15.74241853}
\toyPoint{25.29199170}{19.71988339}
\toyPoint{16.52364085}{22.19482206}
\toyPoint{42.31995890}{14.39309551}
\toyPoint{49.24828360}{15.27840676}
\toyPoint{30.78410979}{16.98559915}
\toyPoint{53.43189516}{16.62864039}
\toyPoint{61.59261396}{52.23234746}
\toyPoint{57.36858737}{57.52528683}
\toyPoint{25.42437861}{19.59659484}
\toyPoint{21.12319823}{65.22806506}
\toyPoint{53.28199756}{16.84820083}
\toyPoint{21.14020286}{21.79420194}
\toyPoint{65.05596069}{43.62167743}
\toyPoint{64.57571030}{32.16946171}
\toyPoint{30.99613082}{63.38972092}
\toyPoint{26.05547720}{18.42701174}
\toyPoint{49.12442515}{65.70629427}
\toyPoint{27.61010862}{18.83277247}
\toyPoint{60.18917145}{22.42015069}
\toyPoint{63.53611608}{48.42170561}
\toyPoint{17.90291694}{31.18497372}
\toyPoint{22.38145459}{56.75084637}
\toyPoint{64.27366011}{46.85948095}
\toyPoint{49.91848284}{15.64432698}
\toyPoint{30.70006878}{64.31659545}


==> figures/toy8_native_data/logistic_10000.tex <==
% Generated from original vector marker centers; do not edit by hand.
\toyPoint{20.83554545}{20.09346685}
\toyPoint{20.52932216}{19.58629516}
\toyPoint{60.02921104}{21.90702161}
\toyPoint{34.82273786}{63.22298942}
\toyPoint{59.28436833}{25.21063405}
\toyPoint{10.61616528}{37.73747479}
\toyPoint{62.11566125}{52.10702389}
\toyPoint{60.20157691}{21.50732133}
\toyPoint{21.63324325}{21.15765049}
\toyPoint{36.75452325}{62.52065597}
\toyPoint{20.20724481}{19.03071065}
\toyPoint{10.25040657}{30.23545711}
\toyPoint{59.00362815}{24.34787566}
\toyPoint{19.66362430}{18.15474541}
\toyPoint{20.45800424}{19.37852952}
\toyPoint{18.14424422}{22.11996632}
\toyPoint{60.16721233}{19.91460831}
\toyPoint{20.39465873}{19.15735245}
\toyPoint{59.24104075}{25.20034975}
\toyPoint{58.97163699}{23.87095236}
\toyPoint{22.44209905}{22.71993975}
\toyPoint{20.61153966}{19.72104780}
\toyPoint{19.94973429}{18.51863677}
\toyPoint{59.42302489}{22.77303634}
\toyPoint{20.45263598}{19.43938624}
\toyPoint{57.90330641}{24.00868293}
\toyPoint{63.49933194}{31.44604668}
\toyPoint{59.66853142}{22.39469067}
\toyPoint{20.54197065}{24.05225354}
\toyPoint{22.51173573}{23.87891246}
\toyPoint{20.19184297}{18.98844134}
\toyPoint{63.33813790}{20.89619144}
\toyPoint{60.23703667}{24.57519008}
\toyPoint{58.97375199}{23.18308246}
\toyPoint{59.64883189}{21.63504293}
\toyPoint{20.39161928}{20.31970455}
\toyPoint{35.72868501}{15.57344437}
\toyPoint{60.01401532}{25.09136169}
\toyPoint{59.61468727}{22.52206003}
\toyPoint{19.93141297}{18.86092586}
\toyPoint{20.06363838}{18.92755693}
\toyPoint{59.03962166}{25.31835771}
\toyPoint{59.95678409}{21.77177983}
\toyPoint{19.46964695}{18.23092245}
\toyPoint{20.99906368}{21.31923522}
\toyPoint{19.90950154}{18.62762943}
\toyPoint{53.25398261}{61.13309368}
\toyPoint{59.46704618}{22.64556393}
\toyPoint{37.33984336}{16.38230016}
\toyPoint{58.94297907}{24.04151547}
\toyPoint{60.20794807}{24.31265123}
\toyPoint{59.45617737}{22.70299050}
\toyPoint{58.96778537}{23.36259473}
\toyPoint{20.12070041}{19.09519749}
\toyPoint{19.72267520}{18.21724184}
\toyPoint{22.21096531}{22.32193455}
\toyPoint{59.63955356}{22.30390703}
\toyPoint{46.22683071}{17.59109620}
\toyPoint{19.45141177}{18.50179980}
\toyPoint{21.90892281}{21.60349015}
\toyPoint{21.24848950}{20.92414179}
\toyPoint{21.09541093}{20.44096116}
\toyPoint{59.19253565}{22.97143905}
\toyPoint{18.65489990}{17.36245894}
\toyPoint{19.12459835}{21.79689377}
\toyPoint{59.47204067}{22.64151696}
\toyPoint{63.14795217}{21.20422517}
\toyPoint{59.81761379}{23.60588474}
\toyPoint{58.90368308}{24.45603155}
\toyPoint{20.72369483}{19.97671866}
\toyPoint{61.39957643}{54.77922932}
\toyPoint{60.92317766}{24.53135798}
\toyPoint{22.28427825}{22.21844704}
\toyPoint{21.12215227}{20.49579128}
\toyPoint{59.33689733}{23.06321021}
\toyPoint{20.40904383}{19.21479441}
\toyPoint{59.49163868}{21.85519557}
\toyPoint{34.36291918}{17.97780960}
\toyPoint{20.65892804}{19.82591660}
\toyPoint{21.77022626}{21.53465025}
\toyPoint{57.91944196}{24.09651172}
\toyPoint{20.37311185}{19.12143123}
\toyPoint{59.09168613}{23.57573478}
\toyPoint{59.59438939}{22.51229871}
\toyPoint{20.79766458}{20.05978830}
\toyPoint{59.01238657}{24.08833165}
\toyPoint{59.67918334}{25.25646425}
\toyPoint{20.44698161}{19.51027347}
\toyPoint{20.61164733}{19.69680909}
\toyPoint{59.88573690}{22.06296582}
\toyPoint{62.53797593}{22.00476708}
\toyPoint{20.17129437}{18.96951706}
\toyPoint{58.48902856}{23.42530651}
\toyPoint{63.20345756}{24.27228005}
\toyPoint{64.61189147}{49.34998143}
\toyPoint{19.37826187}{17.99905039}
\toyPoint{20.13835107}{19.21309625}
\toyPoint{20.56179785}{19.62135500}
\toyPoint{57.78483545}{24.63993688}
\toyPoint{59.21477472}{22.89240560}
\toyPoint{59.19107745}{22.14526023}
\toyPoint{58.94911643}{23.54260998}
\toyPoint{65.29529910}{39.78788497}
\toyPoint{19.48941415}{18.78549484}
\toyPoint{60.88255728}{20.29235409}
\toyPoint{59.65334800}{22.48311012}
\toyPoint{59.30741495}{22.97887464}
\toyPoint{58.98767102}{23.51457657}
\toyPoint{45.06240552}{17.15758354}
\toyPoint{19.50092131}{20.35478900}
\toyPoint{65.26374940}{37.78851713}
\toyPoint{59.18328347}{22.60538963}
\toyPoint{58.83961155}{23.40794040}
\toyPoint{62.47110797}{53.46477232}
\toyPoint{57.86091712}{17.05450981}
\toyPoint{40.00486186}{15.90408479}
\toyPoint{58.82296531}{23.07720154}
\toyPoint{59.70247299}{22.35467634}
\toyPoint{59.77388320}{22.32309895}
\toyPoint{16.22228130}{14.65985821}
\toyPoint{59.24252049}{22.87089102}
\toyPoint{59.24369258}{22.88345029}
\toyPoint{50.11219640}{19.28927022}
\toyPoint{21.48708190}{21.31596658}
\toyPoint{20.55486679}{19.67751103}
\toyPoint{20.25447938}{18.92154571}
\toyPoint{58.50455192}{23.49107619}
\toyPoint{58.30628918}{24.35159499}
\toyPoint{20.30579167}{19.03095984}
\toyPoint{61.95991854}{24.60519545}
\toyPoint{59.37168490}{22.87649155}
\toyPoint{24.71960252}{17.63517134}
\toyPoint{57.96841468}{24.29667104}
\toyPoint{21.50185770}{23.38219735}
\toyPoint{59.22714479}{25.19732260}
\toyPoint{20.78147058}{20.08469920}
\toyPoint{20.28516308}{18.99729513}
\toyPoint{27.34601467}{17.25889760}
\toyPoint{19.56645104}{18.13409990}
\toyPoint{19.79694182}{18.88642588}
\toyPoint{58.86604678}{24.36949330}
\toyPoint{21.85222533}{22.18538377}
\toyPoint{49.51788041}{15.92208616}
\toyPoint{59.15913243}{25.29444664}
\toyPoint{59.03713288}{23.41807704}
\toyPoint{63.59444710}{22.78742759}
\toyPoint{58.72005770}{23.36281007}
\toyPoint{62.10113464}{29.52200259}
\toyPoint{20.65456421}{19.91929516}
\toyPoint{59.06081784}{23.05407493}
\toyPoint{59.11085344}{23.75765431}
\toyPoint{51.35575541}{20.19737736}
\toyPoint{60.86533423}{24.99648340}
\toyPoint{20.45087014}{19.54987711}
\toyPoint{58.84282943}{23.20592142}
\toyPoint{58.30600615}{17.79575163}
\toyPoint{20.52993282}{19.67494226}
\toyPoint{20.44256087}{19.43719126}
\toyPoint{59.16245799}{23.11717587}
\toyPoint{59.38622690}{22.73589842}
\toyPoint{20.26265944}{18.96084632}
\toyPoint{50.00522875}{61.57961938}
\toyPoint{11.53260631}{40.94508000}
\toyPoint{30.95782234}{61.62366375}
\toyPoint{58.58494051}{23.31221150}
\toyPoint{19.84305197}{19.27926125}
\toyPoint{13.50766582}{36.19168312}
\toyPoint{54.89347027}{17.91749585}
\toyPoint{18.86053824}{17.26967873}
\toyPoint{49.35470058}{15.50294169}
\toyPoint{59.24815332}{23.26822712}
\toyPoint{58.90064055}{23.49967157}
\toyPoint{59.69895670}{22.36577742}
\toyPoint{59.33742954}{23.07704618}
\toyPoint{59.37517197}{22.79183603}
\toyPoint{20.40861776}{19.19114482}
\toyPoint{59.87466197}{22.24916920}
\toyPoint{40.63249666}{16.23472521}
\toyPoint{59.73023261}{22.41310427}
\toyPoint{21.83414705}{21.57392317}
\toyPoint{20.71884647}{20.29166652}
\toyPoint{33.95517649}{16.52358547}
\toyPoint{26.29155005}{17.81169953}
\toyPoint{58.83531386}{24.59766296}
\toyPoint{60.72896957}{17.57634501}
\toyPoint{18.58206072}{19.88448912}
\toyPoint{21.49973808}{23.89908575}
\toyPoint{17.77942842}{49.95982693}
\toyPoint{20.05314489}{18.73698050}
\toyPoint{59.48541210}{22.62518914}
\toyPoint{58.94589701}{24.48483252}
\toyPoint{31.83953424}{14.37010273}
\toyPoint{19.20846631}{17.70897650}
\toyPoint{20.55742787}{19.82817311}
\toyPoint{18.81928105}{17.62485627}
\toyPoint{58.76596635}{23.03602434}
\toyPoint{59.49372599}{22.70965084}
\toyPoint{21.08488821}{20.47757610}
\toyPoint{20.08426082}{18.73548231}
\toyPoint{59.69793227}{22.46898959}
\toyPoint{30.87257154}{61.54809429}
\toyPoint{21.21785041}{20.58654108}
\toyPoint{58.59269450}{23.77824753}
\toyPoint{38.54715236}{63.67221925}
\toyPoint{21.38387126}{20.85022280}
\toyPoint{20.27775518}{18.98454051}
\toyPoint{59.56265972}{16.51139998}
\toyPoint{21.70630855}{21.19085989}
\toyPoint{20.35462441}{19.08775883}
\toyPoint{21.44822582}{20.95646827}
\toyPoint{58.87350390}{24.38207411}
\toyPoint{18.13044210}{52.13748147}
\toyPoint{51.96809507}{20.27659539}
\toyPoint{57.52249195}{24.72437090}
\toyPoint{19.58491541}{18.15213819}
\toyPoint{20.80033333}{20.04396192}
\toyPoint{39.09776353}{62.98166521}
\toyPoint{62.87575045}{23.35824782}
\toyPoint{59.28038597}{22.83679716}
\toyPoint{21.85538323}{21.97317739}
\toyPoint{21.50981626}{23.20377873}
\toyPoint{58.48411868}{23.62327699}
\toyPoint{22.17170008}{21.90493584}
\toyPoint{12.49262102}{35.30730324}
\toyPoint{20.29368154}{19.04613556}
\toyPoint{30.66863906}{19.75265749}
\toyPoint{20.03694165}{18.81507258}
\toyPoint{39.25751287}{13.24864172}
\toyPoint{62.39906249}{24.08263114}
\toyPoint{59.13627501}{23.19000275}
\toyPoint{20.50231318}{19.50712635}
\toyPoint{59.15712510}{23.34652532}
\toyPoint{20.45300207}{19.32893538}
\toyPoint{58.84066982}{23.26965147}
\toyPoint{13.26189779}{44.36709043}
\toyPoint{58.99753540}{24.67175576}
\toyPoint{46.39266506}{17.48925301}
\toyPoint{59.49623785}{22.71359167}
\toyPoint{55.96810433}{57.71611091}
\toyPoint{59.02818064}{24.84210199}
\toyPoint{54.35847436}{60.43325363}
\toyPoint{59.94960846}{21.58613636}
\toyPoint{20.65155091}{19.83220008}
\toyPoint{22.07457142}{24.17774170}
\toyPoint{21.76634081}{21.27162072}
\toyPoint{19.97598956}{18.53953761}
\toyPoint{59.56959386}{25.31192964}
\toyPoint{47.37516649}{18.13686094}
\toyPoint{21.15545857}{20.54621297}
\toyPoint{59.83217732}{22.27148210}
\toyPoint{20.45929786}{19.37150002}
\toyPoint{21.07388712}{20.53948802}
\toyPoint{58.72359860}{24.57866176}
\toyPoint{59.60016989}{22.57102043}
\toyPoint{57.80922490}{23.95932105}
\toyPoint{59.09041251}{23.52895860}
\toyPoint{60.91438847}{23.05501169}
\toyPoint{20.28439245}{18.99357734}
\toyPoint{59.00147930}{25.32309994}
\toyPoint{35.83788649}{60.98525109}
\toyPoint{59.18038707}{23.16944491}
\toyPoint{20.93087904}{20.28951460}
\toyPoint{20.97809515}{20.29935591}
\toyPoint{63.59398565}{22.95423292}
\toyPoint{56.12208582}{18.51978733}
\toyPoint{19.30197254}{17.78748851}
\toyPoint{23.54972101}{57.88614488}
\toyPoint{58.66302490}{23.34510096}
\toyPoint{59.92759705}{22.11607472}
\toyPoint{13.94779267}{37.84725943}
\toyPoint{60.09508225}{21.82706525}
\toyPoint{58.99646021}{24.03142960}
\toyPoint{20.16648139}{18.90951095}
\toyPoint{20.52637346}{19.70683498}
\toyPoint{21.83397170}{21.34775777}
\toyPoint{17.72720091}{22.75758989}
\toyPoint{19.33209173}{18.41640288}
\toyPoint{19.36703005}{17.72202338}
\toyPoint{21.75788079}{23.50537208}
\toyPoint{25.08159576}{22.14011961}
\toyPoint{19.90620982}{18.48336312}
\toyPoint{21.31882298}{21.67487114}
\toyPoint{20.83008643}{20.08613279}
\toyPoint{18.80556968}{20.67625415}
\toyPoint{21.19783248}{20.56308070}
\toyPoint{58.61013136}{24.66014247}
\toyPoint{58.96913282}{22.65681728}
\toyPoint{59.93568482}{22.10008990}
\toyPoint{25.59638300}{17.44027107}
\toyPoint{59.50257978}{22.60844754}
\toyPoint{21.44136398}{23.05940936}
\toyPoint{59.26496106}{23.22427196}
\toyPoint{20.61126893}{19.72505785}
\toyPoint{58.98985217}{23.17946465}
\toyPoint{21.18374425}{20.61338855}
\toyPoint{21.90549266}{21.46812993}
\toyPoint{60.12167746}{25.72788239}
\toyPoint{46.39885587}{15.86064646}
\toyPoint{59.01022388}{24.46705111}
\toyPoint{20.30617160}{19.78745891}
\toyPoint{21.85392810}{21.49458055}
\toyPoint{61.85394533}{20.89302432}
\toyPoint{54.54388095}{23.47105057}
\toyPoint{40.55119092}{62.29729314}
\toyPoint{58.99116578}{25.80842787}
\toyPoint{22.39911141}{23.51999406}
\toyPoint{31.78210920}{16.97767596}
\toyPoint{19.99368791}{18.71002074}
\toyPoint{20.28358952}{19.03383163}
\toyPoint{60.28401898}{55.06571154}
\toyPoint{59.00494791}{23.64342413}
\toyPoint{20.44401138}{19.46510930}
\toyPoint{63.28243717}{19.78286436}
\toyPoint{62.46037145}{20.87857769}
\toyPoint{58.99420523}{24.19798882}
\toyPoint{35.53113407}{12.30582391}
\toyPoint{62.45159611}{24.30041959}
\toyPoint{58.65993007}{24.39641922}
\toyPoint{59.30298959}{23.13727994}
\toyPoint{59.03707904}{24.92483477}
\toyPoint{20.75512301}{20.64074363}
\toyPoint{58.99260859}{24.65955488}
\toyPoint{23.94393459}{17.62548385}
\toyPoint{20.40385708}{19.34847032}
\toyPoint{59.00356354}{23.85697642}
\toyPoint{20.32866755}{19.33831984}
\toyPoint{20.78448080}{20.16667828}
\toyPoint{39.25395284}{16.47331453}
\toyPoint{19.14199521}{18.09710195}
\toyPoint{58.37853770}{23.61119763}
\toyPoint{20.74958555}{20.01659455}
\toyPoint{22.07057214}{21.86697037}
\toyPoint{46.44623426}{16.01061483}
\toyPoint{59.06780120}{23.95368207}
\toyPoint{59.18106694}{23.27335235}
\toyPoint{22.05690845}{22.00008946}
\toyPoint{20.16115773}{18.78581478}
\toyPoint{21.10374020}{20.45194072}
\toyPoint{59.53615527}{22.61073328}
\toyPoint{21.19445462}{20.64638261}
\toyPoint{59.39069686}{22.78595401}
\toyPoint{20.42189383}{19.50567430}
\toyPoint{20.45926248}{19.49367646}
\toyPoint{19.63041952}{18.10318855}
\toyPoint{22.33447382}{23.21147427}
\toyPoint{59.56868941}{22.53227818}
\toyPoint{59.88639678}{22.04773780}
\toyPoint{59.24354645}{23.26775951}
\toyPoint{58.95121297}{24.45968013}
\toyPoint{21.72732476}{21.23515806}
\toyPoint{21.98238803}{23.21894677}
\toyPoint{55.38500940}{60.01422913}
\toyPoint{19.87822410}{18.45524973}
\toyPoint{58.84142199}{22.89104277}
\toyPoint{21.65383954}{21.21463714}
\toyPoint{21.92722259}{23.12845999}
\toyPoint{59.50292280}{22.57491204}
\toyPoint{20.19999227}{19.23301266}
\toyPoint{21.66596197}{22.47971073}
\toyPoint{20.50774605}{19.52421865}
\toyPoint{58.03441201}{23.79871615}
\toyPoint{21.92354787}{21.47918024}
\toyPoint{20.52084215}{19.53881295}
\toyPoint{59.77755946}{22.24143674}
\toyPoint{19.73707876}{18.58328358}
\toyPoint{41.69087052}{15.51581168}
\toyPoint{60.12803785}{21.79382970}
\toyPoint{12.79880585}{30.12324041}
\toyPoint{59.17864584}{23.45499808}
\toyPoint{16.70301776}{47.40548795}
\toyPoint{20.41961116}{19.21392072}
\toyPoint{21.86262961}{21.61918886}
\toyPoint{20.78385015}{20.01856650}
\toyPoint{19.42467043}{21.89856006}
\toyPoint{58.34454075}{23.58380718}
\toyPoint{59.15697282}{23.02739359}
\toyPoint{19.92318215}{18.77103744}
\toyPoint{58.97810659}{23.70462695}
\toyPoint{22.20967477}{21.96916580}
\toyPoint{20.05561982}{18.70125002}
\toyPoint{60.26820029}{25.49091893}
\toyPoint{20.26832611}{18.96971241}
\toyPoint{59.41975317}{22.85281274}
\toyPoint{59.89801007}{22.17036340}
\toyPoint{20.40120832}{19.20094459}
\toyPoint{21.52056817}{21.20588333}
\toyPoint{21.04321572}{20.41286007}
\toyPoint{57.50165109}{18.44235820}
\toyPoint{22.49690610}{24.16719744}
\toyPoint{14.65113055}{44.08072318}
\toyPoint{58.04990615}{24.29918597}
\toyPoint{19.24675019}{17.72364924}
\toyPoint{20.12902967}{18.81061493}
\toyPoint{17.98021224}{22.60526350}
\toyPoint{20.21461887}{18.91412704}
\toyPoint{20.40849624}{19.22477107}
\toyPoint{18.74082442}{17.72376153}
\toyPoint{20.22549691}{19.08694052}
\toyPoint{20.62400818}{19.78280898}
\toyPoint{20.43807706}{19.27977808}
\toyPoint{21.49821066}{21.04483543}
\toyPoint{64.76710966}{47.49866655}
\toyPoint{48.59800769}{62.09179478}
\toyPoint{20.43767252}{19.29787482}
\toyPoint{57.90039309}{24.76113658}
\toyPoint{21.13098452}{20.49654499}
\toyPoint{20.19149842}{19.09825848}
\toyPoint{29.50320136}{16.59005196}
\toyPoint{21.88419034}{21.85743209}
\toyPoint{59.63653872}{23.70052153}
\toyPoint{59.16978744}{23.50444917}
\toyPoint{45.80183575}{63.41614693}
\toyPoint{20.02780637}{18.61419186}
\toyPoint{22.36580972}{22.41508084}
\toyPoint{63.48246728}{48.86127718}
\toyPoint{59.62621289}{22.45828998}
\toyPoint{59.87517726}{21.91479714}
\toyPoint{23.33747925}{17.75615723}
\toyPoint{20.40963296}{19.50569891}
\toyPoint{60.89840674}{24.28047242}


==> figures/toy8_native_data/logistic_20000.tex <==
% Generated from original vector marker centers; do not edit by hand.
\toyPoint{23.05315356}{23.57676383}
\toyPoint{23.06355323}{23.82005230}
\toyPoint{57.99726486}{19.98351743}
\toyPoint{22.71030611}{26.98155649}
\toyPoint{56.08256371}{16.71361892}
\toyPoint{23.32487229}{19.17090385}
\toyPoint{26.70565082}{52.49371344}
\toyPoint{58.43992972}{20.09988877}
\toyPoint{23.23006476}{23.43968545}
\toyPoint{21.29378596}{55.01121675}
\toyPoint{23.03058224}{24.15323073}
\toyPoint{25.01983304}{16.96470907}
\toyPoint{55.61583242}{18.12402479}
\toyPoint{22.97114218}{25.15940328}
\toyPoint{23.11895094}{24.52006309}
\toyPoint{17.96576561}{24.28556842}
\toyPoint{56.55129156}{25.18965936}
\toyPoint{23.14863636}{24.76978733}
\toyPoint{55.96683687}{16.91014813}
\toyPoint{55.28671172}{18.87169930}
\toyPoint{23.70067227}{23.69497330}
\toyPoint{23.13735839}{23.78675522}
\toyPoint{23.06880766}{25.12402196}
\toyPoint{57.67054219}{20.62194855}
\toyPoint{23.07029970}{24.59673851}
\toyPoint{57.85423833}{22.02858125}
\toyPoint{62.53577325}{47.41015634}
\toyPoint{57.18831062}{19.63758592}
\toyPoint{22.37796753}{24.58068602}
\toyPoint{24.31526769}{24.11271803}
\toyPoint{23.03770404}{24.20099751}
\toyPoint{57.93500223}{24.40751722}
\toyPoint{58.13828868}{23.08835491}
\toyPoint{57.63987387}{21.13190589}
\toyPoint{59.91782496}{20.85524497}
\toyPoint{23.86067267}{24.17683571}
\toyPoint{49.73239022}{19.63719522}
\toyPoint{57.27176943}{23.18052599}
\toyPoint{57.60103010}{20.22889322}
\toyPoint{22.50378947}{25.60319716}
\toyPoint{22.98295236}{24.08758871}
\toyPoint{55.32526478}{17.67418892}
\toyPoint{57.48722292}{19.74947652}
\toyPoint{22.40729301}{25.65499244}
\toyPoint{60.48997725}{18.27519909}
\toyPoint{23.00899075}{24.27923725}
\toyPoint{21.13073534}{48.15077443}
\toyPoint{57.17467462}{19.94636720}
\toyPoint{61.12809766}{25.11745699}
\toyPoint{55.75799450}{18.29522471}
\toyPoint{58.39754966}{22.94140447}
\toyPoint{56.76670351}{19.38632657}
\toyPoint{56.14675214}{19.05557386}
\toyPoint{23.17220134}{24.12295311}
\toyPoint{22.99820346}{25.07056698}
\toyPoint{23.94860606}{23.75220760}
\toyPoint{59.26808819}{20.92970079}
\toyPoint{60.06707345}{28.13773278}
\toyPoint{21.55351147}{25.54847317}
\toyPoint{23.45725152}{23.51162941}
\toyPoint{23.59920440}{23.60778593}
\toyPoint{22.98651172}{23.46470864}
\toyPoint{57.29873380}{20.66208593}
\toyPoint{21.73329753}{25.56918483}
\toyPoint{18.31203399}{24.77524788}
\toyPoint{57.19631072}{19.96876932}
\toyPoint{57.51765897}{24.55501064}
\toyPoint{59.01060843}{22.45149120}
\toyPoint{55.69147264}{17.91330891}
\toyPoint{22.86352158}{23.57724528}
\toyPoint{36.52726112}{59.87560026}
\toyPoint{57.99482376}{23.25080256}
\toyPoint{23.57404586}{23.58864015}
\toyPoint{23.09953905}{23.47781551}
\toyPoint{56.07682936}{18.97830779}
\toyPoint{23.14512622}{24.43093146}
\toyPoint{59.95384309}{20.99943592}
\toyPoint{59.80943218}{25.78716709}
\toyPoint{23.01816756}{23.67304341}
\toyPoint{23.61597676}{23.57746063}
\toyPoint{58.01359423}{22.14880420}
\toyPoint{23.14616603}{24.62029580}
\toyPoint{59.17780907}{22.27329254}
\toyPoint{57.38996967}{20.00473515}
\toyPoint{22.90423732}{23.55424173}
\toyPoint{55.70173540}{18.28761993}
\toyPoint{56.59757245}{15.88664486}
\toyPoint{23.13309762}{24.26774702}
\toyPoint{23.79759942}{24.46974293}
\toyPoint{57.51442417}{19.73609124}
\toyPoint{56.37775052}{24.65343291}
\toyPoint{22.96948556}{25.43618110}
\toyPoint{58.95788408}{21.84644638}
\toyPoint{59.36707343}{11.47922824}
\toyPoint{47.81058419}{59.68713268}
\toyPoint{22.62080839}{25.55754077}
\toyPoint{22.52684685}{25.44035112}
\toyPoint{23.15739632}{23.87177375}
\toyPoint{57.43753187}{22.46686997}
\toyPoint{56.86100806}{19.97602955}
\toyPoint{59.92348394}{21.42831864}
\toyPoint{56.00703116}{18.79734347}
\toyPoint{66.24031805}{43.59461538}
\toyPoint{21.19117521}{25.19485997}
\toyPoint{56.61531848}{25.10415170}
\toyPoint{57.67759631}{20.24488880}
\toyPoint{56.43952708}{19.12751629}
\toyPoint{56.02550476}{18.79240590}
\toyPoint{56.59563126}{25.98060608}
\toyPoint{18.87127784}{22.61910100}
\toyPoint{65.86695148}{43.04376521}
\toyPoint{59.46035662}{21.28759938}
\toyPoint{56.10218325}{19.20207054}
\toyPoint{37.36134833}{59.88574613}
\toyPoint{60.20117083}{24.53121493}
\toyPoint{57.71583865}{25.46959046}
\toyPoint{59.04005235}{21.53993237}
\toyPoint{57.32143894}{19.74366834}
\toyPoint{57.76507285}{20.13255058}
\toyPoint{17.05549425}{23.93036935}
\toyPoint{56.82828165}{19.84845869}
\toyPoint{57.09335389}{20.30893880}
\toyPoint{63.25337625}{41.88801808}
\toyPoint{23.77733231}{23.66488795}
\toyPoint{23.24073976}{23.92480266}
\toyPoint{23.14264667}{24.93555131}
\toyPoint{59.10744021}{21.99140487}
\toyPoint{58.30190228}{22.50062543}
\toyPoint{23.12465606}{24.50022513}
\toyPoint{57.36986253}{23.66656150}
\toyPoint{56.07420521}{19.14157375}
\toyPoint{24.72547377}{19.23005319}
\toyPoint{58.04492704}{22.33960982}
\toyPoint{22.73068397}{24.20633808}
\toyPoint{55.89819385}{17.02327544}
\toyPoint{23.27650409}{23.66804584}
\toyPoint{23.13403283}{25.11069513}
\toyPoint{24.62322604}{19.35857773}
\toyPoint{22.84232386}{25.43919902}
\toyPoint{21.99897274}{25.53384350}
\toyPoint{55.10601351}{18.64843184}
\toyPoint{22.78800595}{23.90754731}
\toyPoint{59.57056599}{25.37671335}
\toyPoint{55.54541588}{17.43017443}
\toyPoint{56.09344021}{18.86499897}
\toyPoint{58.18558785}{23.32309415}
\toyPoint{57.54761357}{21.31163197}
\toyPoint{58.76346219}{52.26095538}
\toyPoint{23.31532940}{23.78297744}
\toyPoint{58.39668366}{21.27051015}
\toyPoint{55.63338464}{18.64650911}
\toyPoint{57.79850991}{24.30081183}
\toyPoint{57.26174201}{23.39382295}
\toyPoint{23.16271382}{24.18563720}
\toyPoint{56.39676863}{19.97499897}
\toyPoint{58.91490721}{24.95769808}
\toyPoint{22.92740083}{23.70659890}
\toyPoint{23.01663245}{24.88309614}
\toyPoint{56.36303625}{19.16665846}
\toyPoint{58.68037255}{21.06598700}
\toyPoint{23.13307916}{25.11664175}
\toyPoint{29.49022985}{58.88580784}
\toyPoint{23.10638089}{20.01643458}
\toyPoint{15.24046129}{41.94749005}
\toyPoint{59.22103820}{21.86504764}
\toyPoint{24.49368323}{19.08038170}
\toyPoint{47.55388275}{15.62492278}
\toyPoint{56.60736453}{25.62327047}
\toyPoint{22.45239719}{25.38836664}
\toyPoint{60.58590458}{24.96200961}
\toyPoint{55.86124359}{18.91695884}
\toyPoint{56.03453698}{18.92200562}
\toyPoint{57.37356801}{19.80874277}
\toyPoint{56.14095472}{18.94779021}
\toyPoint{56.72132861}{19.42362293}
\toyPoint{23.14703972}{24.62888349}
\toyPoint{58.49044677}{20.52677954}
\toyPoint{59.85862793}{25.62575925}
\toyPoint{57.89710137}{20.33220537}
\toyPoint{22.86588576}{23.62651640}
\toyPoint{23.60196698}{23.78126391}
\toyPoint{31.27449989}{17.42645817}
\toyPoint{21.77775260}{20.77541167}
\toyPoint{55.73907329}{17.66688562}
\toyPoint{61.16560167}{23.82936601}
\toyPoint{35.64720969}{16.84410464}
\toyPoint{62.80427871}{22.22709471}
\toyPoint{50.08848452}{17.19255570}
\toyPoint{23.02935016}{25.38431967}
\toyPoint{57.02782877}{19.69424648}
\toyPoint{55.66975194}{17.92192582}
\toyPoint{62.92596602}{18.61020796}
\toyPoint{22.65062609}{25.43621802}
\toyPoint{22.88546993}{23.74751153}
\toyPoint{21.57376935}{25.60284953}
\toyPoint{59.50784499}{21.76397354}
\toyPoint{58.23059974}{20.84787246}
\toyPoint{23.18732785}{23.50744709}
\toyPoint{23.08024099}{25.27489939}
\toyPoint{57.97525037}{20.44741231}
\toyPoint{15.24242247}{43.23187997}
\toyPoint{22.90874881}{23.43002412}
\toyPoint{55.79789500}{18.88832861}
\toyPoint{16.92026323}{41.43315927}
\toyPoint{23.19197162}{23.44949907}
\toyPoint{23.12018148}{24.53272389}
\toyPoint{63.02501586}{23.00510530}
\toyPoint{22.87335673}{23.43051941}
\toyPoint{23.14458170}{24.63314733}
\toyPoint{22.80761011}{23.58154297}
\toyPoint{55.70202151}{17.97231367}
\toyPoint{25.96766380}{21.28682721}
\toyPoint{61.80404048}{30.46842052}
\toyPoint{60.76824711}{26.26038490}
\toyPoint{22.85581527}{25.43123430}
\toyPoint{23.10283076}{23.61116225}
\toyPoint{20.70054823}{53.36597012}
\toyPoint{56.31802282}{24.11823396}
\toyPoint{58.62553935}{21.14172413}
\toyPoint{22.82688510}{23.83502960}
\toyPoint{22.60910280}{24.21223856}
\toyPoint{59.03726516}{22.09652132}
\toyPoint{23.32495382}{23.49330195}
\toyPoint{40.48004970}{15.14104382}
\toyPoint{23.10625015}{24.37004243}
\toyPoint{59.83394777}{25.82695530}
\toyPoint{23.00030616}{24.20490449}
\toyPoint{64.38529230}{20.26309167}
\toyPoint{56.14055326}{23.74791761}
\toyPoint{56.28614549}{19.07558103}
\toyPoint{23.10936651}{23.91159427}
\toyPoint{59.32852653}{22.15372793}
\toyPoint{23.11569152}{24.72871780}
\toyPoint{57.92047870}{21.32890732}
\toyPoint{25.72472757}{19.66495329}
\toyPoint{55.63787460}{17.79922024}
\toyPoint{56.02065332}{25.81070592}
\toyPoint{58.08986971}{20.78491457}
\toyPoint{44.52285582}{61.71921576}
\toyPoint{55.68124833}{17.59535236}
\toyPoint{26.95705937}{56.12649425}
\toyPoint{57.49854857}{19.86971178}
\toyPoint{22.96864571}{23.65314238}
\toyPoint{23.98430117}{24.16824956}
\toyPoint{23.11595455}{23.41377320}
\toyPoint{23.07530957}{24.93941215}
\toyPoint{56.40256759}{16.16996765}
\toyPoint{58.32727617}{25.58275469}
\toyPoint{22.75378135}{23.47725253}
\toyPoint{57.96595666}{20.23319552}
\toyPoint{23.15434456}{24.30472189}
\toyPoint{23.33686090}{23.54989021}
\toyPoint{55.76377653}{17.60702410}
\toyPoint{58.51336725}{20.83642837}
\toyPoint{57.34657595}{21.87264781}
\toyPoint{55.50426637}{18.96594078}
\toyPoint{58.91373050}{22.40308762}
\toyPoint{23.12215805}{24.53440512}
\toyPoint{55.26191158}{17.74470083}
\toyPoint{33.57232663}{63.75662711}
\toyPoint{56.28779596}{19.03297178}
\toyPoint{18.22154876}{23.88900449}
\toyPoint{22.86673638}{23.48327914}
\toyPoint{57.34076315}{24.14185432}
\toyPoint{56.07769843}{25.39863094}
\toyPoint{22.73952392}{25.38932031}
\toyPoint{13.22057601}{42.18298762}
\toyPoint{56.69162781}{20.92451711}
\toyPoint{58.90651334}{20.61759549}
\toyPoint{49.89904942}{16.16095389}
\toyPoint{58.23912590}{20.08556981}
\toyPoint{55.73999928}{18.31371984}
\toyPoint{23.03576131}{25.37653339}
\toyPoint{22.87799743}{23.68066049}
\toyPoint{22.95001676}{23.42502040}
\toyPoint{17.80076304}{23.95390357}
\toyPoint{21.26943034}{25.48136988}
\toyPoint{22.89104123}{25.04033858}
\toyPoint{23.11534389}{24.08263729}
\toyPoint{62.04126850}{24.52057685}
\toyPoint{23.03067300}{24.63492393}
\toyPoint{24.61814696}{24.15870205}
\toyPoint{23.00956142}{23.56729938}
\toyPoint{19.00890381}{22.37066884}
\toyPoint{22.88877241}{23.43279439}
\toyPoint{54.68377421}{18.88523840}
\toyPoint{59.71584751}{21.51149442}
\toyPoint{58.92594061}{20.61422533}
\toyPoint{25.03836355}{19.13186319}
\toyPoint{58.78021609}{20.98656285}
\toyPoint{22.43005814}{24.26756244}
\toyPoint{55.89663413}{18.93360815}
\toyPoint{23.09362473}{23.75804655}
\toyPoint{56.35055696}{19.45152098}
\toyPoint{22.78323758}{23.57449501}
\toyPoint{22.94778639}{23.45112801}
\toyPoint{56.35844323}{15.72355424}
\toyPoint{59.51189964}{25.54627203}
\toyPoint{55.56155143}{18.07747318}
\toyPoint{23.21312320}{24.10986316}
\toyPoint{22.87796205}{23.53550357}
\toyPoint{56.72557708}{24.95328965}
\toyPoint{48.49877327}{17.23941188}
\toyPoint{28.28586378}{60.20110161}
\toyPoint{55.12995689}{17.47704291}
\toyPoint{23.88547743}{23.92249999}
\toyPoint{25.77768264}{18.96772354}
\toyPoint{22.94687886}{25.47905337}
\toyPoint{23.10224164}{24.36626157}
\toyPoint{44.06806007}{60.94489682}
\toyPoint{55.93858196}{18.62920761}
\toyPoint{23.02650452}{24.69548379}
\toyPoint{59.17935648}{24.10290441}
\toyPoint{57.24283157}{24.79203870}
\toyPoint{55.67708292}{18.20291827}
\toyPoint{59.77430313}{15.43963002}
\toyPoint{57.40791721}{23.76145824}
\toyPoint{55.70483023}{17.91814343}
\toyPoint{56.17811418}{18.90933867}
\toyPoint{55.46158637}{17.81850446}
\toyPoint{23.97624570}{23.92245693}
\toyPoint{55.39856849}{18.10115045}
\toyPoint{26.53971457}{18.50404862}
\toyPoint{23.00571442}{25.13834707}
\toyPoint{55.81870817}{18.44067235}
\toyPoint{22.96417729}{23.88298711}
\toyPoint{23.37539550}{23.68541348}
\toyPoint{42.46143802}{17.20325839}
\toyPoint{21.38603087}{25.57607897}
\toyPoint{58.87664180}{21.99611172}
\toyPoint{22.84880423}{23.56320320}
\toyPoint{22.98708700}{23.55973151}
\toyPoint{59.11919501}{25.67393364}
\toyPoint{55.56378488}{18.53270808}
\toyPoint{55.67504483}{19.05311584}
\toyPoint{22.96199922}{23.63992630}
\toyPoint{23.12278563}{24.89911787}
\toyPoint{22.87002194}{23.45104187}
\toyPoint{57.51609310}{20.27515719}
\toyPoint{22.89471595}{23.70464233}
\toyPoint{56.70054159}{19.37542546}
\toyPoint{22.98481664}{24.63755884}
\toyPoint{23.01883205}{23.84248518}
\toyPoint{22.96374352}{25.11616030}
\toyPoint{23.58223208}{23.82069834}
\toyPoint{57.00892141}{19.55015244}
\toyPoint{57.47816916}{19.70928377}
\toyPoint{56.10514118}{18.83186648}
\toyPoint{55.28789920}{18.38263358}
\toyPoint{23.14841024}{23.41883690}
\toyPoint{23.16111411}{23.95433734}
\toyPoint{24.65001506}{53.43993679}
\toyPoint{23.02965010}{25.26482736}
\toyPoint{59.52841359}{21.61240085}
\toyPoint{23.29922153}{23.45878663}
\toyPoint{23.04796373}{23.97427682}
\toyPoint{56.35300729}{19.27753695}
\toyPoint{22.66584181}{25.42603985}
\toyPoint{22.56389249}{24.13378193}
\toyPoint{23.19270226}{24.04149240}
\toyPoint{57.39656233}{21.73391588}
\toyPoint{23.14323887}{23.42697236}
\toyPoint{23.18358391}{23.98784514}
\toyPoint{57.37394948}{19.70934376}
\toyPoint{22.46915879}{25.64924117}
\toyPoint{61.17764565}{24.97363060}
\toyPoint{58.88665230}{20.39171157}
\toyPoint{42.15648663}{14.37465729}
\toyPoint{55.71602668}{18.85241662}
\toyPoint{53.09740005}{17.58841053}
\toyPoint{23.14453709}{24.70544661}
\toyPoint{23.57650695}{23.55960077}
\toyPoint{23.01190715}{23.59209030}
\toyPoint{18.58955937}{25.00516492}
\toyPoint{55.83852768}{19.99640742}
\toyPoint{56.50470918}{19.42108800}
\toyPoint{22.65864772}{25.60428619}
\toyPoint{55.90621087}{18.58409266}
\toyPoint{23.30488051}{23.49947468}
\toyPoint{23.05476712}{24.51962932}
\toyPoint{56.83826447}{15.41018455}
\toyPoint{23.13353446}{25.11440831}
\toyPoint{56.23834179}{19.08960773}
\toyPoint{58.84345393}{20.63128379}
\toyPoint{23.14340499}{24.42080867}
\toyPoint{23.02571697}{23.95915647}
\toyPoint{23.16385823}{23.51488267}
\toyPoint{57.12420371}{25.45452549}
\toyPoint{24.46832780}{24.23226418}
\toyPoint{42.60339418}{16.24514026}
\toyPoint{58.14216183}{22.37621861}
\toyPoint{22.70618070}{25.39311040}
\toyPoint{23.07777220}{25.30108544}
\toyPoint{18.02768523}{24.51672831}
\toyPoint{23.09430615}{24.47097348}
\toyPoint{23.12125360}{25.00034578}
\toyPoint{20.59448581}{25.38752987}
\toyPoint{23.01801220}{24.09008518}
\toyPoint{22.98653941}{23.68051744}
\toyPoint{23.14554307}{24.46882925}
\toyPoint{23.31903642}{23.47402388}
\toyPoint{56.65191650}{56.20209448}
\toyPoint{27.39791916}{57.76089514}
\toyPoint{23.10792984}{24.92004025}
\toyPoint{57.35147661}{22.55407733}
\toyPoint{23.05696364}{23.46732816}
\toyPoint{22.83337931}{25.46943665}
\toyPoint{29.57544527}{17.76908875}
\toyPoint{22.86159731}{23.74713775}
\toyPoint{58.99252399}{22.46708224}
\toyPoint{55.93561019}{18.68300407}
\toyPoint{19.11671669}{36.26779633}
\toyPoint{23.09289563}{25.06502951}
\toyPoint{23.41405776}{23.59256252}
\toyPoint{59.93773060}{54.55448827}
\toyPoint{56.90630144}{19.40442485}
\toyPoint{59.48194811}{20.73707550}
\toyPoint{26.84606552}{18.37559023}
\toyPoint{22.92279243}{23.77917813}
\toyPoint{58.23604953}{23.10087727}


==> figures/toy8_native_data/logistic_30000.tex <==
% Generated from original vector marker centers; do not edit by hand.
\toyPoint{22.57376609}{20.41426443}
\toyPoint{22.49011347}{19.66056024}
\toyPoint{57.68380442}{23.02416340}
\toyPoint{19.65180797}{55.06695594}
\toyPoint{55.29494870}{20.88485041}
\toyPoint{18.86464365}{56.01660790}
\toyPoint{41.17278935}{64.08768439}
\toyPoint{57.83951021}{22.92950046}
\toyPoint{22.48473444}{21.27611222}
\toyPoint{49.25078161}{63.03943019}
\toyPoint{22.31459279}{19.07996331}
\toyPoint{17.60018072}{55.51509673}
\toyPoint{55.36467152}{21.95775247}
\toyPoint{21.50978396}{18.07273865}
\toyPoint{21.84496203}{18.22007518}
\toyPoint{20.94319374}{23.30255631}
\toyPoint{58.79673927}{26.54818381}
\toyPoint{21.89048459}{18.28024126}
\toyPoint{55.32892719}{20.98380950}
\toyPoint{55.26912566}{22.57958658}
\toyPoint{22.43492496}{21.75215413}
\toyPoint{22.45924827}{19.56178265}
\toyPoint{21.68822719}{18.20496405}
\toyPoint{57.45232613}{23.47986283}
\toyPoint{21.73981328}{18.18417857}
\toyPoint{57.44727319}{24.40141063}
\toyPoint{65.84631212}{24.84124522}
\toyPoint{57.04189854}{23.03681035}
\toyPoint{22.68585205}{22.32341274}
\toyPoint{22.55891185}{21.77608213}
\toyPoint{22.27239732}{18.97074607}
\toyPoint{60.93512474}{24.70775235}
\toyPoint{58.22350564}{25.09795589}
\toyPoint{57.33479807}{23.79486299}
\toyPoint{58.88055801}{22.87293526}
\toyPoint{21.49333154}{18.15233046}
\toyPoint{28.13905101}{15.59155495}
\toyPoint{57.23283645}{25.55527964}
\toyPoint{57.42710606}{23.27437524}
\toyPoint{22.12175677}{18.81532638}
\toyPoint{22.51693172}{19.60952790}
\toyPoint{55.23777900}{21.43508665}
\toyPoint{57.14263885}{23.02759047}
\toyPoint{21.88317360}{18.67306740}
\toyPoint{25.47275912}{23.65574806}
\toyPoint{22.34497962}{19.13819898}
\toyPoint{37.38347838}{64.10498281}
\toyPoint{57.03840533}{23.21405380}
\toyPoint{59.67529020}{21.02798462}
\toyPoint{55.38276672}{22.17827274}
\toyPoint{58.45304428}{24.86913250}
\toyPoint{56.61795339}{22.95851061}
\toyPoint{55.82739276}{22.80346470}
\toyPoint{23.25462957}{20.74302673}
\toyPoint{21.56209761}{18.07765468}
\toyPoint{22.41826334}{21.37283325}
\toyPoint{58.62779894}{23.16788366}
\toyPoint{44.55989799}{13.66195494}
\toyPoint{22.04858226}{18.71328169}
\toyPoint{22.43336062}{21.35189549}
\toyPoint{22.42677566}{20.49712335}
\toyPoint{22.58952018}{20.99610267}
\toyPoint{57.09986964}{23.59199647}
\toyPoint{21.49885670}{18.45418069}
\toyPoint{21.77424246}{22.85003477}
\toyPoint{57.05939078}{23.22221694}
\toyPoint{60.09139830}{25.27510551}
\toyPoint{58.86956000}{24.28470550}
\toyPoint{55.21308807}{21.83896157}
\toyPoint{22.67970085}{20.90936599}
\toyPoint{57.58837546}{56.82050151}
\toyPoint{58.19330185}{25.21571928}
\toyPoint{22.42264102}{21.62982541}
\toyPoint{22.55362049}{20.80608306}
\toyPoint{55.94973380}{22.73329581}
\toyPoint{22.01797547}{18.37162325}
\toyPoint{59.01568597}{22.97252040}
\toyPoint{61.46429862}{23.14723661}
\toyPoint{22.57210332}{20.17657034}
\toyPoint{22.42164427}{21.11827297}
\toyPoint{57.62835903}{24.46119678}
\toyPoint{21.94447487}{18.30012537}
\toyPoint{58.90613187}{24.16419337}
\toyPoint{57.24332225}{23.20012554}
\toyPoint{22.64407804}{20.82951115}
\toyPoint{55.43212398}{22.13466214}
\toyPoint{55.38990236}{20.42094323}
\toyPoint{21.82522866}{18.20159851}
\toyPoint{24.59940418}{21.89264574}
\toyPoint{57.29827543}{23.01965498}
\toyPoint{57.52312107}{26.64734440}
\toyPoint{21.97537391}{18.61145081}
\toyPoint{58.50107870}{23.93817409}
\toyPoint{56.68906366}{18.13668559}
\toyPoint{66.49110979}{45.83563735}
\toyPoint{21.57632428}{18.39347470}
\toyPoint{22.03606759}{18.74682642}
\toyPoint{22.39124667}{19.27181798}
\toyPoint{57.08112840}{24.88784759}
\toyPoint{56.70673124}{23.28992167}
\toyPoint{59.15077856}{23.29045080}
\toyPoint{55.64867266}{22.61871645}
\toyPoint{53.72595603}{15.62865903}
\toyPoint{21.52121882}{18.32501781}
\toyPoint{58.78860381}{26.45663569}
\toyPoint{57.49242044}{23.26359872}
\toyPoint{56.25531104}{22.82713121}
\toyPoint{55.68994215}{22.61154698}
\toyPoint{60.01500899}{26.90916184}
\toyPoint{19.42546106}{23.57000505}
\toyPoint{54.26125496}{15.96304186}
\toyPoint{58.81799390}{23.35490380}
\toyPoint{55.74669346}{22.91061463}
\toyPoint{57.84025777}{56.57862509}
\toyPoint{63.06762511}{21.84009060}
\toyPoint{42.71048623}{13.45258344}
\toyPoint{58.52028139}{23.67691348}
\toyPoint{57.16956169}{23.06920144}
\toyPoint{57.56430595}{23.17723428}
\toyPoint{19.00903302}{14.99923706}
\toyPoint{56.67375103}{23.22226001}
\toyPoint{56.93616067}{23.43480018}
\toyPoint{67.11077659}{24.66830561}
\toyPoint{22.41172914}{20.73355306}
\toyPoint{22.23918484}{18.88633051}
\toyPoint{21.84960427}{18.27805704}
\toyPoint{58.68775583}{24.00398839}
\toyPoint{58.04507779}{24.66950078}
\toyPoint{22.02047040}{18.39854456}
\toyPoint{57.73416304}{25.74958617}
\toyPoint{55.95090435}{22.85959613}
\toyPoint{17.17467585}{23.41809857}
\toyPoint{57.70754476}{24.61514288}
\toyPoint{22.71421925}{22.40990023}
\toyPoint{55.35767740}{21.03903955}
\toyPoint{22.45062674}{19.77513959}
\toyPoint{21.86294802}{18.36169735}
\toyPoint{17.61928189}{23.44887764}
\toyPoint{21.54197816}{18.26805422}
\toyPoint{22.08503723}{18.78009273}
\toyPoint{55.12108926}{22.32899481}
\toyPoint{22.91805021}{22.56105300}
\toyPoint{62.49289174}{23.01387602}
\toyPoint{55.35973703}{21.25605891}
\toyPoint{55.79025330}{22.66300232}
\toyPoint{59.62513155}{24.44113885}
\toyPoint{57.21141877}{23.93323345}
\toyPoint{69.55314267}{35.80205640}
\toyPoint{22.33155589}{19.26634819}
\toyPoint{57.97850209}{23.68070049}
\toyPoint{55.52886963}{22.42438532}
\toyPoint{31.32716887}{14.69537796}
\toyPoint{57.36436967}{25.70623398}
\toyPoint{21.86810401}{18.25312461}
\toyPoint{56.16344298}{23.35891539}
\toyPoint{62.71004185}{23.61653051}
\toyPoint{22.63041589}{20.38121039}
\toyPoint{21.75131275}{18.31468736}
\toyPoint{56.13524345}{22.86112816}
\toyPoint{58.22011394}{23.45610865}
\toyPoint{21.85423882}{18.35344653}
\toyPoint{54.82973406}{59.35777818}
\toyPoint{19.21560349}{55.95413915}
\toyPoint{35.15067377}{64.23362886}
\toyPoint{58.75454534}{23.86949724}
\toyPoint{16.52275793}{23.06734485}
\toyPoint{14.38388948}{36.56662672}
\toyPoint{59.57945055}{26.65408934}
\toyPoint{21.03321445}{17.90448435}
\toyPoint{61.93220815}{21.55665398}
\toyPoint{55.75503657}{22.67886254}
\toyPoint{55.66303007}{22.71535596}
\toyPoint{57.22104319}{23.09420924}
\toyPoint{55.99975863}{22.70977851}
\toyPoint{56.56423384}{22.98705009}
\toyPoint{21.92362170}{18.28187173}
\toyPoint{58.09877273}{23.18173808}
\toyPoint{61.78581299}{22.87156166}
\toyPoint{57.66965466}{23.25286065}
\toyPoint{22.84202853}{22.41068317}
\toyPoint{22.25273163}{19.35093295}
\toyPoint{16.69582675}{22.88346106}
\toyPoint{18.78859120}{23.45474735}
\toyPoint{55.03796731}{21.69341856}
\toyPoint{62.89641903}{20.36690220}
\toyPoint{24.04057872}{17.16826008}
\toyPoint{41.56061534}{18.60284621}
\toyPoint{14.92239860}{31.41898309}
\toyPoint{21.83944764}{18.45907365}
\toyPoint{56.89175175}{23.09905144}
\toyPoint{55.26565706}{21.81762388}
\toyPoint{29.62987623}{21.58985261}
\toyPoint{21.30094774}{18.10979043}
\toyPoint{23.15244029}{21.59876023}
\toyPoint{21.76759904}{18.61231373}
\toyPoint{58.98827399}{23.69815273}
\toyPoint{57.89120859}{23.45723152}
\toyPoint{22.52926027}{20.60175834}
\toyPoint{21.79832582}{18.36836384}
\toyPoint{57.72664593}{23.29609902}
\toyPoint{36.45708992}{64.50918997}
\toyPoint{22.60658633}{21.33189909}
\toyPoint{55.24482081}{22.71686185}
\toyPoint{33.08582275}{63.40577341}
\toyPoint{22.51095126}{21.03191468}
\toyPoint{22.00423948}{18.38467013}
\toyPoint{58.94105019}{18.09268582}
\toyPoint{22.63382296}{21.99795907}
\toyPoint{21.94424260}{18.30246341}
\toyPoint{22.97055767}{22.31635709}
\toyPoint{55.19345161}{21.90821524}
\toyPoint{18.12535686}{53.00501670}
\toyPoint{45.37159904}{13.83808628}
\toyPoint{31.36403453}{14.52838498}
\toyPoint{21.54767559}{18.26604228}
\toyPoint{22.54806149}{20.20414691}
\toyPoint{46.77758955}{63.54431921}
\toyPoint{56.80679629}{26.52215619}
\toyPoint{58.17383920}{23.52383952}
\toyPoint{22.93801277}{22.54476055}
\toyPoint{22.75914654}{22.49051802}
\toyPoint{58.65725056}{24.10800195}
\toyPoint{22.45667181}{21.72549125}
\toyPoint{13.91453712}{43.24114446}
\toyPoint{22.10873142}{18.54880825}
\toyPoint{61.25159541}{23.23449473}
\toyPoint{22.33860231}{19.16500953}
\toyPoint{38.10499337}{18.66534571}
\toyPoint{56.27666566}{26.32956935}
\toyPoint{56.04188027}{22.80451990}
\toyPoint{22.40663928}{19.30517043}
\toyPoint{59.00607078}{24.01777821}
\toyPoint{21.83373328}{18.25677010}
\toyPoint{57.55526912}{23.85352319}
\toyPoint{18.14192311}{53.81626591}
\toyPoint{55.29236763}{21.67050731}
\toyPoint{58.83632598}{27.32529456}
\toyPoint{57.78607369}{23.46058322}
\toyPoint{67.09533322}{45.43827511}
\toyPoint{55.28095738}{21.49642944}
\toyPoint{48.80094498}{62.15291300}
\toyPoint{57.01196855}{23.08154075}
\toyPoint{22.60401449}{20.36579009}
\toyPoint{22.57955890}{21.92852697}
\toyPoint{22.50506770}{21.55787837}
\toyPoint{21.73645235}{18.18524299}
\toyPoint{55.40788220}{20.54144767}
\toyPoint{37.24403812}{13.80431698}
\toyPoint{22.77553743}{21.84864598}
\toyPoint{57.72176835}{23.17692049}
\toyPoint{22.00688824}{18.36432918}
\toyPoint{22.48285478}{20.39467104}
\toyPoint{54.85313293}{21.72544971}
\toyPoint{58.10842330}{23.36244091}
\toyPoint{56.92220626}{24.38611184}
\toyPoint{55.45064988}{22.69418747}
\toyPoint{58.93233638}{24.08174207}
\toyPoint{22.00279359}{18.38073392}
\toyPoint{55.19712171}{21.48905846}
\toyPoint{64.30062756}{53.22552773}
\toyPoint{56.05850651}{22.77337166}
\toyPoint{21.03735216}{23.06400237}
\toyPoint{22.64940170}{21.17461512}
\toyPoint{58.69722489}{25.57296568}
\toyPoint{58.24198846}{27.09534830}
\toyPoint{21.31995355}{18.07760239}
\toyPoint{36.61608512}{65.24003982}
\toyPoint{56.43948401}{23.85759938}
\toyPoint{58.36498322}{23.09309559}
\toyPoint{15.13568632}{33.84391077}
\toyPoint{57.84957763}{23.00446387}
\toyPoint{55.43587408}{22.17370125}
\toyPoint{21.91360966}{18.52386967}
\toyPoint{22.69323841}{20.66596369}
\toyPoint{22.58255989}{21.94312434}
\toyPoint{19.94361385}{23.63333364}
\toyPoint{21.95140285}{18.60017284}
\toyPoint{21.37291785}{17.87462665}
\toyPoint{22.63087734}{22.23941249}
\toyPoint{54.41021735}{19.72348582}
\toyPoint{21.89471614}{18.34309455}
\toyPoint{22.39764860}{20.25672974}
\toyPoint{22.59221354}{20.53003280}
\toyPoint{18.94257269}{23.66513714}
\toyPoint{22.61708598}{21.36023398}
\toyPoint{54.77696819}{22.48555276}
\toyPoint{59.07728257}{23.43907018}
\toyPoint{58.37563515}{23.08398954}
\toyPoint{17.20549337}{23.40662372}
\toyPoint{58.29711545}{23.37159926}
\toyPoint{22.81938799}{22.58121244}
\toyPoint{55.78722923}{22.69410287}
\toyPoint{22.50072541}{19.74782759}
\toyPoint{56.09523835}{23.04920504}
\toyPoint{23.00459154}{22.16634719}
\toyPoint{22.60377915}{22.05316297}
\toyPoint{55.77557133}{20.17855306}
\toyPoint{62.31480229}{23.19881654}
\toyPoint{55.34836523}{21.89111986}
\toyPoint{21.39437860}{17.92234882}
\toyPoint{22.73549541}{22.28583951}
\toyPoint{58.77012407}{26.30427237}
\toyPoint{17.48639814}{20.69183903}
\toyPoint{57.42768749}{58.55241099}
\toyPoint{55.04148053}{21.30409794}
\toyPoint{22.49306371}{21.86568906}
\toyPoint{17.80374712}{23.37004262}
\toyPoint{21.88500404}{18.54774229}
\toyPoint{22.11350595}{18.56218738}
\toyPoint{65.55047774}{47.84803667}
\toyPoint{55.61056106}{22.47611446}
\toyPoint{21.69016992}{18.20482869}
\toyPoint{62.96321315}{22.98554574}
\toyPoint{59.76637687}{25.65340965}
\toyPoint{55.38851953}{22.05538104}
\toyPoint{19.74102728}{28.74406122}
\toyPoint{57.92638533}{25.69811852}
\toyPoint{54.88782821}{21.96808446}
\toyPoint{56.01271168}{22.68134209}
\toyPoint{55.30603132}{21.59980466}
\toyPoint{22.17916335}{19.35767789}
\toyPoint{55.28969273}{21.85727212}
\toyPoint{16.61993888}{23.09393237}
\toyPoint{21.88096785}{18.48371998}
\toyPoint{55.50360957}{22.30158283}
\toyPoint{22.55452341}{19.88923596}
\toyPoint{22.39928523}{19.66531169}
\toyPoint{18.42645338}{20.16760734}
\toyPoint{21.99688235}{18.67961237}
\toyPoint{58.46218109}{24.08154826}
\toyPoint{22.68966213}{21.00097102}
\toyPoint{22.65095219}{22.24750180}
\toyPoint{62.35735924}{23.76050764}
\toyPoint{55.45618273}{22.30969829}
\toyPoint{55.59636362}{22.78340524}
\toyPoint{22.70830339}{22.34744226}
\toyPoint{21.82538863}{18.24672422}
\toyPoint{22.63493200}{21.30616373}
\toyPoint{57.34900628}{23.32152213}
\toyPoint{23.28462416}{22.33485991}
\toyPoint{56.54327147}{22.96020415}
\toyPoint{21.60544672}{18.15352255}
\toyPoint{22.51092665}{19.74396982}
\toyPoint{21.49489741}{18.03901549}
\toyPoint{22.50002707}{21.97962699}
\toyPoint{56.86948192}{23.01935503}
\toyPoint{57.25828263}{23.01322845}
\toyPoint{55.92105896}{22.62304491}
\toyPoint{55.24444242}{22.10496902}
\toyPoint{22.49791976}{21.47298136}
\toyPoint{22.62088530}{22.24305491}
\toyPoint{44.08072318}{63.55154714}
\toyPoint{21.66115976}{18.24908226}
\toyPoint{58.95376021}{23.57668231}
\toyPoint{22.46977868}{21.22726410}
\toyPoint{22.65710954}{22.31200710}
\toyPoint{56.19862895}{22.94286728}
\toyPoint{22.03447711}{18.72948800}
\toyPoint{22.96993625}{22.64012490}
\toyPoint{22.19074895}{18.71215420}
\toyPoint{56.98792365}{24.26683026}
\toyPoint{22.49606625}{21.68412024}
\toyPoint{22.26767663}{18.88896234}
\toyPoint{57.20384629}{23.03829931}
\toyPoint{22.05513185}{18.77999582}
\toyPoint{60.15205506}{20.86840568}
\toyPoint{58.28635277}{22.95712009}
\toyPoint{13.71480696}{42.56207758}
\toyPoint{55.62518458}{22.61446799}
\toyPoint{17.01053004}{28.56944192}
\toyPoint{21.89211046}{18.27168126}
\toyPoint{22.42227185}{21.23023433}
\toyPoint{22.58946634}{20.44034127}
\toyPoint{22.06361340}{22.67747202}
\toyPoint{55.46847744}{23.42889201}
\toyPoint{56.29887396}{23.01238706}
\toyPoint{22.06106309}{18.76050549}
\toyPoint{55.55799977}{22.44057009}
\toyPoint{22.46566711}{21.79219923}
\toyPoint{22.00556078}{18.46522177}
\toyPoint{55.91765189}{19.96506691}
\toyPoint{21.85636305}{18.35506008}
\toyPoint{56.10455975}{22.81409971}
\toyPoint{58.32947270}{23.12411462}
\toyPoint{22.03087776}{18.38978460}
\toyPoint{23.56213108}{22.59204741}
\toyPoint{22.53726344}{20.56611246}
\toyPoint{60.38136913}{25.98570054}
\toyPoint{22.62224813}{21.79901338}
\toyPoint{13.69151885}{39.98405451}
\toyPoint{57.82348079}{24.61756245}
\toyPoint{21.28527672}{18.05807206}
\toyPoint{21.83910616}{18.41781185}
\toyPoint{21.13626665}{23.29144755}
\toyPoint{22.04619962}{18.47081154}
\toyPoint{21.87170029}{18.36214496}
\toyPoint{21.72788774}{18.32693746}
\toyPoint{22.37274078}{19.24553194}
\toyPoint{22.58824502}{20.24114793}
\toyPoint{21.95809549}{18.30284642}
\toyPoint{22.47564377}{21.03457574}
\toyPoint{68.57458976}{32.37320192}
\toyPoint{52.64380563}{60.67950464}
\toyPoint{21.84747388}{18.33151202}
\toyPoint{57.01235771}{24.98808492}
\toyPoint{22.56534607}{20.89799112}
\toyPoint{22.04968360}{18.71175428}
\toyPoint{16.63199825}{22.92073280}
\toyPoint{22.88734344}{22.49510334}
\toyPoint{58.84183730}{24.32499978}
\toyPoint{55.74384320}{22.49694301}
\toyPoint{26.36208350}{60.69243462}
\toyPoint{21.73499415}{18.22095963}
\toyPoint{22.46795747}{21.89455924}
\toyPoint{66.45220911}{26.16185188}
\toyPoint{56.75730367}{22.95115502}
\toyPoint{58.69808936}{22.95848600}
\toyPoint{16.52872455}{22.96665068}
\toyPoint{22.63714083}{20.28337109}
\toyPoint{58.41316531}{24.97937572}


==> figures/toy8_native_data/logistic_5000.tex <==
% Generated from original vector marker centers; do not edit by hand.
\toyPoint{21.55312538}{23.34837421}
\toyPoint{21.16293261}{23.41343326}
\toyPoint{59.17886119}{21.73285146}
\toyPoint{18.72652700}{47.46827741}
\toyPoint{60.39752314}{16.61276017}
\toyPoint{54.16505537}{62.22540455}
\toyPoint{23.67908232}{52.86911503}
\toyPoint{59.32136013}{22.08359288}
\toyPoint{21.70370594}{23.15031759}
\toyPoint{64.31961336}{48.75741282}
\toyPoint{20.95340729}{23.78879178}
\toyPoint{59.42004388}{56.89101804}
\toyPoint{59.51306405}{18.62334713}
\toyPoint{19.64128833}{23.74726234}
\toyPoint{19.09126436}{22.30380397}
\toyPoint{22.40622705}{17.71510616}
\toyPoint{48.24149732}{15.26558445}
\toyPoint{19.27564652}{22.77196884}
\toyPoint{60.10427598}{16.97924029}
\toyPoint{58.88431734}{19.77165561}
\toyPoint{21.41316752}{23.11101237}
\toyPoint{20.95883862}{23.09433845}
\toyPoint{19.49670207}{23.47382392}
\toyPoint{59.02441825}{22.03442174}
\toyPoint{18.73618680}{22.05704997}
\toyPoint{59.15549617}{23.04308307}
\toyPoint{65.36230241}{42.84117576}
\toyPoint{59.68123067}{21.10229277}
\toyPoint{18.45110586}{24.20724561}
\toyPoint{21.43800766}{22.66765841}
\toyPoint{20.85919965}{23.76581130}
\toyPoint{16.64739240}{30.69498893}
\toyPoint{60.56263801}{18.19623639}
\toyPoint{58.69158899}{22.38433253}
\toyPoint{62.81291562}{18.69465889}
\toyPoint{18.75133484}{20.76689782}
\toyPoint{62.07457173}{29.25396242}
\toyPoint{61.68469121}{22.97656275}
\toyPoint{59.30082383}{21.71975843}
\toyPoint{17.93590484}{22.41039707}
\toyPoint{21.60012768}{24.30573094}
\toyPoint{58.70203787}{18.44315806}
\toyPoint{59.18695050}{21.44744442}
\toyPoint{18.28539725}{22.88527458}
\toyPoint{23.56998351}{61.54037260}
\toyPoint{21.36649593}{24.35349311}
\toyPoint{27.95156248}{60.90502708}
\toyPoint{59.63813997}{21.30269204}
\toyPoint{18.55691141}{29.44659233}
\toyPoint{59.86061065}{18.71909603}
\toyPoint{56.33511974}{16.36079173}
\toyPoint{59.86445765}{20.65345826}
\toyPoint{60.09916767}{19.75926553}
\toyPoint{22.24122601}{25.26402750}
\toyPoint{19.76931449}{23.77931349}
\toyPoint{21.51653813}{22.44759960}
\toyPoint{61.56660018}{22.63930659}
\toyPoint{64.99887559}{37.22138932}
\toyPoint{17.07650738}{21.85338513}
\toyPoint{21.63725484}{22.88916926}
\toyPoint{21.18402420}{22.33698876}
\toyPoint{21.78554043}{23.55710891}
\toyPoint{59.14402285}{21.89868004}
\toyPoint{18.08330444}{22.91442010}
\toyPoint{17.45106143}{22.78259154}
\toyPoint{59.61953871}{21.33120075}
\toyPoint{22.52452266}{23.10754684}
\toyPoint{46.93644016}{14.56630891}
\toyPoint{59.90559332}{18.09481159}
\toyPoint{21.87933737}{24.07106400}
\toyPoint{53.50942581}{62.82662238}
\toyPoint{57.52132447}{16.86301047}
\toyPoint{21.54239808}{23.04965111}
\toyPoint{21.66525749}{23.23327034}
\toyPoint{59.55241080}{20.07604384}
\toyPoint{19.73460997}{22.85264969}
\toyPoint{62.66886465}{18.61362888}
\toyPoint{33.10126689}{17.48279418}
\toyPoint{21.49998573}{23.51266000}
\toyPoint{21.52653325}{22.56042234}
\toyPoint{59.88400798}{23.11955544}
\toyPoint{19.57201004}{22.91794715}
\toyPoint{57.45297063}{16.51113233}
\toyPoint{59.51204884}{21.45917923}
\toyPoint{21.83360715}{23.86206473}
\toyPoint{59.63917517}{18.83327238}
\toyPoint{61.32563899}{15.43430944}
\toyPoint{19.13214776}{22.01692643}
\toyPoint{19.93833788}{26.39122286}
\toyPoint{59.43973264}{21.35739296}
\toyPoint{60.01214027}{18.37911267}
\toyPoint{18.54640099}{22.73370189}
\toyPoint{62.84446070}{22.55525097}
\toyPoint{65.03081137}{12.02378550}
\toyPoint{63.25699868}{51.71146131}
\toyPoint{18.77695176}{23.30044439}
\toyPoint{17.63806620}{21.98550593}
\toyPoint{20.70900825}{22.99108474}
\toyPoint{59.11080730}{23.13808441}
\toyPoint{59.76076095}{21.13004931}
\toyPoint{45.94017083}{14.25946882}
\toyPoint{60.06900849}{19.39633093}
\toyPoint{46.01449820}{15.54105636}
\toyPoint{16.16684360}{20.89998922}
\toyPoint{46.51722800}{15.14537534}
\toyPoint{59.25655950}{21.76458113}
\toyPoint{59.91760962}{20.21169170}
\toyPoint{60.03485464}{19.44018149}
\toyPoint{57.83159471}{17.69515745}
\toyPoint{25.37891603}{16.19575685}
\toyPoint{49.76887441}{17.21874945}
\toyPoint{63.47919864}{22.15675508}
\toyPoint{60.16751536}{19.78952469}
\toyPoint{52.03485074}{63.60186423}
\toyPoint{14.82455623}{47.91232970}
\toyPoint{65.44552126}{42.21344425}
\toyPoint{62.04534623}{22.75932497}
\toyPoint{59.60910520}{21.24465019}
\toyPoint{59.26984018}{21.72168270}
\toyPoint{13.31506052}{19.06654727}
\toyPoint{59.81879357}{21.00965561}
\toyPoint{59.48982054}{21.52881130}
\toyPoint{56.84180690}{59.30872086}
\toyPoint{21.25120132}{22.23974782}
\toyPoint{20.17681645}{22.48905520}
\toyPoint{19.40418182}{23.10632706}
\toyPoint{63.93942495}{21.48736646}
\toyPoint{62.73752920}{22.62389091}
\toyPoint{19.96096150}{23.20146376}
\toyPoint{61.14772950}{18.76744270}
\toyPoint{59.41891024}{20.32891673}
\toyPoint{30.33176668}{14.65505292}
\toyPoint{60.70139454}{23.12191809}
\toyPoint{17.99871352}{24.22280896}
\toyPoint{59.91468091}{17.20636706}
\toyPoint{20.92012098}{22.68541982}
\toyPoint{19.06696412}{22.92042978}
\toyPoint{23.63072180}{16.94202546}
\toyPoint{19.09524364}{23.45841285}
\toyPoint{17.27622217}{21.88645147}
\toyPoint{58.67754075}{19.46040861}
\toyPoint{17.64122871}{23.07782758}
\toyPoint{17.66976972}{30.37848134}
\toyPoint{59.04723414}{18.07843916}
\toyPoint{60.01791770}{19.59635181}
\toyPoint{15.66710441}{31.48559724}
\toyPoint{58.58706936}{22.47097077}
\toyPoint{56.79930072}{59.90222623}
\toyPoint{20.45536933}{22.43780444}
\toyPoint{59.20727145}{22.77618039}
\toyPoint{59.31741315}{19.48460425}
\toyPoint{50.23774532}{17.67933722}
\toyPoint{62.90572505}{22.35448099}
\toyPoint{19.25163700}{22.00657445}
\toyPoint{59.93444658}{20.76804376}
\toyPoint{15.14175754}{35.76076923}
\toyPoint{21.74529537}{23.92653311}
\toyPoint{18.38134612}{22.03320503}
\toyPoint{60.00526459}{20.11944371}
\toyPoint{59.57662183}{22.73323121}
\toyPoint{19.10474193}{22.96960246}
\toyPoint{61.90835399}{54.28456768}
\toyPoint{51.02165484}{64.30928599}
\toyPoint{50.02148505}{64.98280617}
\toyPoint{63.98514132}{21.48023544}
\toyPoint{51.55236229}{18.48537814}
\toyPoint{25.02597501}{62.25340259}
\toyPoint{49.57610992}{15.47921211}
\toyPoint{19.21495438}{23.77177946}
\toyPoint{14.78154859}{39.59023508}
\toyPoint{59.40944733}{19.94360462}
\toyPoint{60.12878080}{19.49762652}
\toyPoint{59.57501904}{21.31470834}
\toyPoint{59.64318522}{20.02786329}
\toyPoint{59.90226007}{20.63118227}
\toyPoint{19.41738252}{22.76072318}
\toyPoint{59.10356245}{22.29837725}
\toyPoint{23.90528310}{22.83182575}
\toyPoint{59.12037173}{21.91865183}
\toyPoint{18.04105666}{24.62207856}
\toyPoint{20.27705377}{21.94175536}
\toyPoint{25.24368348}{16.16867711}
\toyPoint{19.59427526}{19.64725648}
\toyPoint{60.26907859}{17.49143108}
\toyPoint{20.87074680}{58.96742236}
\toyPoint{62.09483577}{51.09469937}
\toyPoint{16.11440382}{37.30053563}
\toyPoint{18.39946593}{33.08888220}
\toyPoint{18.90615771}{23.06584820}
\toyPoint{59.77002236}{21.03441269}
\toyPoint{59.76653068}{18.20117704}
\toyPoint{33.04635217}{66.43067760}
\toyPoint{19.13726991}{23.61941153}
\toyPoint{21.03337596}{25.39508543}
\toyPoint{17.72810690}{22.57864675}
\toyPoint{63.43419137}{19.69592156}
\toyPoint{58.90429374}{22.42261179}
\toyPoint{21.51395398}{23.00454232}
\toyPoint{19.09731404}{23.15401231}
\toyPoint{59.03833420}{22.03291739}
\toyPoint{52.59222569}{63.63508901}
\toyPoint{21.77730191}{23.87509161}
\toyPoint{60.36031754}{18.99371116}
\toyPoint{36.27548226}{66.35921355}
\toyPoint{21.68013173}{23.09775629}
\toyPoint{19.97250403}{23.26025163}
\toyPoint{30.98060131}{64.49719214}
\toyPoint{20.63176524}{24.63344882}
\toyPoint{19.61250890}{22.97893463}
\toyPoint{18.36618116}{24.97302148}
\toyPoint{59.97924466}{18.12190056}
\toyPoint{31.63960872}{65.70506065}
\toyPoint{63.00845269}{31.17599610}
\toyPoint{41.03289466}{14.37695072}
\toyPoint{19.10926265}{23.45987412}
\toyPoint{21.39375871}{23.20108844}
\toyPoint{60.54494581}{56.33148193}
\toyPoint{62.51772419}{22.43736913}
\toyPoint{59.53330348}{22.76486089}
\toyPoint{17.62549000}{23.28739905}
\toyPoint{17.61258771}{23.83137026}
\toyPoint{63.93554718}{21.29657315}
\toyPoint{21.46311083}{23.47272258}
\toyPoint{35.33214108}{67.08355688}
\toyPoint{20.23351239}{23.32793020}
\toyPoint{39.30214877}{15.89891034}
\toyPoint{21.22522139}{24.13620303}
\toyPoint{31.60083879}{65.90885470}
\toyPoint{59.63680175}{23.29896158}
\toyPoint{60.00662742}{19.97774001}
\toyPoint{20.83890484}{23.22598857}
\toyPoint{54.15914566}{15.50670562}
\toyPoint{18.93636457}{22.38516469}
\toyPoint{58.69790016}{22.63566417}
\toyPoint{43.09461317}{67.09474871}
\toyPoint{59.61103562}{18.13225869}
\toyPoint{61.77955412}{20.24084645}
\toyPoint{58.87593885}{22.32152539}
\toyPoint{63.44033180}{31.63139405}
\toyPoint{59.68013241}{17.85686062}
\toyPoint{47.61494714}{65.56355999}
\toyPoint{58.94981784}{21.64124181}
\toyPoint{21.65248902}{23.68743620}
\toyPoint{21.09571395}{23.15124050}
\toyPoint{21.64164943}{23.56852378}
\toyPoint{19.77462276}{23.58110766}
\toyPoint{60.85238887}{15.97987267}
\toyPoint{60.87527706}{27.37887259}
\toyPoint{20.83343352}{24.90268030}
\toyPoint{59.14289998}{21.87642866}
\toyPoint{19.60034186}{22.53727267}
\toyPoint{21.28460453}{22.67800116}
\toyPoint{60.70583067}{17.02503204}
\toyPoint{59.13918987}{22.52465648}
\toyPoint{58.32936502}{22.76822182}
\toyPoint{59.07415852}{19.94435833}
\toyPoint{22.98920970}{21.43188723}
\toyPoint{19.95442114}{23.24141656}
\toyPoint{58.61315697}{18.54051282}
\toyPoint{52.40281982}{17.97834181}
\toyPoint{59.97049701}{19.97028597}
\toyPoint{17.59113466}{22.22995881}
\toyPoint{21.83393017}{23.99286424}
\toyPoint{34.00964899}{16.53340986}
\toyPoint{59.70287446}{18.41918084}
\toyPoint{19.26410398}{23.67714113}
\toyPoint{60.65256027}{56.04553038}
\toyPoint{59.16874455}{21.79539557}
\toyPoint{59.81496042}{22.51663639}
\toyPoint{20.57204062}{57.14858393}
\toyPoint{59.11859974}{21.90895511}
\toyPoint{59.72970194}{18.83439679}
\toyPoint{18.75106873}{22.87634080}
\toyPoint{21.89109064}{24.16389804}
\toyPoint{20.90301637}{24.38884981}
\toyPoint{41.73701336}{14.73890243}
\toyPoint{16.79134954}{21.63335246}
\toyPoint{20.11870077}{24.19096239}
\toyPoint{19.20669587}{24.32833764}
\toyPoint{24.48808578}{22.69419824}
\toyPoint{20.39957939}{23.91857455}
\toyPoint{20.59738836}{21.59060940}
\toyPoint{21.64875584}{23.48531108}
\toyPoint{31.25640700}{14.53713263}
\toyPoint{21.76541636}{23.95036267}
\toyPoint{58.15211850}{19.77467814}
\toyPoint{63.32335441}{19.40518471}
\toyPoint{59.87055656}{22.52013114}
\toyPoint{28.71543715}{15.02501703}
\toyPoint{59.73770972}{22.71020151}
\toyPoint{17.59989308}{22.86186649}
\toyPoint{59.42992518}{19.97598033}
\toyPoint{21.15388194}{23.26544608}
\toyPoint{60.06423550}{20.28792873}
\toyPoint{19.09693410}{25.28012614}
\toyPoint{20.47483044}{24.57503165}
\toyPoint{59.39240886}{17.19533828}
\toyPoint{20.55062602}{26.16788310}
\toyPoint{59.39293339}{18.59861620}
\toyPoint{18.50768336}{21.05974505}
\toyPoint{18.99137159}{24.91795140}
\toyPoint{43.81699878}{15.10903728}
\toyPoint{19.78534699}{19.48017120}
\toyPoint{64.97726256}{36.07598551}
\toyPoint{58.09711303}{18.67922014}
\toyPoint{21.21967777}{23.14736274}
\toyPoint{19.71532114}{19.51985021}
\toyPoint{18.72900194}{22.99017875}
\toyPoint{20.26617419}{23.35993674}
\toyPoint{65.19849500}{44.56916940}
\toyPoint{59.94734580}{19.24922512}
\toyPoint{18.48733471}{21.93926042}
\toyPoint{14.79699812}{48.61410479}
\toyPoint{28.46968220}{19.02616378}
\toyPoint{59.63885984}{18.69400363}
\toyPoint{51.92665639}{61.96005698}
\toyPoint{55.46219703}{16.31955916}
\toyPoint{60.56485299}{17.50328279}
\toyPoint{59.74619127}{19.94065131}
\toyPoint{59.10933218}{18.38733427}
\toyPoint{20.07897716}{21.56836725}
\toyPoint{59.06296822}{18.72291688}
\toyPoint{39.08566071}{14.27717947}
\toyPoint{18.33778320}{22.23709291}
\toyPoint{59.82166536}{19.00473995}
\toyPoint{21.55186253}{23.97225718}
\toyPoint{20.73458056}{22.43831050}
\toyPoint{38.28195957}{14.13206100}
\toyPoint{17.19762095}{22.04981435}
\toyPoint{63.08468203}{22.44391411}
\toyPoint{21.88063868}{24.13141004}
\toyPoint{19.38429310}{24.76241327}
\toyPoint{23.54923494}{23.00808168}
\toyPoint{59.27420247}{19.30253859}
\toyPoint{59.18428329}{20.10777197}
\toyPoint{18.62576516}{24.73530739}
\toyPoint{19.61150908}{23.31342513}
\toyPoint{21.78991349}{23.99861397}
\toyPoint{59.31443522}{21.71545459}
\toyPoint{18.03888475}{24.68351056}
\toyPoint{59.89934829}{20.58678104}
\toyPoint{18.34093186}{21.75181881}
\toyPoint{21.31100901}{23.63107866}
\toyPoint{19.74579565}{23.82535135}
\toyPoint{20.81903458}{23.65911053}
\toyPoint{59.77492917}{20.93163583}
\toyPoint{59.44288592}{21.32864583}
\toyPoint{59.76346201}{19.78583613}
\toyPoint{58.90984043}{19.10545103}
\toyPoint{21.68737196}{23.43234831}
\toyPoint{19.25396735}{24.39273988}
\toyPoint{37.16305925}{65.71943345}
\toyPoint{19.30705317}{23.42510346}
\toyPoint{64.10001909}{20.70399530}
\toyPoint{21.67547257}{23.01345764}
\toyPoint{18.75557407}{24.46032616}
\toyPoint{59.46562336}{20.58817156}
\toyPoint{17.81915049}{22.09975304}
\toyPoint{18.49099867}{21.41820200}
\toyPoint{20.06953424}{22.61021183}
\toyPoint{58.37463379}{22.69620557}
\toyPoint{21.51866390}{23.66948405}
\toyPoint{20.30224462}{22.76595454}
\toyPoint{59.56456707}{21.25602661}
\toyPoint{18.10680482}{22.64338124}
\toyPoint{15.92256454}{35.29104194}
\toyPoint{59.83555978}{22.38136076}
\toyPoint{40.32008305}{67.32798053}
\toyPoint{59.31233406}{19.81763501}
\toyPoint{18.80204570}{31.76115990}
\toyPoint{19.25188926}{22.67501093}
\toyPoint{21.57960984}{22.66790759}
\toyPoint{21.61362679}{23.48844128}
\toyPoint{17.60570126}{23.60819355}
\toyPoint{60.09726340}{20.25032166}
\toyPoint{59.99874730}{20.42706213}
\toyPoint{18.21073378}{22.64207225}
\toyPoint{59.95796696}{19.15371926}
\toyPoint{21.35781903}{23.60487723}
\toyPoint{20.40422470}{23.75291363}
\toyPoint{60.80449750}{15.94952429}
\toyPoint{19.09691565}{22.95819375}
\toyPoint{59.58223927}{20.27975636}
\toyPoint{59.65239894}{22.50550301}
\toyPoint{19.78989540}{22.89931666}
\toyPoint{20.56203012}{20.21183783}
\toyPoint{21.51556292}{23.05209375}
\toyPoint{35.37696031}{16.46105059}
\toyPoint{21.44732291}{22.60886900}
\toyPoint{21.86934840}{58.52846299}
\toyPoint{61.29745637}{23.05301051}
\toyPoint{19.25732367}{23.69165851}
\toyPoint{18.98765533}{23.05335352}
\toyPoint{23.93463935}{16.90786546}
\toyPoint{20.21583403}{23.45815597}
\toyPoint{18.84335210}{22.57151881}
\toyPoint{16.50817287}{21.53199227}
\toyPoint{21.09452340}{23.83355294}
\toyPoint{21.58010514}{23.63955252}
\toyPoint{19.48933109}{22.64098014}
\toyPoint{21.61900736}{22.88701580}
\toyPoint{62.97086870}{30.89897525}
\toyPoint{60.37905109}{56.59986742}
\toyPoint{18.77934056}{22.42960591}
\toyPoint{59.11376830}{23.15501367}
\toyPoint{21.72223491}{23.35195357}
\toyPoint{18.19818220}{22.44921161}
\toyPoint{30.77628736}{14.54540653}
\toyPoint{17.63436225}{23.96991914}
\toyPoint{51.09129537}{15.00227036}
\toyPoint{59.68644204}{19.52821178}
\toyPoint{19.96011088}{48.79599663}
\toyPoint{19.51816743}{23.41700800}
\toyPoint{21.12521787}{23.66670916}
\toyPoint{54.07050625}{19.77371523}
\toyPoint{59.74162286}{20.80340970}
\toyPoint{62.71088477}{22.33459534}
\toyPoint{42.53894675}{14.85907462}
\toyPoint{21.76805435}{24.07066407}
\toyPoint{51.59855243}{15.26771638}


==> figures/toy8_native_data/nextgan_0.tex <==
% Generated from original vector marker centers; do not edit by hand.
\toyPoint{40.41417864}{39.90581646}
\toyPoint{40.44728152}{39.90325303}
\toyPoint{40.58649836}{40.13321936}
\toyPoint{40.73147382}{39.83377199}
\toyPoint{41.12307447}{40.15253559}
\toyPoint{40.33770905}{39.96868067}
\toyPoint{40.80145463}{39.75011262}
\toyPoint{40.50027572}{40.12581327}
\toyPoint{40.31243418}{39.89858325}
\toyPoint{40.38169844}{39.96649718}
\toyPoint{40.56778644}{39.88890711}
\toyPoint{40.29253988}{39.94904889}
\toyPoint{40.89780765}{40.26286107}
\toyPoint{40.68574625}{39.88023336}
\toyPoint{40.16941315}{39.82813966}
\toyPoint{40.45256307}{39.93493233}
\toyPoint{40.67207116}{39.92559972}
\toyPoint{40.29241106}{39.87669134}
\toyPoint{41.09261880}{40.22338783}
\toyPoint{40.70530936}{40.31790637}
\toyPoint{40.22477214}{39.87115855}
\toyPoint{40.36353902}{39.89782256}
\toyPoint{40.56371823}{39.90430647}
\toyPoint{40.73310704}{40.00602238}
\toyPoint{40.11335585}{39.79580598}
\toyPoint{40.77322606}{39.87847762}
\toyPoint{40.54787191}{39.93317247}
\toyPoint{40.68903830}{40.13260822}
\toyPoint{40.31608961}{39.91548536}
\toyPoint{40.14901531}{39.80821746}
\toyPoint{40.56362839}{39.89025702}
\toyPoint{40.44838007}{40.01479738}
\toyPoint{40.61167815}{39.99039913}
\toyPoint{40.76887877}{39.93142161}
\toyPoint{40.41321785}{40.06170431}
\toyPoint{39.99254375}{39.58745972}
\toyPoint{40.59438814}{39.90645937}
\toyPoint{40.79108880}{39.82384354}
\toyPoint{40.70775771}{40.05958464}
\toyPoint{40.31564346}{39.88202971}
\toyPoint{40.71249806}{39.82892765}
\toyPoint{40.89505363}{40.44367967}
\toyPoint{40.54728427}{40.16575698}
\toyPoint{40.56904189}{39.92268609}
\toyPoint{40.44486556}{39.99250132}
\toyPoint{40.74191757}{39.81679067}
\toyPoint{40.71198219}{39.84585994}
\toyPoint{40.74811953}{40.05450662}
\toyPoint{40.58712022}{39.96493975}
\toyPoint{40.91794460}{40.14359355}
\toyPoint{40.56195225}{40.01379833}
\toyPoint{40.74383655}{40.12804957}
\toyPoint{40.87638690}{40.01353180}
\toyPoint{40.88017746}{39.68431284}
\toyPoint{40.67448919}{39.87985422}
\toyPoint{40.16651192}{39.82949536}
\toyPoint{40.54591875}{40.07426792}
\toyPoint{40.59816837}{39.90723394}
\toyPoint{40.27179884}{39.86322403}
\toyPoint{40.24894827}{39.87901423}
\toyPoint{40.18748927}{39.84331251}
\toyPoint{40.43590184}{39.90884842}
\toyPoint{40.78488257}{39.94780251}
\toyPoint{40.77969451}{39.90794973}
\toyPoint{40.29176791}{39.91455231}
\toyPoint{40.74677722}{40.05335795}
\toyPoint{40.49709995}{40.01062411}
\toyPoint{40.47530176}{40.03635060}
\toyPoint{40.97803858}{40.13647430}
\toyPoint{40.57903374}{39.88401472}
\toyPoint{40.58557511}{39.92609627}
\toyPoint{40.59681939}{39.99507565}
\toyPoint{40.23990235}{39.87747210}
\toyPoint{40.36860435}{39.90476390}
\toyPoint{40.70544972}{40.24330640}
\toyPoint{40.30829974}{39.88194238}
\toyPoint{40.42803268}{40.06209410}
\toyPoint{40.69500645}{39.89225034}
\toyPoint{40.46470271}{39.90400480}
\toyPoint{40.20550629}{39.85625455}
\toyPoint{40.75190269}{39.89968807}
\toyPoint{40.33061324}{39.88693842}
\toyPoint{40.51128879}{40.03724997}
\toyPoint{40.71636890}{40.07458936}
\toyPoint{40.52906111}{39.89714899}
\toyPoint{40.88353388}{40.22413731}
\toyPoint{41.20082171}{40.01230136}
\toyPoint{40.11599941}{39.79599659}
\toyPoint{41.00803346}{39.52997008}
\toyPoint{40.61905302}{40.15133521}
\toyPoint{40.73159049}{39.87598421}
\toyPoint{40.34465492}{39.89053391}
\toyPoint{40.61918329}{40.01628406}
\toyPoint{41.60852075}{40.29167682}
\toyPoint{40.52366742}{39.94620009}
\toyPoint{40.68285148}{39.90556632}
\toyPoint{40.13999453}{39.81096255}
\toyPoint{40.33898363}{39.89260524}
\toyPoint{40.81985535}{39.79885893}
\toyPoint{40.80489189}{39.98854900}
\toyPoint{40.39307360}{40.04024367}
\toyPoint{40.88989158}{40.04565426}
\toyPoint{40.33143807}{39.94323540}
\toyPoint{39.97629466}{39.69666932}
\toyPoint{40.65642720}{39.93822053}
\toyPoint{40.69739694}{40.06528046}
\toyPoint{40.78138901}{40.13588128}
\toyPoint{40.87955210}{40.06752139}
\toyPoint{40.79922546}{39.78359339}
\toyPoint{40.44419126}{39.93787617}
\toyPoint{40.35847911}{39.94913171}
\toyPoint{40.53911964}{40.06028307}
\toyPoint{40.89894399}{39.93873666}
\toyPoint{40.60305509}{39.91716548}
\toyPoint{40.40602059}{40.00596860}
\toyPoint{40.64924359}{39.87742413}
\toyPoint{40.60762153}{40.03232408}
\toyPoint{40.68341561}{40.12331408}
\toyPoint{40.66806424}{40.09236922}
\toyPoint{40.39440886}{39.84962957}
\toyPoint{40.80063093}{40.00867497}
\toyPoint{40.79157650}{39.97115923}
\toyPoint{40.72153302}{39.82494851}
\toyPoint{40.16463880}{39.82804639}
\toyPoint{40.22167261}{39.85537576}
\toyPoint{40.40577227}{39.90044916}
\toyPoint{40.58631022}{40.02586556}
\toyPoint{40.69155309}{39.94891435}
\toyPoint{40.40997656}{39.89990838}
\toyPoint{40.67125319}{39.94287196}
\toyPoint{40.65530048}{40.24706981}
\toyPoint{40.43457833}{39.94143346}
\toyPoint{40.74248915}{39.90399632}
\toyPoint{40.42152458}{39.92631135}
\toyPoint{41.06947230}{40.27063907}
\toyPoint{40.26543213}{39.87591313}
\toyPoint{40.35864865}{39.89309676}
\toyPoint{40.35843496}{39.93709823}
\toyPoint{40.66486934}{39.89993861}
\toyPoint{40.18926643}{39.83220865}
\toyPoint{40.74718450}{40.35389652}
\toyPoint{40.62858212}{39.87074418}
\toyPoint{40.53782021}{39.98939165}
\toyPoint{40.94752937}{40.42852351}
\toyPoint{40.86359314}{40.07886133}
\toyPoint{40.38927310}{40.01594775}
\toyPoint{40.78850946}{39.89526671}
\toyPoint{40.66968390}{39.86935206}
\toyPoint{40.21314078}{39.85296719}
\toyPoint{40.68323901}{40.00264058}
\toyPoint{40.76609821}{40.28910070}
\toyPoint{40.44348581}{39.94881193}
\toyPoint{40.76179860}{39.85762964}
\toyPoint{40.11726591}{39.79638916}
\toyPoint{40.87595774}{39.87402175}
\toyPoint{40.46633698}{40.00803123}
\toyPoint{40.57334347}{39.88540740}
\toyPoint{40.10376654}{39.79077777}
\toyPoint{40.82526726}{40.07542498}
\toyPoint{40.63477870}{40.04205195}
\toyPoint{40.37601364}{39.89647429}
\toyPoint{40.46002269}{39.96420973}
\toyPoint{40.36374095}{39.97522055}
\toyPoint{40.47429194}{39.96975341}
\toyPoint{40.57316889}{40.03390826}
\toyPoint{40.61436084}{39.89118121}
\toyPoint{40.49982994}{39.97947764}
\toyPoint{40.70978615}{39.88876920}
\toyPoint{40.88665178}{39.81854307}
\toyPoint{40.48588168}{40.00080201}
\toyPoint{40.70759539}{40.26503128}
\toyPoint{40.89689599}{40.00075098}
\toyPoint{40.68656225}{40.11434021}
\toyPoint{40.72635672}{40.22975617}
\toyPoint{40.76871586}{40.09987140}
\toyPoint{40.28599770}{39.87507233}
\toyPoint{40.60982896}{40.08449968}
\toyPoint{40.62128305}{39.94836235}
\toyPoint{40.67340357}{40.07238350}
\toyPoint{40.63109681}{39.86753327}
\toyPoint{40.12452799}{39.79743323}
\toyPoint{40.34427374}{39.93628567}
\toyPoint{40.30896337}{39.92447531}
\toyPoint{41.03351368}{40.00932914}
\toyPoint{40.33290466}{39.98612262}
\toyPoint{40.82875317}{39.70951609}
\toyPoint{40.60198768}{39.95024202}
\toyPoint{40.72422090}{39.84880445}
\toyPoint{40.45715936}{39.90919249}
\toyPoint{40.74291595}{40.08763065}
\toyPoint{40.96117123}{40.18997163}
\toyPoint{40.34692819}{39.98238954}
\toyPoint{40.78073966}{39.86819880}
\toyPoint{40.80133340}{39.74836981}
\toyPoint{40.66298362}{39.93016300}
\toyPoint{40.52070747}{40.04781829}
\toyPoint{40.67665841}{40.03233809}
\toyPoint{40.32365149}{39.89627213}
\toyPoint{40.46695605}{39.90862742}
\toyPoint{40.67476553}{40.06235662}
\toyPoint{40.45764528}{39.97141365}
\toyPoint{40.47979802}{39.90753459}
\toyPoint{40.95999164}{39.84168210}
\toyPoint{40.59228905}{39.93189218}
\toyPoint{40.32251506}{39.89890508}
\toyPoint{40.42922377}{39.90147171}
\toyPoint{40.29477537}{39.96052706}
\toyPoint{40.52953593}{39.90288786}
\toyPoint{40.34891461}{39.89085238}
\toyPoint{40.70746690}{39.82005685}
\toyPoint{40.97888352}{40.10203036}
\toyPoint{40.52259497}{39.96707180}
\toyPoint{40.54134361}{39.93119318}
\toyPoint{40.36371129}{39.94609251}
\toyPoint{40.66039485}{39.90033957}
\toyPoint{40.38225492}{39.90286143}
\toyPoint{40.43136324}{39.96933575}
\toyPoint{40.82285818}{39.76625229}
\toyPoint{40.64673275}{40.03205677}
\toyPoint{40.64709004}{39.86022103}
\toyPoint{40.47599635}{39.92243616}
\toyPoint{40.59110176}{40.02116497}
\toyPoint{40.30854147}{39.90214240}
\toyPoint{40.42822871}{39.98575563}
\toyPoint{40.44189172}{39.90180918}
\toyPoint{40.73742011}{39.85025544}
\toyPoint{40.67401235}{39.85257123}
\toyPoint{40.33680253}{39.98057237}
\toyPoint{40.89395460}{39.65869092}
\toyPoint{40.83289358}{40.08192047}
\toyPoint{40.40002758}{39.90080160}
\toyPoint{40.48284305}{40.04152181}
\toyPoint{40.18702721}{39.83665168}
\toyPoint{40.74522683}{39.94515077}
\toyPoint{40.41848974}{39.98167456}
\toyPoint{40.96036907}{40.25299487}
\toyPoint{40.84588701}{39.71966698}
\toyPoint{40.69004110}{40.02783346}
\toyPoint{40.36895535}{39.95802948}
\toyPoint{40.99326612}{40.25223654}
\toyPoint{40.58757374}{39.92825120}
\toyPoint{40.50173892}{40.15586292}
\toyPoint{40.50669135}{39.90003048}
\toyPoint{40.17818054}{39.83931244}
\toyPoint{40.36752359}{39.91045325}
\toyPoint{40.57301396}{39.89927942}
\toyPoint{41.17923752}{40.12358715}
\toyPoint{40.53649030}{39.93146631}
\toyPoint{40.64182834}{39.85937625}
\toyPoint{40.64930647}{40.09246997}
\toyPoint{40.22735605}{39.85549332}
\toyPoint{40.25693000}{39.87603734}
\toyPoint{41.05876096}{39.84083625}
\toyPoint{40.63882225}{40.05346069}
\toyPoint{40.83056092}{39.80372890}
\toyPoint{40.68627240}{40.29417728}
\toyPoint{40.38560163}{40.02346373}
\toyPoint{40.42358372}{39.90108901}
\toyPoint{40.88165172}{40.44477534}
\toyPoint{40.25063381}{39.91051499}
\toyPoint{40.82001321}{40.10834687}
\toyPoint{40.28374676}{39.91293069}
\toyPoint{40.53066847}{39.89790275}
\toyPoint{40.53230591}{40.00751371}
\toyPoint{40.77779726}{39.81610965}
\toyPoint{40.76734904}{39.86777774}
\toyPoint{40.37317180}{39.96980117}
\toyPoint{40.86726229}{39.80093453}
\toyPoint{40.56247336}{40.08883178}
\toyPoint{40.54666847}{39.96652993}
\toyPoint{40.56517836}{40.12693847}
\toyPoint{40.89262551}{40.19450476}
\toyPoint{40.38204597}{39.89855095}
\toyPoint{40.62395132}{39.86749901}
\toyPoint{40.47736081}{39.91261771}
\toyPoint{40.64762951}{39.86840873}
\toyPoint{40.23354109}{39.84650674}
\toyPoint{40.82693158}{39.80649984}
\toyPoint{40.33871157}{39.91756653}
\toyPoint{40.67732002}{39.90278457}
\toyPoint{40.64830357}{39.87395296}
\toyPoint{40.07586003}{39.71605799}
\toyPoint{40.44551271}{39.90624647}
\toyPoint{40.50663314}{39.92887403}
\toyPoint{40.49491424}{39.90558363}
\toyPoint{40.70964934}{40.36623103}
\toyPoint{40.49116011}{40.05628572}
\toyPoint{40.55924933}{40.08944383}
\toyPoint{40.41592967}{39.94190002}
\toyPoint{40.61613913}{40.05422867}
\toyPoint{40.53617935}{39.91007350}
\toyPoint{40.70498047}{40.26164819}
\toyPoint{40.40618229}{39.90271552}
\toyPoint{40.86094506}{39.97165857}
\toyPoint{40.73126939}{39.80275225}
\toyPoint{40.49450897}{39.91108663}
\toyPoint{41.06424805}{40.59542117}
\toyPoint{40.57667898}{39.97362862}
\toyPoint{40.89261993}{40.29501021}
\toyPoint{39.99272338}{39.65498327}
\toyPoint{40.58481857}{39.88760047}
\toyPoint{40.63170310}{39.95628816}
\toyPoint{40.22628697}{39.88494265}
\toyPoint{40.33792805}{39.95555902}
\toyPoint{40.88047789}{40.50078227}
\toyPoint{40.19864625}{39.85598354}
\toyPoint{40.28714737}{39.91792141}
\toyPoint{40.45616425}{39.91034052}
\toyPoint{40.45119332}{39.90202150}
\toyPoint{40.45260268}{39.96062534}
\toyPoint{40.87916226}{40.11310176}
\toyPoint{40.08664006}{39.77838161}
\toyPoint{40.36625615}{40.00200305}
\toyPoint{40.54329220}{39.99824997}
\toyPoint{40.89968039}{40.22447277}
\toyPoint{40.26958287}{39.93388295}
\toyPoint{40.62182353}{39.97493394}
\toyPoint{41.03212778}{39.85332054}
\toyPoint{40.75844094}{40.20687667}
\toyPoint{40.90713097}{40.37313229}
\toyPoint{40.07306371}{39.73818655}
\toyPoint{40.85987631}{40.35560785}
\toyPoint{40.50034672}{39.93359660}
\toyPoint{40.15736564}{39.82159875}
\toyPoint{40.88492747}{40.16295501}
\toyPoint{40.60410634}{39.87630724}
\toyPoint{40.21394174}{39.85476177}
\toyPoint{40.41790730}{39.94610576}
\toyPoint{40.42520805}{39.90792706}
\toyPoint{40.62739686}{40.00735163}
\toyPoint{40.58649000}{39.88165052}
\toyPoint{40.50846079}{39.91083366}
\toyPoint{40.59943223}{39.96296078}
\toyPoint{40.78915944}{40.29957886}
\toyPoint{40.66825820}{40.27711045}
\toyPoint{40.53599073}{39.90531660}
\toyPoint{40.47288532}{39.90509908}
\toyPoint{40.51511776}{39.90174166}
\toyPoint{40.72585066}{40.04158624}
\toyPoint{40.79568274}{39.74753193}
\toyPoint{40.76328516}{40.11230438}
\toyPoint{40.05246127}{39.75189365}
\toyPoint{40.50729311}{39.89893309}
\toyPoint{40.70603423}{39.87133259}
\toyPoint{40.25970123}{39.89044409}
\toyPoint{40.71597349}{40.12652850}
\toyPoint{40.61426754}{40.15594034}
\toyPoint{40.78233682}{40.20077728}
\toyPoint{40.80131600}{40.35407255}
\toyPoint{40.35028958}{39.90748204}
\toyPoint{40.36323777}{39.92063975}
\toyPoint{40.65873977}{39.88701687}
\toyPoint{40.57601746}{39.90642458}
\toyPoint{40.52675408}{40.05129150}
\toyPoint{40.28757261}{39.89160941}
\toyPoint{40.40089183}{39.92418677}
\toyPoint{40.62897369}{40.22733928}
\toyPoint{40.15944432}{39.82142787}
\toyPoint{40.64103623}{39.86507587}
\toyPoint{40.24719873}{39.86477403}
\toyPoint{40.82146372}{39.82438885}
\toyPoint{40.36504838}{39.91149736}
\toyPoint{40.28423883}{39.87777765}
\toyPoint{40.65756507}{40.14007529}
\toyPoint{40.43486333}{39.91023305}
\toyPoint{40.53742581}{39.98594503}
\toyPoint{40.52635035}{40.10507936}
\toyPoint{40.38259498}{39.98321767}
\toyPoint{40.71748101}{40.27981295}
\toyPoint{40.72123677}{39.85273373}
\toyPoint{40.26342864}{39.86764697}
\toyPoint{40.21752888}{39.86346009}
\toyPoint{40.44989605}{39.90571038}
\toyPoint{40.24598157}{39.89332742}
\toyPoint{40.94857802}{39.71350547}
\toyPoint{40.82451163}{40.03402646}
\toyPoint{40.38483191}{39.90018991}
\toyPoint{40.88961711}{40.10595908}
\toyPoint{40.32094107}{39.90580078}
\toyPoint{40.58255412}{39.89002706}
\toyPoint{41.22800373}{40.42094434}
\toyPoint{40.37186367}{39.89570338}
\toyPoint{40.68259729}{40.23226036}
\toyPoint{40.57315687}{40.08636948}
\toyPoint{40.32090372}{39.88514375}
\toyPoint{40.82277713}{39.71860335}
\toyPoint{40.33599898}{39.89847240}
\toyPoint{40.62167779}{39.95733268}
\toyPoint{40.13877129}{39.79257797}
\toyPoint{40.56080020}{39.95873602}
\toyPoint{40.72637912}{39.91996409}
\toyPoint{40.78307333}{39.86242612}
\toyPoint{40.43313157}{39.90588506}
\toyPoint{40.49165348}{39.92899821}
\toyPoint{40.48639784}{39.90193541}
\toyPoint{40.24203749}{39.85941732}
\toyPoint{40.37936698}{39.89228786}
\toyPoint{40.57752839}{39.88597868}
\toyPoint{40.49774171}{39.90099815}
\toyPoint{40.25241288}{39.86447090}
\toyPoint{40.27606742}{39.88658254}
\toyPoint{40.41550484}{39.95843602}
\toyPoint{40.46931347}{39.96380429}
\toyPoint{40.20022437}{39.84243758}
\toyPoint{40.82769932}{39.78453704}
\toyPoint{40.39194697}{39.90740945}
\toyPoint{40.26126444}{39.86515809}
\toyPoint{40.40990547}{39.94313311}
\toyPoint{40.63346903}{39.86720289}
\toyPoint{40.49411991}{40.03531891}
\toyPoint{40.80219916}{40.21925996}
\toyPoint{40.76062689}{39.80077679}
\toyPoint{40.53134383}{39.90586701}
\toyPoint{40.30099067}{39.90253585}
\toyPoint{40.34103283}{39.94847177}
\toyPoint{40.68311172}{40.16760869}
\toyPoint{40.49290234}{40.08392122}
\toyPoint{40.52633021}{39.92726408}
\toyPoint{40.61912412}{39.87002778}
\toyPoint{40.54651441}{40.01599236}


==> figures/toy8_native_data/nextgan_1000.tex <==
% Generated from original vector marker centers; do not edit by hand.
\toyPoint{52.77827447}{14.62622735}
\toyPoint{48.52806491}{12.43375163}
\toyPoint{40.62869258}{67.57431461}
\toyPoint{13.70492566}{28.38947435}
\toyPoint{12.64045592}{41.59493214}
\toyPoint{60.27834308}{56.76583752}
\toyPoint{19.22482952}{23.98913722}
\toyPoint{48.56869605}{64.67623834}
\toyPoint{66.71445416}{29.97234145}
\toyPoint{63.36865087}{53.45537093}
\toyPoint{37.76968225}{12.30391041}
\toyPoint{55.47794650}{58.78108671}
\toyPoint{20.78542525}{56.50266186}
\toyPoint{39.05700299}{13.35545632}
\toyPoint{65.14704427}{35.67252436}
\toyPoint{49.67465678}{32.69429638}
\toyPoint{11.08629288}{41.83546716}
\toyPoint{61.96786019}{25.34564664}
\toyPoint{13.91517085}{45.70708629}
\toyPoint{39.04573416}{64.05636695}
\toyPoint{65.11962152}{45.01384043}
\toyPoint{58.63639893}{17.72427836}
\toyPoint{45.62591476}{14.03465702}
\toyPoint{14.55051791}{51.89831380}
\toyPoint{65.12981046}{40.52292453}
\toyPoint{11.40909318}{34.76248564}
\toyPoint{25.77607524}{35.97890031}
\toyPoint{27.66125710}{64.66324222}
\toyPoint{67.97535004}{40.82780700}
\toyPoint{57.11953840}{55.78953343}
\toyPoint{38.54637423}{12.27415577}
\toyPoint{55.53080928}{62.02681265}
\toyPoint{22.51425835}{57.86220766}
\toyPoint{11.25209685}{41.02112245}
\toyPoint{52.06364478}{62.47850357}
\toyPoint{60.10380837}{61.80759676}
\toyPoint{16.97590859}{28.47222559}
\toyPoint{13.66950435}{29.45438400}
\toyPoint{19.85405153}{59.20718378}
\toyPoint{62.48857560}{27.24892601}
\toyPoint{28.59599867}{15.41210421}
\toyPoint{32.19433108}{61.95180462}
\toyPoint{45.75636664}{65.23948916}
\toyPoint{51.38073860}{16.27349054}
\toyPoint{56.38757183}{58.79815286}
\toyPoint{29.12482646}{15.14435707}
\toyPoint{13.19196270}{28.53105730}
\toyPoint{16.99481903}{55.32317131}
\toyPoint{22.65858312}{51.95692401}
\toyPoint{15.31435259}{49.30803207}
\toyPoint{34.44130159}{63.63846225}
\toyPoint{22.26540166}{60.58469557}
\toyPoint{12.95253508}{43.31971299}
\toyPoint{26.09196140}{16.13622296}
\toyPoint{38.77266749}{13.34872523}
\toyPoint{61.19268910}{49.96609580}
\toyPoint{42.89641426}{67.67586554}
\toyPoint{16.34006931}{29.46997658}
\toyPoint{65.26239272}{30.55871579}
\toyPoint{67.38726831}{39.01859097}
\toyPoint{65.15853759}{42.55781585}
\toyPoint{49.41450519}{14.42592344}
\toyPoint{11.68124722}{42.22093001}
\toyPoint{44.45550642}{12.75216195}
\toyPoint{66.40277801}{46.61781526}
\toyPoint{16.98705273}{55.34086966}
\toyPoint{47.69794064}{62.97329903}
\toyPoint{52.03591285}{64.52936172}
\toyPoint{14.08009806}{45.91037350}
\toyPoint{30.40194788}{13.65998914}
\toyPoint{18.21281495}{36.42243039}
\toyPoint{25.44349209}{59.38441338}
\toyPoint{66.58437298}{42.10667752}
\toyPoint{59.91808953}{20.09033818}
\toyPoint{34.27530150}{65.14646592}
\toyPoint{61.45438963}{23.08480478}
\toyPoint{52.85358398}{62.83656059}
\toyPoint{10.34760137}{35.50375092}
\toyPoint{45.52068026}{11.96672809}
\toyPoint{65.31028409}{43.26333584}
\toyPoint{10.78335977}{37.45983097}
\toyPoint{60.05647690}{21.89683576}
\toyPoint{46.56700980}{65.86046957}
\toyPoint{20.39480025}{59.60542894}
\toyPoint{35.55679983}{12.26499127}
\toyPoint{19.57830121}{55.58837891}
\toyPoint{11.16175621}{33.66967563}
\toyPoint{64.94261342}{41.27397651}
\toyPoint{24.96989896}{13.67358054}
\toyPoint{37.62450553}{67.32838661}
\toyPoint{10.87570313}{34.10674034}
\toyPoint{60.31629932}{24.35736625}
\toyPoint{24.79692090}{61.70755017}
\toyPoint{8.39595302}{39.04743731}
\toyPoint{33.17402224}{41.61912864}
\toyPoint{44.25086098}{13.70269222}
\toyPoint{66.18726915}{38.02080816}
\toyPoint{60.65498906}{19.80109184}
\toyPoint{14.90475255}{27.71203333}
\toyPoint{12.65886491}{45.21971756}
\toyPoint{53.29033144}{61.83342903}
\toyPoint{13.41566086}{44.83489460}
\toyPoint{65.12450218}{50.84983349}
\toyPoint{68.28672163}{47.13590114}
\toyPoint{12.39968085}{44.66518979}
\toyPoint{21.16613203}{60.53358632}
\toyPoint{20.21838588}{58.10064623}
\toyPoint{13.98591195}{46.85471489}
\toyPoint{16.17776163}{26.46979793}
\toyPoint{52.26489006}{35.21163702}
\toyPoint{65.48141326}{49.63942697}
\toyPoint{43.13276995}{67.35922414}
\toyPoint{12.53044805}{37.07486572}
\toyPoint{15.44767933}{34.53801763}
\toyPoint{58.62085558}{60.07569344}
\toyPoint{13.66843993}{27.19150251}
\toyPoint{28.47994189}{64.23135388}
\toyPoint{27.50129515}{64.71490214}
\toyPoint{26.53163448}{64.49183310}
\toyPoint{70.12957419}{26.79195219}
\toyPoint{13.29169243}{47.30413391}
\toyPoint{12.22690890}{44.30970461}
\toyPoint{15.62576878}{26.00366808}
\toyPoint{63.07677730}{46.69705406}
\toyPoint{65.82387617}{32.13604158}
\toyPoint{55.57166192}{18.41920545}
\toyPoint{31.29323959}{64.49354203}
\toyPoint{11.98954551}{46.34354045}
\toyPoint{54.26476202}{16.24423888}
\toyPoint{12.14616345}{45.65523563}
\toyPoint{39.49521105}{65.26452003}
\toyPoint{55.13029068}{38.24163318}
\toyPoint{10.63278690}{38.12118815}
\toyPoint{55.28606722}{28.14130599}
\toyPoint{15.32670421}{48.65703783}
\toyPoint{66.22454859}{29.43515516}
\toyPoint{58.83761498}{21.96348375}
\toyPoint{66.36632612}{44.35572363}
\toyPoint{43.14020899}{13.66341006}
\toyPoint{66.34603746}{35.04959929}
\toyPoint{37.75740908}{63.64787440}
\toyPoint{19.83855586}{20.13008641}
\toyPoint{36.45313986}{59.14662546}
\toyPoint{27.41023233}{60.02619159}
\toyPoint{14.54116421}{48.56587272}
\toyPoint{56.73529225}{60.68635571}
\toyPoint{11.43733732}{36.42717646}
\toyPoint{12.88285532}{28.20935526}
\toyPoint{66.27573321}{34.36706497}
\toyPoint{16.69554372}{55.35735746}
\toyPoint{31.70287348}{63.66891676}
\toyPoint{54.14915823}{42.45446832}
\toyPoint{11.86692146}{32.38210801}
\toyPoint{64.87729596}{41.55503894}
\toyPoint{12.86778727}{32.91767690}
\toyPoint{53.18559954}{61.82674408}
\toyPoint{32.67573664}{12.91955333}
\toyPoint{65.31873026}{40.87932896}
\toyPoint{15.26747488}{50.88746209}
\toyPoint{25.64438051}{63.52485964}
\toyPoint{57.86444264}{20.93078367}
\toyPoint{52.12060298}{50.02474908}
\toyPoint{61.76129741}{56.32643361}
\toyPoint{49.33979250}{52.30430295}
\toyPoint{34.62050007}{65.71724615}
\toyPoint{15.98848035}{25.54516146}
\toyPoint{44.24835105}{56.01052130}
\toyPoint{10.39607263}{35.46083135}
\toyPoint{34.60333355}{11.82780235}
\toyPoint{49.34269505}{61.15653869}
\toyPoint{35.54088731}{64.93446565}
\toyPoint{12.76854361}{41.46599268}
\toyPoint{26.40657856}{64.18004005}
\toyPoint{31.22893580}{64.55216992}
\toyPoint{18.74869377}{56.94211652}
\toyPoint{62.33200688}{25.46423297}
\toyPoint{33.57916001}{67.28790468}
\toyPoint{15.88316087}{47.08571326}
\toyPoint{24.10680217}{62.98230356}
\toyPoint{20.99149273}{19.19748675}
\toyPoint{63.32195159}{45.96788199}
\toyPoint{66.73590568}{46.15756858}
\toyPoint{66.48726740}{47.28464434}
\toyPoint{12.53168783}{37.21124384}
\toyPoint{54.94151546}{59.93541718}
\toyPoint{21.97442024}{21.52536423}
\toyPoint{18.36410769}{47.29965625}
\toyPoint{12.45107466}{29.96257397}
\toyPoint{54.03510186}{18.15569908}
\toyPoint{19.49452554}{58.26373685}
\toyPoint{15.64252115}{49.52454921}
\toyPoint{58.48221133}{58.36915170}
\toyPoint{38.42172246}{12.86959310}
\toyPoint{24.70659256}{18.21181513}
\toyPoint{50.35991484}{14.81638385}
\toyPoint{45.50410017}{66.60354799}
\toyPoint{20.00267398}{59.38950323}
\toyPoint{64.48295163}{24.89639836}
\toyPoint{52.83221399}{17.20951573}
\toyPoint{23.03098063}{62.18098333}
\toyPoint{53.30567637}{52.97714326}
\toyPoint{41.51173136}{13.30149681}
\toyPoint{13.46213556}{29.40307402}
\toyPoint{17.65229133}{39.69439271}
\toyPoint{65.49658437}{27.12647269}
\toyPoint{52.72232302}{15.44361391}
\toyPoint{51.26152546}{61.55834013}
\toyPoint{31.75138474}{15.09790390}
\toyPoint{58.93425603}{20.61004762}
\toyPoint{21.66644958}{20.00804224}
\toyPoint{13.51404006}{44.01898315}
\toyPoint{36.81456051}{51.75367217}
\toyPoint{27.00706728}{34.14320800}
\toyPoint{65.68781453}{47.84408200}
\toyPoint{43.24512528}{13.68933462}
\toyPoint{57.13926254}{16.90006379}
\toyPoint{58.27414574}{52.56225724}
\toyPoint{16.77270212}{25.61844364}
\toyPoint{23.05222296}{61.71352448}
\toyPoint{19.75992387}{20.34558450}
\toyPoint{41.92550536}{22.99650992}
\toyPoint{29.87299165}{63.75174953}
\toyPoint{67.71357259}{33.91850041}
\toyPoint{58.69987365}{57.24491273}
\toyPoint{51.07890375}{14.22117726}
\toyPoint{12.16112691}{30.85971848}
\toyPoint{31.19040274}{14.30844461}
\toyPoint{57.19850417}{58.81421920}
\toyPoint{20.20340243}{20.46713029}
\toyPoint{15.32018538}{50.80463086}
\toyPoint{54.44598782}{14.87982012}
\toyPoint{51.08005124}{65.05329501}
\toyPoint{64.88552063}{34.07251497}
\toyPoint{11.40031015}{43.65677495}
\toyPoint{59.91746349}{56.33821764}
\toyPoint{17.74741419}{52.67908389}
\toyPoint{19.07340757}{23.23315190}
\toyPoint{18.49319673}{57.80416120}
\toyPoint{64.46970171}{51.74493836}
\toyPoint{16.69260579}{51.03445791}
\toyPoint{18.05151478}{37.63383577}
\toyPoint{47.53307958}{63.73242224}
\toyPoint{39.56945681}{11.64305102}
\toyPoint{59.13918680}{53.03791077}
\toyPoint{61.83678842}{24.35071053}
\toyPoint{43.63312537}{13.45624124}
\toyPoint{11.88003909}{38.94062829}
\toyPoint{28.12806991}{33.80980038}
\toyPoint{23.65267938}{17.48267266}
\toyPoint{28.81565679}{65.69359195}
\toyPoint{64.74605806}{30.38763354}
\toyPoint{67.19459534}{32.96112753}
\toyPoint{12.60277348}{27.89058962}
\toyPoint{26.33377937}{64.18598821}
\toyPoint{14.61628914}{28.06730624}
\toyPoint{39.31065565}{64.40359362}
\toyPoint{55.23041571}{61.11919157}
\toyPoint{53.20472379}{15.71252085}
\toyPoint{33.30819730}{62.24456726}
\toyPoint{54.79371286}{58.62652071}
\toyPoint{16.84952982}{53.50029669}
\toyPoint{65.51866654}{47.97774330}
\toyPoint{34.31049593}{12.76929732}
\toyPoint{39.94734355}{62.91053188}
\toyPoint{14.20271289}{28.58134131}
\toyPoint{38.17378136}{13.00604543}
\toyPoint{63.00722522}{54.73130872}
\toyPoint{14.61523241}{27.75221302}
\toyPoint{41.24900899}{67.92911837}
\toyPoint{30.95636337}{52.00343640}
\toyPoint{42.98214036}{67.33794797}
\toyPoint{17.86971677}{53.56780914}
\toyPoint{58.25342947}{21.83768180}
\toyPoint{28.47653174}{14.79479082}
\toyPoint{41.29475969}{16.08653807}
\toyPoint{16.04949705}{23.90582915}
\toyPoint{66.52061216}{32.73561047}
\toyPoint{32.20334638}{13.25965205}
\toyPoint{67.17435898}{36.52236777}
\toyPoint{10.43823734}{36.82343948}
\toyPoint{36.36294688}{13.28402919}
\toyPoint{57.14040849}{58.74938780}
\toyPoint{47.95869135}{12.94435809}
\toyPoint{35.03926000}{29.37474605}
\toyPoint{38.93077074}{13.06170310}
\toyPoint{41.25517153}{63.11705312}
\toyPoint{50.10918310}{65.73769016}
\toyPoint{41.77538914}{67.89002388}
\toyPoint{59.17923804}{39.98799405}
\toyPoint{29.61681397}{65.60266064}
\toyPoint{28.25234828}{20.25822332}
\toyPoint{35.57035200}{64.99959084}
\toyPoint{53.72297041}{14.47853088}
\toyPoint{12.43723716}{40.93510593}
\toyPoint{22.57853754}{19.64366175}
\toyPoint{37.70330421}{16.05228270}
\toyPoint{32.76721093}{61.43201828}
\toyPoint{25.83351412}{54.63474766}
\toyPoint{22.75503651}{58.08499367}
\toyPoint{62.03620941}{55.62857166}
\toyPoint{24.03220638}{17.35979326}
\toyPoint{15.78704588}{49.32893215}
\toyPoint{56.85785324}{56.36670789}
\toyPoint{63.28007606}{53.80551554}
\toyPoint{38.02526774}{62.57906391}
\toyPoint{61.97404369}{49.47510965}
\toyPoint{64.79247124}{49.42124705}
\toyPoint{54.69310791}{18.72721918}
\toyPoint{50.18905947}{13.85994081}
\toyPoint{53.45323440}{48.49138921}
\toyPoint{15.27319385}{49.78854625}
\toyPoint{65.09824845}{42.56677424}
\toyPoint{56.97212496}{59.83643655}
\toyPoint{36.40826179}{61.16162700}
\toyPoint{18.88082074}{54.64347224}
\toyPoint{50.49957198}{62.13973076}
\toyPoint{19.11977460}{54.14789692}
\toyPoint{12.84360086}{28.96005231}
\toyPoint{26.63027979}{62.63134987}
\toyPoint{26.46970564}{59.99929797}
\toyPoint{60.00460932}{53.65041118}
\toyPoint{28.62300688}{61.42506415}
\toyPoint{37.20837070}{32.28699515}
\toyPoint{65.28600077}{36.67350208}
\toyPoint{16.87418538}{52.34937560}
\toyPoint{32.18620254}{13.38957018}
\toyPoint{66.52046142}{35.69247307}
\toyPoint{59.27532381}{42.39138988}
\toyPoint{60.58093163}{23.03975136}
\toyPoint{22.57422601}{59.95315244}
\toyPoint{29.51984682}{14.02963023}
\toyPoint{34.57371850}{17.12275751}
\toyPoint{20.44253934}{51.36908454}
\toyPoint{30.41877408}{63.02712779}
\toyPoint{39.93247027}{64.61468327}
\toyPoint{29.32918887}{17.40284089}
\toyPoint{50.60867002}{15.32620430}
\toyPoint{35.98671929}{12.84923677}
\toyPoint{17.28030605}{56.09648428}
\toyPoint{23.49315582}{19.55297655}
\toyPoint{19.84948158}{58.16428092}
\toyPoint{64.83518047}{45.51707168}
\toyPoint{41.14692853}{11.52838246}
\toyPoint{37.65983916}{13.35577934}
\toyPoint{66.90132510}{42.91109816}
\toyPoint{24.49041459}{62.61251327}
\toyPoint{38.53087587}{67.26093415}
\toyPoint{24.29187652}{60.99279434}
\toyPoint{33.17642027}{63.14111956}
\toyPoint{63.83889229}{26.06746274}
\toyPoint{64.88326103}{33.12760215}
\toyPoint{11.65385216}{31.35486772}
\toyPoint{45.99194188}{14.25879509}
\toyPoint{44.67198472}{66.86873405}
\toyPoint{67.65446324}{33.08858918}
\toyPoint{59.15139844}{29.03262077}
\toyPoint{40.93332145}{65.44566739}
\toyPoint{65.82319014}{36.73095172}
\toyPoint{18.99300052}{20.92513546}
\toyPoint{64.97650116}{28.82233174}
\toyPoint{13.72672789}{29.61335690}
\toyPoint{62.55582809}{25.69429767}
\toyPoint{63.80894384}{25.06800436}
\toyPoint{31.90983772}{66.44505655}
\toyPoint{57.64374856}{21.13990292}
\toyPoint{36.06206879}{58.24328207}
\toyPoint{46.73121022}{66.64390379}
\toyPoint{61.31638065}{57.12367458}
\toyPoint{35.57626324}{64.67537542}
\toyPoint{12.18045265}{30.33577750}
\toyPoint{63.15164997}{27.53020610}
\toyPoint{65.91244175}{42.33856574}
\toyPoint{47.35435255}{12.64502433}
\toyPoint{62.59973711}{50.45756802}
\toyPoint{16.01186076}{22.23518249}
\toyPoint{13.81218018}{47.84720375}
\toyPoint{59.39902459}{23.16170785}
\toyPoint{14.83275321}{48.71692550}
\toyPoint{67.25056064}{32.84351718}
\toyPoint{39.71002996}{12.71960781}
\toyPoint{15.75361344}{49.71093101}
\toyPoint{58.09983715}{21.16840547}
\toyPoint{35.86029514}{65.59114118}
\toyPoint{39.42703593}{67.97294432}
\toyPoint{60.74773850}{22.01116746}
\toyPoint{23.53009070}{19.72807884}
\toyPoint{63.26454193}{23.14936392}
\toyPoint{16.89735351}{49.68425428}
\toyPoint{55.86530285}{57.75741270}
\toyPoint{26.63219483}{49.28663515}
\toyPoint{10.61265515}{40.64285205}
\toyPoint{37.65701486}{12.90285480}
\toyPoint{55.04881459}{18.79470702}
\toyPoint{38.81041934}{28.52170283}
\toyPoint{47.40755604}{13.25838151}
\toyPoint{63.70934333}{29.93464208}
\toyPoint{63.69464136}{25.76015965}
\toyPoint{36.36918191}{12.46293099}
\toyPoint{41.00017776}{11.57182694}
\toyPoint{63.79372812}{28.07734982}
\toyPoint{67.63945672}{33.51998837}
\toyPoint{60.51556803}{48.83211859}
\toyPoint{49.86451257}{49.77325209}
\toyPoint{64.64333503}{33.12838739}
\toyPoint{15.58957377}{26.76644295}
\toyPoint{56.66947949}{17.86020925}
\toyPoint{63.66161962}{29.92513687}
\toyPoint{60.45857214}{41.30725436}
\toyPoint{20.30520408}{19.75753046}
\toyPoint{49.35388919}{65.21936355}
\toyPoint{24.03230483}{60.42474439}
\toyPoint{16.08079603}{26.44724815}
\toyPoint{47.34217705}{14.40838968}
\toyPoint{68.10331468}{36.61870387}
\toyPoint{64.94355171}{51.37926732}
\toyPoint{31.11327125}{65.69305051}
\toyPoint{49.82164721}{65.60699986}
\toyPoint{30.11379826}{30.06942395}
\toyPoint{29.98353481}{14.18778635}
\toyPoint{37.86593914}{64.14670452}


==> figures/toy8_native_data/nextgan_10000.tex <==
% Generated from original vector marker centers; do not edit by hand.
\toyPoint{63.02284856}{31.20743736}
\toyPoint{59.49222319}{16.81231806}
\toyPoint{34.71535990}{63.27303579}
\toyPoint{21.25237649}{20.59842971}
\toyPoint{17.11516503}{39.22491889}
\toyPoint{44.17418365}{62.48703895}
\toyPoint{21.62775347}{21.78166420}
\toyPoint{39.14761291}{66.01053176}
\toyPoint{60.88262804}{49.57500704}
\toyPoint{48.92575633}{59.22066442}
\toyPoint{57.88689552}{19.34856415}
\toyPoint{49.60494164}{60.12109603}
\toyPoint{18.66487657}{44.91363310}
\toyPoint{60.02585473}{19.75968084}
\toyPoint{66.51958466}{39.06750879}
\toyPoint{63.10607203}{34.59959884}
\toyPoint{21.60210425}{21.32734760}
\toyPoint{67.61135101}{38.19243685}
\toyPoint{16.62214618}{39.47817710}
\toyPoint{40.38357252}{66.23405149}
\toyPoint{57.91985573}{59.03459487}
\toyPoint{67.87398369}{39.85462463}
\toyPoint{59.23261304}{18.85100611}
\toyPoint{16.11583125}{39.56605319}
\toyPoint{65.12630186}{39.70307155}
\toyPoint{22.57543502}{21.66511136}
\toyPoint{29.49736011}{20.09269314}
\toyPoint{22.23249066}{57.97923580}
\toyPoint{57.72563534}{59.36580443}
\toyPoint{57.00986585}{59.25985429}
\toyPoint{59.79756971}{19.75830570}
\toyPoint{40.45713321}{66.14483679}
\toyPoint{14.25842439}{39.17808963}
\toyPoint{23.42218399}{24.12713851}
\toyPoint{39.88919458}{66.30866266}
\toyPoint{59.14961876}{61.80526949}
\toyPoint{37.95846862}{15.59898438}
\toyPoint{22.17727446}{20.90029993}
\toyPoint{15.52057543}{38.60277234}
\toyPoint{68.49944022}{39.39757662}
\toyPoint{40.64410836}{12.68121781}
\toyPoint{29.16632437}{59.52263463}
\toyPoint{38.92032156}{65.83408663}
\toyPoint{59.62594371}{18.79647593}
\toyPoint{40.21362872}{66.94583401}
\toyPoint{40.73457706}{12.63303572}
\toyPoint{20.99297400}{21.27319428}
\toyPoint{16.29634642}{39.60617325}
\toyPoint{19.55933694}{29.41603015}
\toyPoint{16.03296311}{39.91586360}
\toyPoint{22.10800386}{57.64190889}
\toyPoint{16.46714334}{42.30895300}
\toyPoint{16.93664335}{38.08660842}
\toyPoint{39.85603902}{12.45675364}
\toyPoint{59.53867789}{19.68322846}
\toyPoint{57.43163755}{59.17097799}
\toyPoint{27.77614870}{60.25645933}
\toyPoint{35.42576382}{17.00967327}
\toyPoint{67.02358307}{38.07786980}
\toyPoint{57.90272959}{59.34550039}
\toyPoint{57.92382117}{59.14276154}
\toyPoint{60.29844869}{23.48015662}
\toyPoint{18.82864706}{35.86578723}
\toyPoint{58.80963695}{19.35409546}
\toyPoint{57.65522957}{59.90874660}
\toyPoint{16.29628489}{39.59064088}
\toyPoint{25.34224264}{59.57639110}
\toyPoint{40.90920291}{66.54678898}
\toyPoint{16.18310990}{39.38400484}
\toyPoint{38.70744251}{12.18343366}
\toyPoint{24.23314402}{22.73169764}
\toyPoint{15.55501538}{43.04648511}
\toyPoint{58.03478887}{58.92734497}
\toyPoint{67.53504784}{39.48534350}
\toyPoint{22.04376467}{57.75643902}
\toyPoint{67.76347130}{38.30038048}
\toyPoint{39.80231514}{66.40466998}
\toyPoint{21.44107634}{20.69721191}
\toyPoint{60.13720236}{17.68772648}
\toyPoint{57.95237449}{58.98780484}
\toyPoint{22.58044028}{21.75433374}
\toyPoint{68.45715246}{39.21088257}
\toyPoint{31.01243788}{62.01834186}
\toyPoint{15.20283576}{38.43026496}
\toyPoint{49.81175823}{17.22282871}
\toyPoint{16.14158354}{38.68314882}
\toyPoint{16.22138762}{38.89861730}
\toyPoint{57.73990354}{58.32545188}
\toyPoint{39.92915084}{11.04054113}
\toyPoint{23.03240345}{58.11176577}
\toyPoint{21.75787157}{20.84625583}
\toyPoint{67.96984642}{38.68808831}
\toyPoint{16.02436312}{42.34436566}
\toyPoint{18.20833114}{38.69761236}
\toyPoint{21.23968647}{20.17897606}
\toyPoint{58.72752713}{19.16516181}
\toyPoint{67.17927810}{38.17027777}
\toyPoint{67.82135933}{38.74672736}
\toyPoint{22.41161377}{21.09164853}
\toyPoint{16.49447072}{39.06773048}
\toyPoint{40.05144794}{66.27713911}
\toyPoint{16.59706762}{38.34605782}
\toyPoint{58.97692065}{57.82495591}
\toyPoint{66.65360358}{38.81405619}
\toyPoint{21.94402879}{20.74675683}
\toyPoint{14.70803876}{38.04605515}
\toyPoint{15.47343316}{38.77744029}
\toyPoint{16.22097538}{38.75334770}
\toyPoint{21.86757641}{20.45538164}
\toyPoint{64.51360918}{41.37879310}
\toyPoint{58.82140560}{57.11713268}
\toyPoint{24.31712274}{58.88757675}
\toyPoint{17.08970808}{39.94125825}
\toyPoint{24.12732001}{22.49714451}
\toyPoint{39.32608614}{65.99826013}
\toyPoint{33.79658661}{16.88922882}
\toyPoint{22.52746982}{56.69254611}
\toyPoint{22.32869179}{58.19430474}
\toyPoint{23.01967036}{57.98365039}
\toyPoint{68.60996800}{37.23197145}
\toyPoint{16.40764944}{38.52637687}
\toyPoint{16.52649264}{39.84646995}
\toyPoint{26.39843695}{20.15040121}
\toyPoint{57.67535363}{59.11201631}
\toyPoint{65.71302998}{39.26549369}
\toyPoint{60.48093273}{19.91238871}
\toyPoint{22.07381464}{57.79830687}
\toyPoint{22.80000225}{23.33094043}
\toyPoint{60.50824473}{20.41246014}
\toyPoint{22.74139743}{20.61893217}
\toyPoint{41.34562100}{66.40418699}
\toyPoint{63.55149023}{53.43391326}
\toyPoint{22.49455267}{21.72499288}
\toyPoint{68.07118816}{41.47581947}
\toyPoint{16.91946184}{39.87701329}
\toyPoint{65.13143632}{39.94281124}
\toyPoint{66.87205345}{36.59018324}
\toyPoint{58.13885012}{59.18588915}
\toyPoint{58.69129673}{18.99345429}
\toyPoint{66.70044130}{37.99802649}
\toyPoint{41.10839240}{66.39489943}
\toyPoint{41.88016853}{12.17436144}
\toyPoint{22.23985088}{58.86645133}
\toyPoint{22.54742622}{57.68843897}
\toyPoint{16.04172461}{39.11193040}
\toyPoint{39.72593054}{66.33549475}
\toyPoint{23.19084567}{21.64431818}
\toyPoint{25.63231345}{20.67203030}
\toyPoint{59.41488481}{55.13444993}
\toyPoint{16.00678321}{40.12649238}
\toyPoint{21.81648716}{58.29778764}
\toyPoint{61.90951532}{58.88366976}
\toyPoint{22.07321167}{20.98545228}
\toyPoint{57.19586926}{60.05895953}
\toyPoint{23.99115224}{21.49050743}
\toyPoint{41.23734013}{67.02516740}
\toyPoint{40.99995848}{13.24593452}
\toyPoint{66.33347358}{38.85550641}
\toyPoint{16.05777710}{39.42080398}
\toyPoint{20.22941928}{49.58499447}
\toyPoint{64.40681611}{30.46333990}
\toyPoint{34.59138493}{60.98649856}
\toyPoint{41.74275060}{63.20998561}
\toyPoint{22.24717571}{59.56900012}
\toyPoint{21.96181020}{57.62762839}
\toyPoint{41.05341394}{13.33141450}
\toyPoint{20.19492703}{58.54193749}
\toyPoint{21.58001746}{20.82983263}
\toyPoint{36.97915700}{10.93384035}
\toyPoint{27.87920091}{61.01807594}
\toyPoint{31.17709129}{61.13960789}
\toyPoint{17.16338096}{38.13102234}
\toyPoint{22.87569631}{58.41171019}
\toyPoint{22.06414561}{58.02067757}
\toyPoint{16.20082209}{39.73518077}
\toyPoint{67.29742604}{38.07085837}
\toyPoint{21.71273816}{58.01386803}
\toyPoint{22.67658449}{19.89404586}
\toyPoint{18.66860820}{46.48985678}
\toyPoint{41.49024917}{12.31402859}
\toyPoint{57.68297995}{59.25258944}
\toyPoint{58.26003444}{58.95100071}
\toyPoint{57.81408710}{59.79195072}
\toyPoint{17.16025076}{38.53869811}
\toyPoint{38.67331232}{66.64328544}
\toyPoint{33.45367647}{17.67364287}
\toyPoint{22.98421368}{19.52241436}
\toyPoint{21.30248900}{20.25831715}
\toyPoint{60.27500368}{18.52251761}
\toyPoint{15.81832486}{39.15007238}
\toyPoint{16.32308775}{40.10235692}
\toyPoint{39.00983284}{65.82947208}
\toyPoint{56.95993639}{19.25159393}
\toyPoint{39.94201064}{12.90137506}
\toyPoint{59.64438500}{18.72086187}
\toyPoint{30.39422620}{61.64942218}
\toyPoint{15.33952190}{38.26242482}
\toyPoint{66.53637855}{37.53765272}
\toyPoint{60.22142257}{19.04364524}
\toyPoint{15.34173842}{40.43519216}
\toyPoint{33.34600049}{63.76849113}
\toyPoint{59.80075375}{19.93624903}
\toyPoint{21.57070068}{28.10882107}
\toyPoint{22.13086436}{22.36560668}
\toyPoint{65.21932817}{38.77793212}
\toyPoint{60.14586080}{17.49562571}
\toyPoint{41.37438505}{64.12508842}
\toyPoint{40.07385938}{13.27170218}
\toyPoint{68.08608394}{39.29448385}
\toyPoint{40.85911366}{12.55228719}
\toyPoint{16.50118643}{39.04260097}
\toyPoint{20.63681203}{55.59373948}
\toyPoint{32.98521626}{17.75045364}
\toyPoint{59.10975825}{57.56040358}
\toyPoint{58.70164102}{18.97814166}
\toyPoint{67.30180679}{40.25689965}
\toyPoint{45.10493555}{63.36926922}
\toyPoint{22.12410558}{20.71965402}
\toyPoint{14.52640072}{38.76942596}
\toyPoint{41.76524578}{12.20166114}
\toyPoint{50.43285862}{18.66674700}
\toyPoint{22.31923811}{57.37872554}
\toyPoint{57.61235422}{59.52234238}
\toyPoint{39.08801202}{65.93030622}
\toyPoint{60.24470760}{17.36787642}
\toyPoint{21.45299266}{20.27263918}
\toyPoint{38.96567349}{11.75293276}
\toyPoint{39.15408569}{65.88423145}
\toyPoint{22.20705986}{20.80074864}
\toyPoint{16.03956192}{39.51125537}
\toyPoint{63.57083751}{31.24180271}
\toyPoint{41.06685258}{66.65605853}
\toyPoint{66.58231489}{38.86979865}
\toyPoint{21.72242103}{28.18141030}
\toyPoint{39.26794460}{64.94114445}
\toyPoint{17.20628861}{39.73476411}
\toyPoint{22.15458316}{20.71756055}
\toyPoint{15.96616591}{39.02689688}
\toyPoint{55.48862303}{57.19201150}
\toyPoint{17.10578826}{40.12607649}
\toyPoint{23.05146463}{22.89369306}
\toyPoint{39.60943225}{65.90284348}
\toyPoint{59.98436989}{20.37315338}
\toyPoint{57.20482457}{59.30329261}
\toyPoint{67.00601086}{37.78707854}
\toyPoint{59.13655035}{18.59473536}
\toyPoint{17.29179167}{39.17399230}
\toyPoint{33.49739013}{17.00205311}
\toyPoint{40.85675447}{12.56436502}
\toyPoint{22.16276938}{58.11588041}
\toyPoint{66.56602860}{38.98054523}
\toyPoint{58.32592718}{57.91352457}
\toyPoint{15.96120681}{38.92912392}
\toyPoint{22.31941039}{54.26229016}
\toyPoint{22.59822015}{21.32151173}
\toyPoint{40.54623437}{66.25634593}
\toyPoint{39.92786444}{66.36429571}
\toyPoint{60.06737494}{17.81349767}
\toyPoint{37.70536461}{63.96971180}
\toyPoint{58.14394151}{57.66273283}
\toyPoint{16.29197182}{40.23479229}
\toyPoint{57.62689314}{60.12166823}
\toyPoint{45.74914409}{15.70330558}
\toyPoint{21.99026969}{58.03800983}
\toyPoint{21.78437602}{20.44757228}
\toyPoint{55.54375156}{18.86034904}
\toyPoint{45.78865774}{60.73039855}
\toyPoint{22.77363470}{21.61808137}
\toyPoint{24.69524230}{58.88257765}
\toyPoint{20.53728688}{44.85122281}
\toyPoint{40.96937149}{66.30948405}
\toyPoint{16.85591021}{40.16087137}
\toyPoint{63.20984564}{27.34198001}
\toyPoint{39.25355565}{11.99244961}
\toyPoint{56.40662993}{19.21680481}
\toyPoint{41.76523232}{12.33663990}
\toyPoint{66.46624965}{37.76080808}
\toyPoint{40.01914405}{11.74531260}
\toyPoint{57.49905771}{60.05109633}
\toyPoint{21.43435601}{20.82942809}
\toyPoint{47.90348822}{15.79884222}
\toyPoint{57.39910956}{60.21586049}
\toyPoint{59.14581330}{18.14670224}
\toyPoint{37.11509251}{12.93162192}
\toyPoint{56.62392001}{19.87631675}
\toyPoint{39.48911609}{65.77442815}
\toyPoint{40.68441572}{66.52150431}
\toyPoint{27.30267094}{59.95987738}
\toyPoint{59.25974508}{58.24525556}
\toyPoint{22.20279448}{58.05502830}
\toyPoint{39.10926857}{11.89637153}
\toyPoint{30.79802575}{60.96548850}
\toyPoint{63.21565536}{31.01633872}
\toyPoint{16.98579911}{39.12065902}
\toyPoint{40.52969513}{12.70744078}
\toyPoint{49.51849722}{17.33078157}
\toyPoint{41.99611745}{66.37723800}
\toyPoint{16.24933797}{39.34632980}
\toyPoint{22.66832444}{58.11851686}
\toyPoint{58.08781932}{60.18822547}
\toyPoint{40.12220875}{12.19279505}
\toyPoint{22.62393552}{23.26889315}
\toyPoint{57.29756171}{59.33479002}
\toyPoint{54.71375804}{58.05152124}
\toyPoint{39.78726814}{66.42409725}
\toyPoint{57.53119961}{59.29910875}
\toyPoint{57.80011731}{60.11353585}
\toyPoint{60.22355141}{18.29570001}
\toyPoint{60.31853276}{17.74416862}
\toyPoint{44.04456623}{61.39345138}
\toyPoint{15.98042027}{39.75145707}
\toyPoint{63.36534069}{42.95943887}
\toyPoint{39.01891976}{66.67850371}
\toyPoint{22.31630018}{58.04233674}
\toyPoint{16.66209590}{39.12484769}
\toyPoint{49.32997888}{59.85168303}
\toyPoint{16.90616885}{37.70953040}
\toyPoint{16.26569040}{39.35757403}
\toyPoint{22.20338052}{57.31721355}
\toyPoint{22.55340207}{57.44765466}
\toyPoint{57.46100303}{59.75600181}
\toyPoint{22.49354670}{57.63450253}
\toyPoint{35.68889949}{13.92702410}
\toyPoint{66.77355428}{38.44491059}
\toyPoint{16.50493037}{40.42514724}
\toyPoint{39.15568944}{12.12618551}
\toyPoint{57.59814447}{60.36118661}
\toyPoint{59.55947415}{58.89071003}
\toyPoint{60.67515004}{20.71780359}
\toyPoint{14.14263756}{38.28620226}
\toyPoint{38.51410120}{11.98802271}
\toyPoint{42.64484306}{14.51680553}
\toyPoint{20.87379702}{27.60013273}
\toyPoint{22.19697245}{58.03813442}
\toyPoint{40.28131811}{66.19166836}
\toyPoint{38.69960316}{12.18915878}
\toyPoint{60.17400649}{19.30842830}
\toyPoint{49.97045425}{17.56227832}
\toyPoint{16.27353514}{39.43285950}
\toyPoint{40.40146151}{12.56145477}
\toyPoint{15.67805475}{39.01728303}
\toyPoint{57.29484527}{58.04654983}
\toyPoint{60.80325927}{19.82503060}
\toyPoint{53.38530971}{18.03763574}
\toyPoint{58.02063450}{58.98611746}
\toyPoint{23.10312302}{55.73035948}
\toyPoint{28.34822562}{60.15213659}
\toyPoint{23.01990724}{58.29661862}
\toyPoint{26.77559668}{58.74235676}
\toyPoint{66.13515854}{37.42224755}
\toyPoint{59.02359532}{54.83350569}
\toyPoint{21.59498553}{21.88847726}
\toyPoint{59.25386767}{18.92738927}
\toyPoint{27.80373758}{60.41072076}
\toyPoint{57.80830660}{59.03381809}
\toyPoint{66.17150276}{39.87268460}
\toyPoint{40.50687554}{66.23450679}
\toyPoint{67.05362689}{38.17480887}
\toyPoint{42.04312340}{12.08794009}
\toyPoint{66.58774161}{38.86871653}
\toyPoint{22.65341943}{21.43586497}
\toyPoint{66.59871809}{37.39972718}
\toyPoint{66.69076304}{38.48612009}
\toyPoint{21.80527687}{57.70459606}
\toyPoint{59.70850268}{17.16197968}
\toyPoint{22.14841966}{59.37581955}
\toyPoint{40.17525357}{66.28361487}
\toyPoint{38.94681679}{64.82216743}
\toyPoint{33.93321276}{62.46202807}
\toyPoint{21.30026018}{20.24985252}
\toyPoint{66.89684899}{38.03352356}
\toyPoint{57.99709874}{58.98129986}
\toyPoint{59.29462648}{17.47294672}
\toyPoint{57.42561863}{60.15306258}
\toyPoint{22.22718547}{21.32465578}
\toyPoint{16.33646073}{38.40475994}
\toyPoint{63.24337036}{27.37399655}
\toyPoint{15.96622744}{39.49477027}
\toyPoint{58.08476756}{57.90149597}
\toyPoint{60.81524941}{19.54935412}
\toyPoint{17.99544181}{39.18275649}
\toyPoint{65.07463271}{32.17224275}
\toyPoint{27.55975539}{59.54147431}
\toyPoint{20.81321870}{58.42951929}
\toyPoint{68.12730420}{38.65382333}
\toyPoint{40.92973421}{12.33683678}
\toyPoint{66.76039973}{38.04701382}
\toyPoint{22.60430059}{23.44234190}
\toyPoint{56.92913578}{59.34629563}
\toyPoint{21.24452406}{23.94821690}
\toyPoint{22.69969571}{21.43251019}
\toyPoint{51.23860421}{17.48681807}
\toyPoint{60.21721563}{17.55574719}
\toyPoint{40.50407062}{14.28351525}
\toyPoint{59.79729899}{18.99585693}
\toyPoint{66.77475099}{38.03214112}
\toyPoint{67.89176510}{37.48270089}
\toyPoint{52.25486417}{17.54079911}
\toyPoint{60.83425983}{20.18966952}
\toyPoint{66.72264653}{38.26958141}
\toyPoint{57.67993742}{59.58134405}
\toyPoint{55.97212515}{58.46784930}
\toyPoint{29.24367812}{59.84691159}
\toyPoint{66.73302620}{38.34089125}
\toyPoint{22.39615810}{21.05156652}
\toyPoint{67.23982719}{40.67485052}
\toyPoint{67.16297334}{38.04664158}
\toyPoint{58.79104030}{58.90671023}
\toyPoint{41.69430414}{12.24461956}
\toyPoint{40.14106776}{66.38521502}
\toyPoint{22.92992653}{58.27477025}
\toyPoint{21.41102176}{20.93869302}
\toyPoint{59.47113622}{19.13435505}
\toyPoint{57.57323819}{59.89883761}
\toyPoint{58.43080674}{57.35043064}
\toyPoint{21.90935043}{57.48508484}
\toyPoint{39.23676127}{66.09914964}
\toyPoint{37.11226763}{13.67312524}
\toyPoint{38.69439948}{11.77240310}
\toyPoint{22.08155940}{57.83023034}


==> figures/toy8_native_data/nextgan_20000.tex <==
% Generated from original vector marker centers; do not edit by hand.
\toyPoint{61.40488471}{34.28621146}
\toyPoint{58.07553076}{21.85764743}
\toyPoint{24.39300137}{57.88927355}
\toyPoint{22.49876115}{22.92053130}
\toyPoint{15.96987140}{37.57749554}
\toyPoint{38.75408065}{65.07145174}
\toyPoint{22.50990375}{23.04099575}
\toyPoint{40.87818965}{65.61825629}
\toyPoint{59.65988836}{52.41885539}
\toyPoint{42.91505629}{63.41075251}
\toyPoint{57.88003829}{21.38121943}
\toyPoint{42.79555186}{63.74766411}
\toyPoint{19.77877432}{51.62428471}
\toyPoint{57.23513296}{21.91373118}
\toyPoint{64.80546428}{40.72696002}
\toyPoint{66.10756043}{41.20883161}
\toyPoint{21.44406503}{22.56815480}
\toyPoint{65.74303535}{41.56020762}
\toyPoint{16.02583670}{37.88219256}
\toyPoint{42.59119695}{66.86861100}
\toyPoint{58.29777379}{57.29604813}
\toyPoint{65.94814301}{41.80569772}
\toyPoint{57.60971008}{22.01370239}
\toyPoint{15.51822816}{37.99207372}
\toyPoint{64.44606750}{40.53800965}
\toyPoint{21.69167888}{22.42247643}
\toyPoint{29.46123815}{21.56960241}
\toyPoint{19.24228022}{57.51555320}
\toyPoint{58.40594353}{56.69048032}
\toyPoint{58.18302216}{57.21877436}
\toyPoint{57.31919473}{21.25345938}
\toyPoint{40.50758969}{65.54037802}
\toyPoint{13.72769387}{39.46065165}
\toyPoint{22.99469025}{21.80839631}
\toyPoint{40.87564299}{65.88422837}
\toyPoint{60.12354020}{58.87454217}
\toyPoint{37.31837588}{16.87286100}
\toyPoint{22.03305275}{22.61272830}
\toyPoint{14.16403986}{39.09931565}
\toyPoint{65.72947625}{42.38138630}
\toyPoint{38.54878995}{14.29444252}
\toyPoint{19.59100816}{57.43192980}
\toyPoint{40.51477316}{65.94146113}
\toyPoint{57.10589932}{21.87877132}
\toyPoint{40.63041213}{65.84734578}
\toyPoint{38.27961845}{14.28877277}
\toyPoint{22.65653887}{23.02946706}
\toyPoint{14.90718749}{38.70698058}
\toyPoint{17.54409082}{32.15451133}
\toyPoint{15.38676108}{38.35183986}
\toyPoint{19.63537401}{57.72922239}
\toyPoint{12.42650678}{38.45826424}
\toyPoint{15.01671853}{37.48216771}
\toyPoint{38.15430410}{15.43847945}
\toyPoint{57.25336659}{21.84368533}
\toyPoint{58.06446506}{57.25163306}
\toyPoint{23.18011530}{57.13729828}
\toyPoint{34.08306383}{18.84399199}
\toyPoint{64.86568113}{42.07704940}
\toyPoint{58.43286637}{57.32564126}
\toyPoint{58.21144935}{57.52744798}
\toyPoint{57.75815256}{21.13541142}
\toyPoint{16.17095824}{36.39321527}
\toyPoint{57.74145711}{22.16457213}
\toyPoint{58.35654013}{57.31547694}
\toyPoint{14.91570903}{38.69194406}
\toyPoint{25.58119958}{58.17441756}
\toyPoint{40.72986998}{65.46561456}
\toyPoint{15.71287309}{37.88957046}
\toyPoint{37.71004108}{13.62887167}
\toyPoint{22.12526229}{23.76029230}
\toyPoint{12.77221680}{37.96622876}
\toyPoint{58.38576255}{57.29238725}
\toyPoint{65.73204810}{41.02301115}
\toyPoint{19.40702285}{57.48103019}
\toyPoint{65.63062176}{41.56679048}
\toyPoint{40.83070301}{65.74204322}
\toyPoint{21.59964931}{22.30543906}
\toyPoint{57.85450905}{21.97397878}
\toyPoint{58.23789689}{57.48318672}
\toyPoint{21.61328993}{22.47003555}
\toyPoint{66.13364189}{41.80958183}
\toyPoint{32.39629469}{61.26247498}
\toyPoint{14.02971945}{39.10359296}
\toyPoint{57.31583226}{21.78124582}
\toyPoint{13.81095271}{37.29744850}
\toyPoint{14.92056816}{37.96527105}
\toyPoint{57.14312184}{58.28151980}
\toyPoint{36.29868154}{15.40003254}
\toyPoint{19.71447206}{57.58361017}
\toyPoint{21.69671489}{22.35360115}
\toyPoint{66.19977151}{43.55977204}
\toyPoint{12.61810918}{37.42367537}
\toyPoint{15.51414890}{38.02817202}
\toyPoint{23.60423580}{24.36049184}
\toyPoint{57.45690530}{22.32940243}
\toyPoint{66.53520030}{41.54963049}
\toyPoint{65.49864707}{41.48740786}
\toyPoint{22.16447676}{22.73196528}
\toyPoint{15.06353163}{37.84698159}
\toyPoint{41.08706893}{65.53621415}
\toyPoint{15.14022243}{37.85725590}
\toyPoint{59.78647940}{58.00073501}
\toyPoint{65.79593812}{41.05319167}
\toyPoint{21.60782937}{22.79214059}
\toyPoint{13.90452354}{38.89408071}
\toyPoint{13.97465244}{38.56319302}
\toyPoint{15.32351248}{38.06497501}
\toyPoint{22.17453803}{22.73210372}
\toyPoint{64.24676495}{44.21395417}
\toyPoint{59.49627938}{57.78567529}
\toyPoint{21.48025543}{57.11745877}
\toyPoint{14.31008277}{38.34227004}
\toyPoint{22.15500155}{23.61853630}
\toyPoint{40.99254664}{64.99806650}
\toyPoint{33.53829045}{19.22805509}
\toyPoint{20.53857896}{56.92299228}
\toyPoint{19.17949923}{57.62789603}
\toyPoint{19.46089775}{58.33485634}
\toyPoint{63.97156531}{42.94567347}
\toyPoint{15.41374237}{37.56806377}
\toyPoint{14.50107605}{39.20453588}
\toyPoint{24.67902214}{23.56769316}
\toyPoint{58.03262003}{57.47037365}
\toyPoint{65.40381493}{39.87940634}
\toyPoint{57.16089710}{21.72758010}
\toyPoint{19.47211881}{58.17094587}
\toyPoint{23.26548453}{21.78860449}
\toyPoint{57.45931256}{21.26688157}
\toyPoint{22.20076561}{22.41217521}
\toyPoint{41.68629423}{67.28506827}
\toyPoint{58.21639922}{53.63515392}
\toyPoint{21.60123210}{22.47533614}
\toyPoint{66.80198916}{41.14130483}
\toyPoint{15.31986544}{38.58858845}
\toyPoint{65.16680533}{40.39039201}
\toyPoint{65.31501093}{44.22397890}
\toyPoint{57.91325385}{57.68762373}
\toyPoint{57.44724858}{22.37990410}
\toyPoint{66.07587999}{41.77799002}
\toyPoint{39.82608663}{65.87925388}
\toyPoint{39.54841445}{14.38381103}
\toyPoint{20.03218405}{57.87913999}
\toyPoint{19.79940753}{56.94352704}
\toyPoint{15.37506011}{38.23649718}
\toyPoint{41.16780112}{65.00447304}
\toyPoint{21.69394309}{22.64902176}
\toyPoint{23.17323962}{24.04569164}
\toyPoint{58.19890699}{56.87956933}
\toyPoint{14.92768841}{38.45393329}
\toyPoint{19.37147848}{57.60785964}
\toyPoint{58.44473962}{59.14571331}
\toyPoint{21.82408887}{22.43209162}
\toyPoint{57.42991017}{58.07128383}
\toyPoint{22.57275397}{22.06368877}
\toyPoint{41.35034746}{66.40721106}
\toyPoint{38.62716467}{14.62725947}
\toyPoint{64.69809901}{40.83904372}
\toyPoint{15.29525142}{38.45542975}
\toyPoint{14.46307367}{43.22284679}
\toyPoint{62.50795364}{40.89543221}
\toyPoint{33.83289276}{62.92571375}
\toyPoint{38.37619066}{65.08628445}
\toyPoint{21.48550372}{57.00535436}
\toyPoint{19.74216554}{57.72644904}
\toyPoint{40.20791408}{14.81320596}
\toyPoint{20.96425456}{57.62464739}
\toyPoint{21.59769274}{22.31424978}
\toyPoint{36.22109475}{13.77798019}
\toyPoint{30.83171352}{60.96287204}
\toyPoint{19.41800087}{57.40018937}
\toyPoint{14.89058125}{37.35348436}
\toyPoint{19.14901395}{58.09551331}
\toyPoint{19.48851893}{57.70880453}
\toyPoint{14.27247724}{39.18980204}
\toyPoint{65.62906050}{41.55136422}
\toyPoint{19.64117450}{57.69964310}
\toyPoint{21.70753448}{22.24855085}
\toyPoint{13.15174841}{40.84222776}
\toyPoint{39.40034978}{14.41259661}
\toyPoint{58.00583101}{57.44859911}
\toyPoint{57.88888285}{58.04540849}
\toyPoint{58.08343549}{57.83462494}
\toyPoint{14.80892212}{37.80604859}
\toyPoint{40.13822163}{64.24545134}
\toyPoint{33.92778643}{19.14747423}
\toyPoint{21.52239861}{21.85559550}
\toyPoint{22.21616437}{22.73067782}
\toyPoint{57.51673760}{21.67439122}
\toyPoint{14.14648610}{39.20448473}
\toyPoint{15.31027179}{38.44242940}
\toyPoint{39.65747595}{64.49338513}
\toyPoint{57.36597400}{21.91502633}
\toyPoint{38.46655938}{15.48585861}
\toyPoint{57.05402713}{21.84639254}
\toyPoint{29.98420931}{59.84408440}
\toyPoint{14.29535312}{38.74795166}
\toyPoint{65.15997887}{40.90312179}
\toyPoint{57.64999667}{21.53195996}
\toyPoint{12.71121856}{37.80527142}
\toyPoint{38.87177906}{65.87973995}
\toyPoint{57.72099464}{21.65238442}
\toyPoint{21.97489554}{24.77411424}
\toyPoint{22.08892730}{22.53460392}
\toyPoint{65.30480969}{40.08649053}
\toyPoint{57.93068301}{21.32495111}
\toyPoint{38.79704733}{64.33404307}
\toyPoint{37.77946549}{14.73439863}
\toyPoint{66.21629777}{42.55018319}
\toyPoint{38.95633421}{14.77968739}
\toyPoint{15.47365773}{37.86944985}
\toyPoint{21.27654599}{58.39602378}
\toyPoint{35.99337578}{18.04656336}
\toyPoint{58.90402148}{58.01301279}
\toyPoint{57.44027599}{22.37046426}
\toyPoint{66.07339428}{42.21766599}
\toyPoint{38.86221943}{65.15649026}
\toyPoint{22.19883980}{22.68578283}
\toyPoint{13.49139183}{38.08631155}
\toyPoint{39.40034843}{14.38796413}
\toyPoint{54.54181979}{22.16145731}
\toyPoint{20.21598478}{57.51555935}
\toyPoint{57.39555021}{58.57178288}
\toyPoint{39.98884922}{65.34355194}
\toyPoint{57.99030304}{21.99176173}
\toyPoint{21.97361577}{22.59415626}
\toyPoint{38.94286202}{13.96584480}
\toyPoint{39.57838520}{64.45592573}
\toyPoint{21.96214399}{22.24976447}
\toyPoint{15.27973421}{38.48176116}
\toyPoint{61.69170841}{36.96773002}
\toyPoint{41.02533785}{65.54564322}
\toyPoint{65.30779070}{40.66585334}
\toyPoint{21.49577264}{25.98397624}
\toyPoint{39.30523336}{65.19725215}
\toyPoint{14.65594969}{38.62950377}
\toyPoint{22.14375281}{22.49725680}
\toyPoint{14.62371549}{38.52985538}
\toyPoint{54.58332154}{59.18407256}
\toyPoint{14.90538782}{38.75952342}
\toyPoint{22.22297699}{23.17832793}
\toyPoint{40.95030867}{65.59922280}
\toyPoint{57.43341415}{21.08301778}
\toyPoint{58.19361718}{57.00409766}
\toyPoint{65.62808837}{40.64491173}
\toyPoint{57.47834144}{22.03144996}
\toyPoint{15.68130801}{37.70235073}
\toyPoint{37.80122080}{17.09708521}
\toyPoint{39.16515947}{14.41784489}
\toyPoint{19.24367997}{57.85252017}
\toyPoint{65.07888117}{40.73488033}
\toyPoint{57.62711771}{58.60444930}
\toyPoint{14.98626863}{37.15018176}
\toyPoint{20.14804010}{53.74725219}
\toyPoint{22.17692529}{22.77770627}
\toyPoint{42.62652828}{67.10011698}
\toyPoint{41.18855594}{65.15961432}
\toyPoint{57.87961068}{20.78817552}
\toyPoint{19.82778088}{57.41389921}
\toyPoint{60.15772943}{57.29381777}
\toyPoint{14.81527790}{38.89885370}
\toyPoint{58.32923735}{57.48011804}
\toyPoint{48.80756994}{18.96049100}
\toyPoint{20.54036171}{57.80907877}
\toyPoint{22.08734451}{22.69601791}
\toyPoint{57.64929679}{22.02132102}
\toyPoint{39.53634835}{64.73233592}
\toyPoint{22.32636298}{23.02689368}
\toyPoint{20.56018430}{57.43195288}
\toyPoint{13.46806065}{37.83089661}
\toyPoint{42.24435868}{67.12248525}
\toyPoint{14.56587669}{38.85817795}
\toyPoint{61.42834971}{36.58340562}
\toyPoint{39.36715788}{13.99455655}
\toyPoint{59.11460815}{22.84306372}
\toyPoint{40.41261738}{14.26961007}
\toyPoint{65.17641591}{41.93171155}
\toyPoint{38.30026281}{13.99418123}
\toyPoint{57.69744196}{57.72369262}
\toyPoint{21.52615793}{22.27012850}
\toyPoint{56.39540580}{21.53477023}
\toyPoint{58.65711058}{58.10714814}
\toyPoint{58.03110953}{20.84976289}
\toyPoint{39.38705121}{14.10674557}
\toyPoint{59.03873105}{21.97733356}
\toyPoint{40.42705296}{64.84448494}
\toyPoint{40.99791519}{65.42747836}
\toyPoint{21.67951953}{57.10305368}
\toyPoint{57.56666860}{59.15004792}
\toyPoint{19.31495636}{58.33944782}
\toyPoint{39.47812519}{14.32915318}
\toyPoint{19.41766401}{57.40266738}
\toyPoint{61.47681329}{35.48296390}
\toyPoint{14.69170017}{37.67498643}
\toyPoint{38.80769618}{15.00668033}
\toyPoint{55.60690788}{22.02296226}
\toyPoint{20.55400849}{57.38339547}
\toyPoint{13.41192922}{39.39984876}
\toyPoint{18.87798894}{57.29794625}
\toyPoint{59.25581809}{57.49457544}
\toyPoint{39.85880006}{14.44369255}
\toyPoint{22.57292009}{22.09804873}
\toyPoint{58.36496323}{57.54613538}
\toyPoint{53.10381120}{59.99963483}
\toyPoint{42.02089106}{64.75012656}
\toyPoint{58.21091867}{57.11773565}
\toyPoint{58.17247176}{57.96801629}
\toyPoint{57.45742829}{21.73310218}
\toyPoint{58.00155024}{22.01093366}
\toyPoint{43.06528345}{63.72526200}
\toyPoint{15.32628121}{38.42161354}
\toyPoint{61.99807013}{44.86081723}
\toyPoint{41.05643734}{64.56001774}
\toyPoint{19.96399941}{57.53243016}
\toyPoint{14.34523644}{38.19023782}
\toyPoint{41.42641289}{63.95665415}
\toyPoint{14.06221821}{39.94911691}
\toyPoint{14.85764565}{37.59562150}
\toyPoint{19.43099545}{57.53180565}
\toyPoint{19.80613709}{57.44647026}
\toyPoint{58.33511630}{57.46154293}
\toyPoint{19.64711497}{57.28632527}
\toyPoint{38.62666765}{15.60961170}
\toyPoint{65.85566121}{41.01116771}
\toyPoint{14.82702040}{38.80750093}
\toyPoint{37.02772517}{13.55855511}
\toyPoint{57.77413430}{58.70727231}
\toyPoint{58.55083435}{58.94294985}
\toyPoint{59.48312790}{24.39874341}
\toyPoint{13.97884861}{38.38219208}
\toyPoint{38.45807072}{13.70712526}
\toyPoint{40.74881162}{16.50899118}
\toyPoint{19.13900037}{28.67395616}
\toyPoint{19.47247567}{57.54568008}
\toyPoint{42.37135541}{66.82546493}
\toyPoint{38.30467855}{14.23433335}
\toyPoint{57.95098705}{21.58337224}
\toyPoint{57.34984306}{21.96256084}
\toyPoint{14.89164260}{38.57829030}
\toyPoint{38.75548232}{15.40825413}
\toyPoint{14.08424501}{39.04807450}
\toyPoint{57.10743904}{57.87985986}
\toyPoint{57.39887884}{21.16666732}
\toyPoint{58.74456867}{22.35314892}
\toyPoint{58.44570714}{57.09982657}
\toyPoint{20.26655720}{57.49586136}
\toyPoint{19.79182428}{57.55493226}
\toyPoint{18.94750872}{57.43557069}
\toyPoint{19.38519293}{57.62022203}
\toyPoint{65.62186487}{40.04479294}
\toyPoint{57.46601905}{57.33649315}
\toyPoint{22.58360432}{22.85529690}
\toyPoint{57.54287289}{22.03880710}
\toyPoint{25.58364222}{57.76636954}
\toyPoint{57.40343494}{58.84155427}
\toyPoint{66.40513143}{39.47550273}
\toyPoint{42.37621723}{67.00350977}
\toyPoint{66.46389008}{41.59779701}
\toyPoint{39.57218882}{14.34559791}
\toyPoint{64.97399238}{40.90587591}
\toyPoint{22.06906780}{22.69189250}
\toyPoint{65.75566846}{40.20637132}
\toyPoint{65.07754757}{41.05934787}
\toyPoint{19.56548506}{57.72460322}
\toyPoint{57.38472600}{21.38697070}
\toyPoint{20.06910816}{58.30474638}
\toyPoint{41.19053635}{65.72974236}
\toyPoint{39.47580638}{64.75307834}
\toyPoint{19.44897067}{57.36417124}
\toyPoint{22.17044184}{22.68897149}
\toyPoint{65.66175307}{41.52038730}
\toyPoint{58.30667527}{57.44244637}
\toyPoint{58.02741943}{21.53190459}
\toyPoint{58.43374314}{57.17610974}
\toyPoint{22.69537187}{23.71486971}
\toyPoint{15.39987410}{37.81377296}
\toyPoint{62.21243920}{37.10018923}
\toyPoint{15.41050757}{38.28258003}
\toyPoint{57.12846141}{58.64705240}
\toyPoint{57.23742947}{21.54037999}
\toyPoint{14.65731559}{38.65130003}
\toyPoint{63.30927234}{42.85101302}
\toyPoint{19.44819235}{57.41336546}
\toyPoint{20.08920608}{57.99310715}
\toyPoint{65.78501394}{41.62304813}
\toyPoint{38.76318555}{15.44560740}
\toyPoint{65.07448197}{41.05271272}
\toyPoint{22.25889975}{22.36524367}
\toyPoint{58.24475104}{57.46282731}
\toyPoint{21.01649592}{23.36098271}
\toyPoint{21.69627036}{22.65776480}
\toyPoint{58.95174211}{22.57894824}
\toyPoint{57.42079489}{21.89539756}
\toyPoint{38.53153690}{15.46544998}
\toyPoint{58.07387721}{21.69208650}
\toyPoint{65.86169089}{41.58948350}
\toyPoint{65.08374184}{45.27307487}
\toyPoint{59.70474336}{22.19750620}
\toyPoint{57.45018652}{21.11553500}
\toyPoint{65.48115023}{41.19740646}
\toyPoint{57.54152237}{58.82611552}
\toyPoint{54.53785281}{58.90447524}
\toyPoint{22.36480067}{58.61979884}
\toyPoint{65.83640929}{41.13514191}
\toyPoint{22.21347101}{22.76018173}
\toyPoint{66.22667128}{42.07893137}
\toyPoint{65.64074609}{41.75042345}
\toyPoint{57.93365632}{59.33210281}
\toyPoint{39.44084421}{14.39721169}
\toyPoint{42.41619714}{66.66609672}
\toyPoint{18.92487588}{57.34908935}
\toyPoint{22.56470773}{23.00972600}
\toyPoint{57.80838505}{21.87746079}
\toyPoint{58.11049984}{57.40670050}
\toyPoint{59.66199567}{57.78535381}
\toyPoint{19.56611418}{57.76014297}
\toyPoint{40.64105334}{65.37898864}
\toyPoint{41.43246939}{14.21702570}
\toyPoint{38.88753218}{13.74356793}
\toyPoint{20.22088543}{57.62605175}


==> figures/toy8_native_data/nextgan_30000.tex <==
% Generated from original vector marker centers; do not edit by hand.
\toyPoint{62.86975922}{29.68598535}
\toyPoint{57.78355722}{22.11652694}
\toyPoint{22.70796807}{57.67947751}
\toyPoint{17.63741862}{17.82482024}
\toyPoint{11.38420536}{37.02405526}
\toyPoint{38.19466760}{63.49498041}
\toyPoint{17.43020058}{18.32143076}
\toyPoint{39.56937894}{66.08068835}
\toyPoint{56.85133442}{52.35846243}
\toyPoint{42.95244205}{60.53094372}
\toyPoint{59.54380620}{20.11900071}
\toyPoint{39.62751942}{63.97747809}
\toyPoint{23.35931532}{55.38794579}
\toyPoint{59.16612348}{19.20767107}
\toyPoint{64.47685580}{41.28374148}
\toyPoint{66.81361783}{35.81351703}
\toyPoint{18.19598259}{19.59054670}
\toyPoint{65.91433679}{41.07791030}
\toyPoint{12.06177250}{37.79233759}
\toyPoint{40.56639535}{65.27973267}
\toyPoint{56.14487402}{60.07624718}
\toyPoint{66.13790881}{40.50520383}
\toyPoint{59.32864343}{20.76028670}
\toyPoint{12.05367242}{37.53172609}
\toyPoint{60.16161026}{44.60543440}
\toyPoint{17.65595067}{19.25673608}
\toyPoint{31.27577966}{16.59317293}
\toyPoint{23.37753665}{58.06842742}
\toyPoint{55.91468780}{58.29056432}
\toyPoint{56.63104334}{60.27642804}
\toyPoint{58.85026809}{19.99231892}
\toyPoint{39.60366593}{64.17073557}
\toyPoint{13.18619759}{39.40276747}
\toyPoint{19.42089112}{20.38186258}
\toyPoint{39.73059104}{66.69949378}
\toyPoint{56.79152827}{62.30557319}
\toyPoint{38.00217825}{11.79663566}
\toyPoint{16.86387185}{18.76269894}
\toyPoint{12.95483005}{38.55961559}
\toyPoint{65.70825546}{41.31831679}
\toyPoint{38.84535170}{10.86219172}
\toyPoint{23.37800272}{59.08410442}
\toyPoint{39.48689082}{65.49401099}
\toyPoint{58.38009281}{21.43502205}
\toyPoint{40.08002505}{63.43356686}
\toyPoint{38.64405644}{10.73415018}
\toyPoint{17.84690395}{18.10597112}
\toyPoint{12.01204915}{37.78859942}
\toyPoint{20.16750582}{22.84790439}
\toyPoint{11.81342033}{37.90039620}
\toyPoint{22.29226605}{58.51322420}
\toyPoint{14.29046169}{40.46612817}
\toyPoint{11.35999433}{36.95618249}
\toyPoint{37.64145863}{10.36996349}
\toyPoint{59.16639420}{19.24191106}
\toyPoint{56.36469595}{60.33020912}
\toyPoint{22.06341497}{57.78116072}
\toyPoint{35.22488194}{13.39320952}
\toyPoint{66.00542499}{40.93020903}
\toyPoint{56.10284928}{59.51079369}
\toyPoint{56.26382951}{59.95979278}
\toyPoint{58.36474019}{21.77268890}
\toyPoint{19.13270304}{23.57907264}
\toyPoint{59.49321993}{20.10513244}
\toyPoint{55.65785869}{58.85599475}
\toyPoint{12.01873718}{37.77309299}
\toyPoint{22.53504076}{57.28793421}
\toyPoint{39.59136075}{64.38761650}
\toyPoint{11.56321003}{37.61964256}
\toyPoint{39.17997141}{11.04714609}
\toyPoint{19.70990981}{21.51168054}
\toyPoint{13.46848826}{38.33400423}
\toyPoint{56.12584206}{59.79177075}
\toyPoint{65.51366591}{40.25269855}
\toyPoint{23.56990968}{58.71794578}
\toyPoint{65.87058467}{40.96349976}
\toyPoint{39.65301906}{66.23213799}
\toyPoint{17.49096347}{18.31027738}
\toyPoint{57.93260728}{21.62797190}
\toyPoint{56.19308687}{60.06689041}
\toyPoint{17.98617578}{19.64463234}
\toyPoint{66.24219464}{41.08132622}
\toyPoint{25.85733137}{57.79447832}
\toyPoint{13.30150912}{38.80694410}
\toyPoint{54.59014493}{18.26670370}
\toyPoint{13.74813018}{37.69285513}
\toyPoint{9.29333287}{35.87787967}
\toyPoint{52.00529145}{61.55786176}
\toyPoint{37.18130538}{9.05265008}
\toyPoint{23.40766199}{58.11044601}
\toyPoint{17.37913901}{18.70969003}
\toyPoint{65.24485896}{41.74118530}
\toyPoint{13.50971776}{37.73706698}
\toyPoint{10.49419341}{36.47896444}
\toyPoint{25.30003948}{21.92923607}
\toyPoint{59.39751102}{20.24054343}
\toyPoint{64.78900417}{41.65705565}
\toyPoint{65.65393755}{40.58452799}
\toyPoint{16.59070107}{18.83595651}
\toyPoint{11.49151833}{37.72104890}
\toyPoint{39.94630112}{66.13511547}
\toyPoint{11.30874203}{37.32877535}
\toyPoint{55.56367566}{58.15697762}
\toyPoint{64.59543751}{42.15486653}
\toyPoint{18.70225137}{20.21705535}
\toyPoint{13.58998022}{38.81318490}
\toyPoint{13.67697685}{38.62315357}
\toyPoint{11.39571098}{37.56764116}
\toyPoint{16.81495913}{18.58265446}
\toyPoint{64.48665711}{41.67849122}
\toyPoint{55.83579279}{57.24451896}
\toyPoint{21.69026529}{58.43148047}
\toyPoint{10.60255850}{37.27967958}
\toyPoint{19.20891393}{21.00113561}
\toyPoint{39.99780588}{63.94128307}
\toyPoint{33.55621184}{13.59221366}
\toyPoint{23.39146952}{57.99725871}
\toyPoint{23.23664050}{58.08184808}
\toyPoint{22.83079978}{58.72370320}
\toyPoint{66.08860077}{40.64173057}
\toyPoint{11.83271531}{37.08202981}
\toyPoint{11.62183331}{38.07674904}
\toyPoint{22.07843996}{18.32527007}
\toyPoint{56.25268536}{60.33069211}
\toyPoint{62.85699998}{41.89762808}
\toyPoint{57.61642425}{22.42085826}
\toyPoint{22.38251748}{58.71908711}
\toyPoint{19.77508883}{20.83991697}
\toyPoint{58.02617811}{22.08685998}
\toyPoint{19.05860255}{20.84585282}
\toyPoint{35.39760159}{62.88389052}
\toyPoint{55.90621394}{50.27501322}
\toyPoint{18.02596554}{19.71537190}
\toyPoint{65.28037256}{41.32813165}
\toyPoint{12.67575110}{38.38650400}
\toyPoint{62.76058351}{41.48668885}
\toyPoint{64.94570055}{41.32421399}
\toyPoint{55.26992398}{57.24707542}
\toyPoint{59.41432030}{20.05550907}
\toyPoint{64.97683956}{41.19890100}
\toyPoint{30.12717739}{59.42041612}
\toyPoint{38.74426876}{11.49946151}
\toyPoint{21.88971704}{59.06264059}
\toyPoint{23.31132858}{58.31971753}
\toyPoint{11.49596368}{37.70030764}
\toyPoint{40.14576772}{64.68816234}
\toyPoint{18.18899001}{19.64302955}
\toyPoint{21.04281425}{19.27159340}
\toyPoint{53.46548757}{58.91775593}
\toyPoint{12.06279078}{37.99941759}
\toyPoint{23.54243463}{58.67147723}
\toyPoint{55.73441567}{56.71058132}
\toyPoint{17.23039965}{18.82557684}
\toyPoint{53.12916971}{61.28929784}
\toyPoint{18.42251562}{19.50735554}
\toyPoint{40.95305164}{64.86850216}
\toyPoint{39.09358236}{11.39285611}
\toyPoint{63.73993627}{42.46794781}
\toyPoint{11.64094063}{37.76546167}
\toyPoint{17.22312866}{45.24576441}
\toyPoint{62.91060263}{35.16952922}
\toyPoint{32.91971345}{58.98957991}
\toyPoint{38.00468626}{63.12125391}
\toyPoint{21.35930953}{57.05552224}
\toyPoint{22.74777012}{58.58125656}
\toyPoint{39.67693225}{10.65270024}
\toyPoint{22.27075915}{57.82616800}
\toyPoint{17.47040256}{18.60420442}
\toyPoint{39.31914287}{9.30807483}
\toyPoint{26.10958438}{57.57119856}
\toyPoint{23.15045141}{58.87830919}
\toyPoint{11.15985809}{36.89033358}
\toyPoint{22.91783948}{58.39635910}
\toyPoint{23.78662909}{58.45504392}
\toyPoint{12.58096203}{38.51478194}
\toyPoint{65.76665263}{41.02538822}
\toyPoint{23.46376880}{58.75572051}
\toyPoint{19.06292177}{20.35814531}
\toyPoint{15.84977458}{43.27191891}
\toyPoint{38.81459071}{11.36788830}
\toyPoint{56.32781336}{60.07390145}
\toyPoint{55.10013457}{57.69497471}
\toyPoint{55.32621999}{58.51523768}
\toyPoint{10.28594786}{36.86805183}
\toyPoint{39.40364111}{64.20754740}
\toyPoint{29.24445414}{14.16184948}
\toyPoint{19.11177451}{20.19237211}
\toyPoint{17.44811120}{17.76232227}
\toyPoint{57.71806132}{21.07597751}
\toyPoint{12.89973228}{38.67628303}
\toyPoint{12.17934516}{38.07851103}
\toyPoint{38.99388532}{63.49915812}
\toyPoint{60.02162318}{18.73313658}
\toyPoint{37.80699668}{10.91041688}
\toyPoint{58.39595149}{21.23971108}
\toyPoint{24.26714866}{57.23300103}
\toyPoint{13.02207639}{38.17291440}
\toyPoint{64.40853580}{40.58685469}
\toyPoint{58.08176810}{21.07283038}
\toyPoint{13.31774312}{38.20124468}
\toyPoint{37.56313235}{62.20296091}
\toyPoint{58.25530760}{20.83156155}
\toyPoint{18.29975467}{19.02878177}
\toyPoint{19.33103961}{19.82639959}
\toyPoint{63.67403123}{40.78791298}
\toyPoint{57.67238955}{21.74488775}
\toyPoint{39.67014443}{64.48935201}
\toyPoint{38.38030550}{11.77181551}
\toyPoint{66.09664548}{41.42787474}
\toyPoint{38.15412779}{11.14303650}
\toyPoint{11.28572464}{37.46487083}
\toyPoint{22.26572006}{55.65627283}
\toyPoint{37.24483625}{12.98720267}
\toyPoint{55.37424980}{57.40953230}
\toyPoint{59.41044254}{20.08908764}
\toyPoint{66.07532932}{40.93176125}
\toyPoint{39.34411010}{61.82382614}
\toyPoint{16.50441047}{18.86881367}
\toyPoint{13.86482916}{38.29937931}
\toyPoint{38.57991338}{11.37103235}
\toyPoint{52.03780251}{19.35764713}
\toyPoint{22.99601155}{58.34031843}
\toyPoint{54.23791455}{60.46177310}
\toyPoint{38.80144308}{62.89481163}
\toyPoint{57.87962760}{21.46958659}
\toyPoint{17.24229290}{18.12460161}
\toyPoint{39.87782182}{11.07085259}
\toyPoint{39.04181726}{63.70593932}
\toyPoint{15.73390930}{19.14222902}
\toyPoint{11.63240064}{37.80671000}
\toyPoint{63.38826887}{32.06187648}
\toyPoint{39.88733549}{64.56780864}
\toyPoint{65.05671132}{40.96134188}
\toyPoint{20.44433748}{19.82296944}
\toyPoint{38.00258087}{62.74427568}
\toyPoint{13.45127290}{38.63645713}
\toyPoint{16.45133849}{18.87728753}
\toyPoint{12.52382771}{37.73830541}
\toyPoint{53.23085600}{57.17365173}
\toyPoint{12.92949000}{38.53963823}
\toyPoint{19.42733303}{20.89208449}
\toyPoint{39.80147625}{67.02449060}
\toyPoint{58.42601838}{20.50866127}
\toyPoint{56.54254544}{60.06763797}
\toyPoint{64.87775280}{40.43865543}
\toyPoint{59.33156598}{20.47425670}
\toyPoint{10.92710618}{36.55218470}
\toyPoint{38.69737721}{12.24964942}
\toyPoint{39.00956058}{11.05451092}
\toyPoint{23.06151821}{58.24554320}
\toyPoint{64.97331404}{40.49314427}
\toyPoint{53.39522792}{60.55012180}
\toyPoint{9.73672375}{34.09076129}
\toyPoint{23.33032208}{55.92413225}
\toyPoint{16.67921435}{18.80919826}
\toyPoint{40.39627139}{65.35307023}
\toyPoint{40.09252141}{65.26394321}
\toyPoint{57.67069447}{21.85986857}
\toyPoint{23.31761206}{59.09120621}
\toyPoint{55.62488310}{59.69202103}
\toyPoint{11.93421395}{38.09164270}
\toyPoint{55.64848654}{59.01890386}
\toyPoint{46.11009444}{14.81087562}
\toyPoint{22.90642923}{58.55730857}
\toyPoint{16.92199984}{18.50440241}
\toyPoint{60.37574091}{18.99755509}
\toyPoint{39.18891807}{62.24245225}
\toyPoint{16.93661874}{18.67710513}
\toyPoint{22.20116246}{58.53740907}
\toyPoint{16.10840028}{31.59450377}
\toyPoint{37.82806885}{64.09792715}
\toyPoint{12.94774517}{38.55107348}
\toyPoint{61.34451251}{30.70281829}
\toyPoint{39.89254302}{11.09751855}
\toyPoint{59.69394684}{21.47106632}
\toyPoint{39.39151983}{10.54480583}
\toyPoint{65.65925967}{40.93117039}
\toyPoint{39.39368406}{10.09979371}
\toyPoint{54.97444184}{59.26177394}
\toyPoint{17.61338295}{18.30601046}
\toyPoint{53.57804883}{17.21365190}
\toyPoint{56.48847672}{61.18883441}
\toyPoint{57.69648829}{22.50899930}
\toyPoint{39.57475547}{11.44041677}
\toyPoint{59.93011044}{20.89371804}
\toyPoint{40.81329624}{64.86898207}
\toyPoint{39.73022380}{64.48426831}
\toyPoint{22.08717069}{58.17836454}
\toyPoint{53.65592557}{57.52857854}
\toyPoint{22.63420905}{58.68101397}
\toyPoint{39.45217409}{12.44456507}
\toyPoint{23.16785597}{58.85237386}
\toyPoint{63.12466406}{30.70694677}
\toyPoint{10.89199251}{37.68674239}
\toyPoint{38.03125993}{11.09538048}
\toyPoint{53.19331354}{18.38016787}
\toyPoint{24.29020759}{57.78460779}
\toyPoint{14.99262133}{36.51717794}
\toyPoint{23.08772887}{58.37735330}
\toyPoint{56.35765414}{60.66347830}
\toyPoint{39.56517450}{11.67487914}
\toyPoint{19.83525953}{20.23147275}
\toyPoint{56.04429522}{59.62386870}
\toyPoint{50.46450138}{58.78620732}
\toyPoint{41.14107709}{64.21669960}
\toyPoint{56.34096792}{60.14754357}
\toyPoint{55.42574206}{59.01663349}
\toyPoint{57.54763203}{21.10499843}
\toyPoint{58.12193932}{21.23987106}
\toyPoint{44.37834032}{59.40241937}
\toyPoint{11.65947268}{37.87150871}
\toyPoint{56.30565736}{48.78870564}
\toyPoint{39.91943644}{64.22463356}
\toyPoint{22.18463621}{58.51793105}
\toyPoint{13.81432441}{38.42652169}
\toyPoint{39.96876351}{64.84087636}
\toyPoint{14.30942751}{35.03070731}
\toyPoint{10.83928816}{33.05803776}
\toyPoint{23.64373022}{58.31340944}
\toyPoint{23.35185359}{58.56004500}
\toyPoint{56.31644003}{60.64105157}
\toyPoint{23.37982085}{58.42070087}
\toyPoint{39.80897000}{11.97290851}
\toyPoint{65.02609684}{41.45522020}
\toyPoint{12.27382045}{38.21867751}
\toyPoint{38.73145723}{10.89302001}
\toyPoint{53.87351098}{61.11932847}
\toyPoint{54.45934388}{57.65828440}
\toyPoint{57.77479418}{22.22770691}
\toyPoint{13.75418448}{38.35749961}
\toyPoint{39.68309422}{11.12898058}
\toyPoint{40.26446139}{13.14402057}
\toyPoint{20.59369210}{20.19459632}
\toyPoint{23.52852637}{58.50997402}
\toyPoint{41.95289293}{66.13777345}
\toyPoint{38.99653485}{12.01400572}
\toyPoint{58.53718911}{21.04521382}
\toyPoint{54.74220368}{18.51157342}
\toyPoint{12.16237899}{37.66565773}
\toyPoint{37.85096530}{11.10902417}
\toyPoint{13.31541738}{38.79024000}
\toyPoint{50.88328131}{61.72225060}
\toyPoint{58.40873072}{20.77009878}
\toyPoint{61.02583147}{19.84694973}
\toyPoint{56.05594235}{59.58514952}
\toyPoint{23.20723041}{58.62417806}
\toyPoint{22.87195236}{58.28471768}
\toyPoint{23.11530236}{58.25754719}
\toyPoint{23.21966663}{59.33742646}
\toyPoint{64.41039393}{40.64267444}
\toyPoint{54.61874746}{57.62749918}
\toyPoint{18.11360205}{18.69451738}
\toyPoint{59.30012088}{20.77692216}
\toyPoint{22.36340861}{57.27164791}
\toyPoint{53.79425603}{60.76130221}
\toyPoint{65.05177375}{39.75493872}
\toyPoint{42.04559161}{66.31693809}
\toyPoint{64.85763334}{41.54385865}
\toyPoint{38.62469627}{11.43396870}
\toyPoint{64.71486522}{40.38936143}
\toyPoint{16.97271685}{18.82398328}
\toyPoint{64.70128305}{40.54785095}
\toyPoint{65.10451348}{40.36114113}
\toyPoint{23.85483373}{58.58483130}
\toyPoint{56.86450743}{21.34449836}
\toyPoint{21.77113533}{59.58866735}
\toyPoint{40.27036763}{64.87231993}
\toyPoint{38.61700246}{62.90259177}
\toyPoint{23.02749664}{58.95443393}
\toyPoint{17.43804993}{17.76179314}
\toyPoint{65.58573446}{41.03791846}
\toyPoint{56.17924629}{59.94487239}
\toyPoint{57.65860434}{22.44550613}
\toyPoint{56.06885848}{59.49071730}
\toyPoint{16.18948567}{18.42953743}
\toyPoint{11.68806445}{37.19256682}
\toyPoint{61.27439745}{29.99330997}
\toyPoint{11.56204101}{37.79917213}
\toyPoint{53.82129423}{60.23844411}
\toyPoint{58.81734171}{19.96324416}
\toyPoint{14.04981429}{38.44069010}
\toyPoint{63.56826567}{37.51034879}
\toyPoint{23.32325874}{58.60551834}
\toyPoint{23.10930037}{58.47902421}
\toyPoint{66.03137416}{40.95332813}
\toyPoint{37.86018575}{10.99991768}
\toyPoint{64.70902320}{40.31923830}
\toyPoint{19.88988507}{19.96233663}
\toyPoint{56.67177293}{60.44286420}
\toyPoint{21.12888798}{19.09382697}
\toyPoint{18.42366157}{20.19744812}
\toyPoint{61.50196721}{19.57565246}
\toyPoint{57.27163868}{21.34811771}
\toyPoint{38.73524846}{12.51692741}
\toyPoint{58.87716785}{21.08116734}
\toyPoint{65.47041524}{41.14392263}
\toyPoint{64.83000448}{38.66167624}
\toyPoint{59.19681641}{19.87965615}
\toyPoint{58.21781128}{20.77591158}
\toyPoint{65.37958084}{40.85322963}
\toyPoint{53.92567696}{60.84646840}
\toyPoint{54.35525033}{56.07529425}
\toyPoint{23.00090144}{58.41716305}
\toyPoint{65.20102532}{41.22255500}
\toyPoint{16.45733587}{18.87271912}
\toyPoint{65.95592622}{41.11603727}
\toyPoint{65.82103668}{41.08479483}
\toyPoint{54.19335488}{58.04231982}
\toyPoint{38.73141377}{11.41826691}
\toyPoint{40.33229243}{65.37977311}
\toyPoint{23.13907346}{58.26460438}
\toyPoint{17.64878119}{18.05693996}
\toyPoint{59.16568202}{21.01634056}
\toyPoint{55.56661513}{59.34066434}
\toyPoint{55.83340091}{57.48882109}
\toyPoint{23.90358494}{58.51448705}
\toyPoint{39.05313888}{64.67778575}
\toyPoint{40.80584749}{11.37842486}
\toyPoint{39.92168469}{11.09987197}
\toyPoint{22.80845919}{58.54468930}


==> figures/toy8_native_data/nextgan_5000.tex <==
% Generated from original vector marker centers; do not edit by hand.
\toyPoint{59.35101632}{22.23411960}
\toyPoint{56.13680624}{19.86358212}
\toyPoint{29.86367256}{65.15841607}
\toyPoint{21.24793883}{23.59532972}
\toyPoint{6.67594294}{43.81300680}
\toyPoint{53.83319516}{60.52176229}
\toyPoint{21.15600617}{24.03406297}
\toyPoint{34.36275075}{66.56838509}
\toyPoint{63.66362079}{38.88609244}
\toyPoint{57.77617393}{56.78973167}
\toyPoint{47.48922517}{12.86911934}
\toyPoint{53.97955956}{59.44744202}
\toyPoint{16.32316312}{50.30279744}
\toyPoint{47.69893815}{12.79994718}
\toyPoint{63.93877891}{45.04076558}
\toyPoint{53.50344227}{18.30294640}
\toyPoint{15.11754497}{29.66590205}
\toyPoint{69.20459624}{32.53776612}
\toyPoint{7.87890773}{44.49467744}
\toyPoint{31.02247069}{66.04787580}
\toyPoint{60.02634694}{57.35903063}
\toyPoint{64.10920358}{27.93655057}
\toyPoint{51.91325341}{16.71223456}
\toyPoint{10.98583714}{48.58669742}
\toyPoint{61.12103585}{50.07161986}
\toyPoint{18.06929465}{23.35919534}
\toyPoint{23.78104394}{20.13574846}
\toyPoint{21.66696333}{55.90600629}
\toyPoint{63.49917966}{47.82954539}
\toyPoint{59.27852938}{60.77563040}
\toyPoint{47.98499584}{13.16271874}
\toyPoint{44.66739285}{64.72176552}
\toyPoint{18.37758680}{62.17233412}
\toyPoint{12.58175265}{37.16742558}
\toyPoint{40.34969502}{64.29509009}
\toyPoint{62.49566816}{65.36384060}
\toyPoint{24.49614740}{19.83334449}
\toyPoint{20.82600409}{20.61441606}
\toyPoint{14.82154139}{51.30507069}
\toyPoint{69.43641909}{31.74618952}
\toyPoint{39.07993424}{13.17177865}
\toyPoint{29.99344457}{64.60140874}
\toyPoint{32.51352741}{66.65290833}
\toyPoint{55.18847712}{20.64269250}
\toyPoint{50.02675949}{61.49076308}
\toyPoint{39.36674675}{13.27557225}
\toyPoint{21.29353985}{23.90213290}
\toyPoint{12.17066057}{48.29447239}
\toyPoint{18.06232975}{54.88903876}
\toyPoint{9.31957122}{43.94519914}
\toyPoint{28.14647275}{68.42891447}
\toyPoint{16.92233209}{50.67437664}
\toyPoint{8.51500542}{43.46386087}
\toyPoint{28.62083189}{21.94469329}
\toyPoint{47.61608924}{12.69476614}
\toyPoint{59.01220968}{60.25230469}
\toyPoint{31.00449700}{66.08584127}
\toyPoint{23.51339679}{20.30688070}
\toyPoint{72.00443637}{33.33623302}
\toyPoint{61.34692131}{52.47818239}
\toyPoint{59.40598488}{57.22877564}
\toyPoint{56.46883103}{19.57849349}
\toyPoint{11.03300402}{41.08093716}
\toyPoint{49.79059665}{14.31684771}
\toyPoint{61.16387275}{55.35527475}
\toyPoint{12.18299373}{48.37266368}
\toyPoint{39.87329952}{66.49965594}
\toyPoint{39.50230770}{66.47277463}
\toyPoint{8.00557413}{43.30668995}
\toyPoint{42.07463695}{12.31828320}
\toyPoint{18.87932408}{22.45907599}
\toyPoint{21.21769967}{65.46183217}
\toyPoint{60.73784490}{55.11111567}
\toyPoint{62.92386486}{27.30414760}
\toyPoint{28.23446843}{62.51651979}
\toyPoint{68.05415738}{32.03321088}
\toyPoint{39.92143777}{65.06127819}
\toyPoint{19.28300211}{21.88754974}
\toyPoint{53.72698968}{18.03798952}
\toyPoint{59.75248706}{57.11570217}
\toyPoint{16.62616699}{26.67740822}
\toyPoint{67.32761137}{30.10650035}
\toyPoint{35.12473691}{66.68124783}
\toyPoint{15.20496461}{50.76385283}
\toyPoint{46.01610599}{13.67673689}
\toyPoint{14.49330207}{48.38326946}
\toyPoint{6.39156957}{43.83500822}
\toyPoint{59.43841288}{54.06392744}
\toyPoint{23.93719427}{23.12325170}
\toyPoint{28.49988214}{63.67942718}
\toyPoint{19.83618552}{20.97317911}
\toyPoint{67.17267929}{30.11215087}
\toyPoint{19.52422634}{62.01235833}
\toyPoint{4.43709712}{48.27545966}
\toyPoint{31.37865959}{31.67757034}
\toyPoint{50.24663679}{15.01696617}
\toyPoint{69.81922396}{38.59439375}
\toyPoint{65.53159345}{30.57752394}
\toyPoint{20.71291370}{20.87942831}
\toyPoint{9.45319022}{44.63354703}
\toyPoint{42.84974498}{63.50874101}
\toyPoint{8.34753713}{43.32907246}
\toyPoint{59.63495285}{56.71613878}
\toyPoint{63.98573199}{45.29683136}
\toyPoint{13.40652097}{34.83579051}
\toyPoint{15.93669276}{52.23245282}
\toyPoint{14.85733032}{48.50385851}
\toyPoint{8.61822067}{43.54228904}
\toyPoint{21.17684857}{22.52280143}
\toyPoint{57.39154016}{23.42674778}
\toyPoint{60.98275615}{53.61688029}
\toyPoint{31.39931433}{66.20157426}
\toyPoint{9.59949616}{41.50128757}
\toyPoint{19.57374665}{21.94222143}
\toyPoint{48.04812062}{63.48802782}
\toyPoint{23.09074063}{22.77872301}
\toyPoint{21.85479103}{62.46599044}
\toyPoint{21.41455650}{55.81482580}
\toyPoint{20.31452856}{55.60557119}
\toyPoint{73.60278529}{31.68258944}
\toyPoint{9.43129878}{45.28134146}
\toyPoint{9.95162349}{43.93427149}
\toyPoint{21.71019708}{24.52661114}
\toyPoint{58.92648358}{59.50932011}
\toyPoint{62.66657429}{46.00101525}
\toyPoint{61.76792545}{25.69151663}
\toyPoint{24.33261071}{65.20809635}
\toyPoint{12.31419471}{40.37218676}
\toyPoint{60.88775942}{24.39390890}
\toyPoint{12.90095052}{37.56997824}
\toyPoint{30.60850913}{65.47353314}
\toyPoint{61.57468027}{30.47575920}
\toyPoint{16.45330737}{27.12886226}
\toyPoint{58.19870087}{18.28415440}
\toyPoint{9.68744647}{45.80777468}
\toyPoint{63.19010304}{43.01693005}
\toyPoint{65.75798188}{28.79754928}
\toyPoint{63.95139202}{46.83540452}
\toyPoint{49.83254525}{14.59184277}
\toyPoint{72.69811138}{35.58884367}
\toyPoint{31.01361690}{65.96310954}
\toyPoint{30.81499192}{17.32130328}
\toyPoint{34.64463649}{70.76395219}
\toyPoint{26.32832189}{60.69487726}
\toyPoint{9.06757355}{43.90127436}
\toyPoint{46.20574567}{63.42641584}
\toyPoint{15.63141700}{28.77107097}
\toyPoint{21.97389726}{23.64550683}
\toyPoint{61.29207888}{49.51687521}
\toyPoint{12.93820843}{52.73472002}
\toyPoint{27.43366887}{61.38984896}
\toyPoint{61.94383067}{39.08052702}
\toyPoint{20.20647110}{20.46518449}
\toyPoint{59.14336143}{55.00016951}
\toyPoint{13.77711573}{31.97985588}
\toyPoint{44.29824898}{64.45444138}
\toyPoint{43.91982986}{12.19491159}
\toyPoint{62.59143706}{47.42821232}
\toyPoint{9.94676898}{44.86890962}
\toyPoint{19.54778825}{58.85911726}
\toyPoint{64.43168240}{27.86968800}
\toyPoint{58.65507095}{54.45898087}
\toyPoint{54.13314727}{60.52735821}
\toyPoint{54.76129563}{59.30222973}
\toyPoint{26.34953191}{65.33377524}
\toyPoint{25.75166425}{20.33651690}
\toyPoint{46.51250424}{66.42662910}
\toyPoint{19.28522633}{21.69759012}
\toyPoint{44.18095704}{11.50057208}
\toyPoint{43.64197031}{65.65336074}
\toyPoint{29.24192152}{63.66191033}
\toyPoint{8.44935879}{43.13542024}
\toyPoint{20.44870130}{54.91478643}
\toyPoint{26.04899837}{59.98849069}
\toyPoint{13.42588978}{47.79219597}
\toyPoint{69.04015818}{33.29666630}
\toyPoint{25.01013940}{61.33261619}
\toyPoint{12.83655597}{40.02524235}
\toyPoint{18.33788626}{54.52551965}
\toyPoint{32.07313599}{16.48169764}
\toyPoint{58.37813316}{59.78224939}
\toyPoint{62.75484608}{50.65731202}
\toyPoint{61.30622710}{54.84522820}
\toyPoint{7.54742284}{42.78165302}
\toyPoint{49.98487242}{60.76516151}
\toyPoint{21.64182478}{24.31079465}
\toyPoint{13.79823500}{41.38843934}
\toyPoint{21.14983343}{22.70896635}
\toyPoint{58.96405835}{24.15790219}
\toyPoint{14.26814879}{49.08321719}
\toyPoint{9.63975353}{44.53868912}
\toyPoint{51.40626938}{61.25352275}
\toyPoint{46.82802123}{12.53705302}
\toyPoint{28.51205303}{21.24200452}
\toyPoint{53.59496270}{18.55180771}
\toyPoint{33.60949839}{66.66262042}
\toyPoint{15.22647150}{54.26747384}
\toyPoint{64.02347134}{34.66769580}
\toyPoint{57.88711394}{23.06573283}
\toyPoint{17.48483073}{54.31650808}
\toyPoint{56.96467553}{57.98493324}
\toyPoint{50.33782805}{16.04337046}
\toyPoint{12.40360937}{33.90011949}
\toyPoint{16.35674323}{26.27726801}
\toyPoint{63.78100272}{35.80714241}
\toyPoint{59.15271359}{23.06068759}
\toyPoint{52.10467431}{59.11541570}
\toyPoint{42.31552143}{13.92972208}
\toyPoint{66.14478142}{28.85978268}
\toyPoint{28.96318943}{19.43264592}
\toyPoint{7.65559412}{42.99019564}
\toyPoint{38.69536094}{60.71144196}
\toyPoint{26.11399128}{17.92095523}
\toyPoint{62.32531732}{50.85657458}
\toyPoint{49.91408440}{14.66638780}
\toyPoint{62.41919271}{25.77765034}
\toyPoint{58.93347002}{54.83466087}
\toyPoint{20.98781647}{22.28599333}
\toyPoint{17.70176088}{57.77507567}
\toyPoint{30.03642451}{17.96899273}
\toyPoint{46.92687650}{12.89339804}
\toyPoint{23.50976975}{65.25269139}
\toyPoint{63.67457728}{42.34850953}
\toyPoint{52.77053894}{59.73873877}
\toyPoint{57.72751193}{21.67922266}
\toyPoint{21.03525869}{21.56026256}
\toyPoint{42.36119263}{11.69029790}
\toyPoint{51.20598854}{60.93500168}
\toyPoint{20.25656669}{23.17638674}
\toyPoint{9.90203242}{44.69893063}
\toyPoint{61.29900532}{24.26118666}
\toyPoint{38.33564181}{66.71431880}
\toyPoint{66.61808075}{41.19819920}
\toyPoint{11.92681220}{39.90983468}
\toyPoint{54.18379353}{58.81097824}
\toyPoint{12.46704101}{47.15407556}
\toyPoint{20.87092215}{23.05058479}
\toyPoint{14.00500390}{52.83876588}
\toyPoint{59.38778200}{55.44764734}
\toyPoint{11.16590931}{46.28157047}
\toyPoint{17.91349811}{23.67699500}
\toyPoint{33.70765763}{66.29138885}
\toyPoint{49.03518892}{14.98704234}
\toyPoint{59.00318976}{60.24817467}
\toyPoint{62.77121236}{27.31720448}
\toyPoint{50.76994096}{15.39973720}
\toyPoint{6.24659877}{44.09442955}
\toyPoint{27.35083995}{17.33382717}
\toyPoint{34.76605385}{14.84002575}
\toyPoint{21.96395289}{57.54445568}
\toyPoint{65.97383684}{40.76581269}
\toyPoint{62.18250767}{47.00469555}
\toyPoint{9.41575081}{39.56027846}
\toyPoint{19.97019522}{58.08379543}
\toyPoint{20.31356412}{20.58080827}
\toyPoint{30.92599192}{65.89607239}
\toyPoint{45.04217071}{63.27051470}
\toyPoint{59.67107250}{23.47736636}
\toyPoint{30.52118563}{65.23451467}
\toyPoint{56.42685552}{58.87424992}
\toyPoint{11.29649501}{45.58300403}
\toyPoint{60.49090939}{56.68921594}
\toyPoint{44.99795291}{13.62235285}
\toyPoint{34.20881579}{69.35188047}
\toyPoint{21.19498068}{21.66477911}
\toyPoint{46.77656512}{12.50075186}
\toyPoint{56.24137355}{58.77316660}
\toyPoint{19.11462630}{21.14599259}
\toyPoint{29.88024496}{65.45301837}
\toyPoint{29.42070546}{59.80806320}
\toyPoint{31.07805298}{66.05362246}
\toyPoint{12.28049617}{46.33368338}
\toyPoint{64.40338750}{28.21673932}
\toyPoint{40.18761529}{12.24062028}
\toyPoint{49.31036395}{15.25392963}
\toyPoint{25.74256589}{21.15947939}
\toyPoint{73.11734046}{34.23224888}
\toyPoint{42.60280640}{11.95674219}
\toyPoint{64.58908942}{40.12441689}
\toyPoint{18.44082925}{22.87705606}
\toyPoint{46.37851800}{11.91739236}
\toyPoint{60.55201992}{62.72435927}
\toyPoint{55.65707576}{19.29187744}
\toyPoint{36.95489368}{13.12341506}
\toyPoint{48.37205148}{15.20010548}
\toyPoint{31.19855358}{67.14819754}
\toyPoint{36.71748377}{67.02365998}
\toyPoint{30.21327419}{65.65799682}
\toyPoint{64.78132709}{35.33447335}
\toyPoint{22.25570802}{60.43235994}
\toyPoint{37.14724133}{14.47847859}
\toyPoint{29.20591339}{63.63047754}
\toyPoint{60.49883719}{23.46417335}
\toyPoint{9.14482732}{43.04066347}
\toyPoint{28.78641205}{19.93296500}
\toyPoint{46.44658112}{14.56301566}
\toyPoint{31.57112106}{67.41673993}
\toyPoint{22.28252319}{62.36014489}
\toyPoint{19.11164837}{53.01395201}
\toyPoint{59.51638345}{63.80850392}
\toyPoint{35.85321334}{14.54774149}
\toyPoint{12.63924076}{44.96786256}
\toyPoint{57.91328153}{59.24657668}
\toyPoint{57.12856600}{58.90754392}
\toyPoint{31.71311009}{67.56968160}
\toyPoint{59.22650183}{59.53075317}
\toyPoint{59.93870735}{57.41005528}
\toyPoint{59.46157640}{24.71048724}
\toyPoint{56.86059429}{20.95848791}
\toyPoint{60.47630433}{51.33233040}
\toyPoint{9.47268209}{44.00936873}
\toyPoint{60.44582674}{51.41940394}
\toyPoint{48.31974014}{62.29023595}
\toyPoint{32.72300351}{70.71601006}
\toyPoint{13.65136300}{47.69938884}
\toyPoint{54.20754156}{58.48501544}
\toyPoint{15.10885269}{55.80986054}
\toyPoint{9.71657661}{39.38668397}
\toyPoint{21.89258422}{55.43135028}
\toyPoint{24.50176177}{58.53820739}
\toyPoint{59.15767270}{62.45459710}
\toyPoint{26.21613133}{60.14923865}
\toyPoint{37.99805706}{14.74607498}
\toyPoint{67.79748055}{40.31805065}
\toyPoint{11.06614267}{45.20552243}
\toyPoint{43.52222458}{11.67733100}
\toyPoint{60.84728518}{51.22532660}
\toyPoint{65.03438611}{39.60421836}
\toyPoint{65.01346988}{29.06591092}
\toyPoint{17.90451819}{60.83980037}
\toyPoint{41.31921345}{12.33334203}
\toyPoint{43.54745811}{14.11415962}
\toyPoint{15.73181891}{51.99682297}
\toyPoint{26.70163154}{60.54897431}
\toyPoint{30.96032112}{65.95155470}
\toyPoint{39.50214355}{14.19434978}
\toyPoint{56.33172343}{21.16744718}
\toyPoint{46.19134441}{14.26116236}
\toyPoint{12.68014108}{49.76859677}
\toyPoint{26.03572692}{22.65956756}
\toyPoint{14.50451389}{48.54192703}
\toyPoint{58.94484489}{55.15268664}
\toyPoint{50.07959150}{15.33670702}
\toyPoint{46.85332744}{12.35192330}
\toyPoint{61.21184872}{54.57297264}
\toyPoint{18.96895716}{52.91159199}
\toyPoint{29.05502750}{64.20999927}
\toyPoint{19.54656539}{52.97090438}
\toyPoint{29.34097982}{63.62498776}
\toyPoint{63.48405776}{30.78591639}
\toyPoint{64.47851704}{32.53265935}
\toyPoint{20.84865078}{22.91999755}
\toyPoint{51.98476053}{16.84527213}
\toyPoint{32.82061284}{66.55075750}
\toyPoint{63.03436187}{44.38150821}
\toyPoint{61.24147415}{22.29321357}
\toyPoint{30.91626752}{65.84823485}
\toyPoint{70.35515816}{37.87609347}
\toyPoint{29.40047910}{18.38681590}
\toyPoint{65.06508212}{40.97306073}
\toyPoint{19.87710891}{20.52702719}
\toyPoint{62.97592471}{27.94799005}
\toyPoint{66.24531407}{36.64352479}
\toyPoint{24.85491506}{59.62211517}
\toyPoint{62.28488153}{27.20164299}
\toyPoint{34.86854730}{70.36644228}
\toyPoint{33.25265192}{66.89276972}
\toyPoint{53.03427911}{61.00812389}
\toyPoint{29.47215695}{63.90146102}
\toyPoint{21.10108991}{22.54198874}
\toyPoint{69.39356219}{34.77289454}
\toyPoint{60.10967654}{56.20891786}
\toyPoint{55.20462344}{19.00921760}
\toyPoint{59.27241048}{58.78780703}
\toyPoint{18.37639470}{21.89519298}
\toyPoint{9.18944389}{44.68499622}
\toyPoint{65.09134200}{29.04905858}
\toyPoint{9.04623278}{43.71351050}
\toyPoint{63.96809209}{39.61982896}
\toyPoint{48.58598217}{13.34705784}
\toyPoint{11.88870215}{49.59414359}
\toyPoint{64.75340289}{28.09245325}
\toyPoint{28.89775814}{63.39856394}
\toyPoint{28.72158450}{64.66447430}
\toyPoint{67.57073064}{31.02494486}
\toyPoint{24.30626931}{23.77285465}
\toyPoint{64.05604855}{32.40421403}
\toyPoint{13.08566186}{46.16242963}
\toyPoint{59.59798105}{60.88248960}
\toyPoint{22.51437064}{50.80037086}
\toyPoint{14.93728668}{31.09594899}
\toyPoint{46.42136374}{12.35330766}
\toyPoint{60.37098331}{25.19248347}
\toyPoint{41.29820262}{12.52085286}
\toyPoint{54.14627414}{18.69109338}
\toyPoint{70.26314705}{35.25418397}
\toyPoint{68.61112164}{31.09191510}
\toyPoint{46.56687444}{12.38021358}
\toyPoint{50.11719550}{15.61786559}
\toyPoint{68.16241172}{36.85390649}
\toyPoint{62.66241350}{45.93902373}
\toyPoint{62.65041567}{49.61650879}
\toyPoint{56.83552342}{54.86707041}
\toyPoint{68.60598718}{38.63386404}
\toyPoint{20.75763487}{21.27311737}
\toyPoint{61.26440387}{24.14638889}
\toyPoint{71.32203010}{33.43373237}
\toyPoint{65.36434666}{38.04651334}
\toyPoint{31.20658136}{17.07211741}
\toyPoint{37.47029043}{66.60573529}
\toyPoint{19.51049805}{52.96092464}
\toyPoint{21.21695826}{23.97423683}
\toyPoint{53.24704232}{18.18216662}
\toyPoint{63.38889953}{45.67338351}
\toyPoint{59.34597415}{56.74107890}
\toyPoint{24.81817399}{59.11726767}
\toyPoint{35.65949863}{66.96721785}
\toyPoint{31.80056433}{14.49511251}
\toyPoint{41.61657545}{11.84599907}
\toyPoint{30.81177327}{68.44034933}

